Convergence of denoising diffusion models under the manifold hypothesis

Denoising diffusion models are a recent class of generative models exhibiting state-of-the-art performance in image and audio synthesis. Such models approximate the time-reversal of a forward noising process from a target distribution to a reference density, which is usually Gaussian. Despite their strong empirical results, the theoretical analysis of such models remains limited. In particular, all current approaches crucially assume that the target density admits a density w.r.t. the Lebesgue measure. This does not cover settings where the target distribution is supported on a lower-dimensional manifold or is given by some empirical distribution. In this paper, we bridge this gap by providing the first convergence results for diffusion models in this more general setting. In particular, we provide quantitative bounds on the Wasserstein distance of order one between the target data distribution and the generative distribution of the diffusion model.

==> arxiv/L2_result.tex <==
\section{Wasserstein controls under $\mathrm{L}^2$ errors}
\label{sec:wass-contr-under}

In this section, we replace the assumption \Cref{assum:score_control} by the
following weaker control.

\begin{assumption}
    \label{assum:score_control_L2}
    There exist $\bm{s} \in \rmc(\ccint{0,T} \times \rset^d, \rset^d)$ and
    $\Mtt \geq 0$ such that for any $k \in \{0, \dots, K\}$ and $x_t \in \rset^d$,
  \begin{equation}
    \expeLigne{\normLigne{\bm{s}(T-t_k, Y_k) - \nabla \log p_{T-t_k}(Y_k)}^2} \leq \Mtt^2 \expeLigne{(1+\normLigne{Y_k}^2)} / \sigma_{T-t_k}^4 \eqsp ,
  \end{equation}
  where we recall that $(Y_k)_{k \in \{0, \dots, K\}}$ is given by \eqref{eq:discretization_improved}.
\end{assumption}

Under this assumption, we have the following theorem, which is an extension of
\Cref{thm:convergence_general}. To prove this theorem, we extend \cite[Theorem
4.1]{lee2022convergence} to the Wasserstein distance of order one and weaker
growth conditions.

\begin{theorem}
  \label{thm:convergence_general_L2}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:step_size}, \rref{assum:score_control_L2} that
  $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$, $t_K = T - \vareps$ and
  $\vareps, \Mtt, \Mtt/\zeta, \delta \leq 1/32$.
  % \begin{equation}
  %   \textstyle{
  %     t_N = \sum_{k=0}^{N-1} \gamma_k = T - (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps)) \eqsp . 
  %     }
  % \end{equation}
   Then, there exists $\Dtt_0 \geq 0$ such that
   \begin{equation}
         \wassersteinD[1](\mathcal{L}(Y_K), \pi) \leq \Dtt_0 (K \zeta + \exp[\kappa/\vareps] (\Mtt/\zeta + \delta^{1/2})/ \vareps^2 + \exp[\kappa/\vareps]\exp[-T/\bar{\beta}] + \vareps^{1/2}) \eqsp ,
       \end{equation}
       with $\kappa = \diam(\M)^2(1+\bar{\beta})/2$ and
       \begin{equation}
         \label{eq:constant_diam_app}         
         \Dtt_0 = D (1 + \bar{\beta})^5(1 + d + \diam(\M)^4) (1 + \log(1 + \diam(\M))) \eqsp ,
       \end{equation}
       and $D$ is a numerical constant.
     \end{theorem}

     We start with the following lemma, which is an extension of
     \Cref{lemma:control_growth_discrete_process} to the setting where
     \rref{assum:score_control} is replaced by \rref{assum:score_control_L2}. 

     \begin{lemma}
  \label{lemma:control_growth_discrete_process_weak}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta} and
  \rref{assum:score_control_L2}. Assume that there exists $\delta >0$ such that for
  any $k \in \{0, \dots, K\}$,
  $\gamma_k \beta_{T-t_k} / \sigma_{T-t_k}^2 \leq \delta$. Assume that there
  exists $\eta >0$ such that $A(\delta, \Mtt, \eta, \diam(\M)) > 0$ with
    \begin{align}
      &A(\delta, \Mtt, \eta, \diam(\M)) = 2 - 2\delta - 32 \delta (1
    + \Mtt^2) - 8 \Mtt -
    4\eta \diam(\M) \eqsp , \\
     & B(\delta, \Mtt, \eta, \diam(\M)) = 32\delta (\Mtt^2 +
    \diam(\M)^2) + 2 
    (1+\delta)(\diam(\M)/\eta + \Mtt) + 4 d \eqsp . 
    \end{align}
  Then, we have for any $k \in \{0, \dots, K\}$
  \begin{equation}
    \label{eq:Ktt_def_l2}
      \expeLigne{\normLigne{Y_k}^2} \leq \Ktt = d + B(\delta, \Mtt, \eta, \diam(\M))(1/A(\delta, \Mtt, \eta, \diam(\M)) + \delta) \eqsp .
    \end{equation}
    In particular if $\Mtt \leq 1/32$ and $\delta \leq 1/32$ then for any $k \in \{0, \dots, K\}$
    \begin{equation}
      \expeLigne{\normLigne{Y_k}^2} \leq \Ktt_0 = 5d + 320 (1+ \diam(\M))^2 \eqsp . 
    \end{equation}
  \end{lemma}

  \begin{proof}
    Recall that using \eqref{eq:discretization_improved}, we have that for any $k \in \{0, \dots, K-1\}$
    \begin{equation}
      \label{eq:discretization_improved_deet}
    \textstyle{
      Y_{k+1} = Y_k + (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1) (Y_{k} + 2 \bm{s}(T-t_k, Y_{k})) + (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)^{1/2} Z_k \eqsp ,
      }
    \end{equation}
    For simplicity, we denote
    \begin{equation}
      \textstyle{ \gamma_{1,k} = (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)/\beta_{T-t_k} \eqsp , \qquad \gamma_{2,k} = (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)/(2\beta_{T-t_k}) \eqsp . }
    \end{equation}
    Then, \eqref{eq:discretization_improved_deet} can be rewritten for any $k \in \{0, \dots, K-1\}$ as
    \begin{equation}
      \label{eq:discretization_improved_deet_duo}
          \textstyle{
      Y_{k+1} = Y_k + \gamma_{1,k} \beta_{T-t_k} (Y_{k} + 2 \bm{s}(T-t_k, Y_{k})) + \sqrt{2 \gamma_{2,k} \beta_{T-t_k}} Z_k \eqsp .
      }
    \end{equation}
    In what follows, we denote $\bar{\gamma}_{1,k} = \gamma_{1,k} \beta_{T-t_k}$
    and $\bar{\gamma}_{2,k} = \gamma_{2,k} \beta_{T-t_k}$. In addition, using
    that $\gamma_k \beta_{T-t_k} \leq \delta \leq 1/4$, we have that
    $\gamma_{1,k} \leq \gamma_{2,k} \leq 2 \gamma_{1,k}$.
    Indeed, we have that for any $k \in \{0, \dots, K-1\}$
    \begin{align}
      &\textstyle{\gamma_{2,k} / \gamma_{1,k} = (1/2) (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] + 1) \geq 1 \eqsp ,} \\ 
        &\textstyle{\gamma_{2,k} / \gamma_{1,k} = (1/2) (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] + 1) \leq (1/2)(\exp[\gamma_k \beta_{T-t_k}] + 1) \leq 2 \eqsp ,}
    \end{align}
    In what follows, for any $t\in \ccint{0,T}$ and $x_t \in \rset^d$, we denote
    $\Delta_t = \normLigne{\bm{s}(t,x_t) - \nabla \log p_t(x_t)}$.  Using
    \Cref{lemma:control_grad}, we have that for any $t \in \ccint{0,T}$,
    $x_t \in \rset^d$ and $\eta >0$
    \begin{align}
      \langle x_t, \bm{s}(t, x_t) \rangle &\leq -\normLigne{x_t}^2/\sigma_t^2 + m_t \diam(\M)\normLigne{x_t}/\sigma_t^2 +  \Delta_t(x_t) \normLigne{x_t}  \\
      &\leq (-1 + \eta  m_t \diam(\M))\norm{x_t}^2/\sigma_t^2 + (m_t \diam(\M)/\eta) / \sigma_t^2 +  \Delta_t(x_t) \normLigne{x_t} \eqsp , \label{eq:s_scalar_product}
    \end{align}
    where we have used that for any $a,b \geq 0$, $2ab \leq \eta a^2 + b^2/\eta$
    in the last line.  In addition, using \Cref{lemma:control_grad}, for any
    $t \in \ccint{0,T}$ and $x_t \in \rset^d$ we have
    \begin{align}      
      \normLigne{\bm{s}(t, x_t)}^2 &\leq 2 \normLigne{\bm{s}(t, x_t) - \nabla \log p_t(x_t)}^2 + 2 \normLigne{\nabla \log p_t(x_t)}^2 \\
                                   &\leq 2\Delta_t(x_t)^2 + 4 \normLigne{x_t}^2/\sigma_t^4 + 4 m_t^2 \diam(\M)^2/\sigma_t^4 \eqsp , \label{eq:s_norm_control}
    \end{align}
    In addition, using \rref{assum:score_control_L2}, the Cauchy-Schwarz
    inequality and \eqref{eq:s_scalar_product} we have
    \begin{align}
      &\expeLigne{\langle Y_k, \bm{s}(T-t_k, Y_k)\rangle } \leq (-1 + \eta  m_{T-t_k} \diam(\M))\expeLigne{\norm{Y_k}^2}/\sigma_{T-t_k}^2 + (m_{T-t_k} \diam(\M)/\eta) / \sigma_{T-t_k}^2 \\
                                                                  & \qquad \qquad + \expeLigne{\Delta_{T-t_k}(Y_k) \normLigne{Y_k}} \\ 
                                                                    &\leq (-1 + \eta  m_{T-t_k} \diam(\M))\expeLigne{\norm{Y_k}^2}/\sigma_{T-t_k}^2 + (m_{T-t_k} \diam(\M)/\eta) / \sigma_{T-t_k}^2 \\
                                                                  & \qquad + \sqexpeLigne{ \Delta_{T-t_k}(Y_k)^2} \sqexpeLigne{\normLigne{Y_k}^2} \\ 
&\leq (-1 + \eta  m_{T-t_k} \diam(\M))\expeLigne{\norm{Y_k}^2}/\sigma_{T-t_k}^2 + (m_{T-t_k} \diam(\M)/\eta) / \sigma_{T-t_k}^2 \\
                                                                  & \qquad + \Mtt (1 + \sqexpeLigne{\normLigne{Y_k}^2}) \sqexpeLigne{\normLigne{Y_k}^2}/\sigma_{T-t_k}^2 \\
      &\leq (-1 + \eta  m_{T-t_k} \diam(\M)+\Mtt)\expeLigne{\norm{Y_k}^2}/\sigma_{T-t_k}^2 + (m_{T-t_k} \diam(\M)/\eta) / \sigma_{T-t_k}^2  + \Mtt \sqexpeLigne{\normLigne{Y_k}^2}/\sigma_{T-t_k}^2 \\
&\leq (-1 + \eta  m_{T-t_k} \diam(\M)+2 \Mtt)\expeLigne{\norm{Y_k}^2}/\sigma_{T-t_k}^2 + (m_{T-t_k} \diam(\M)/\eta + \Mtt) / \sigma_{T-t_k}^2   \eqsp . \label{eq:s_scalar_product_esperance}
    \end{align}
    Finally, using \rref{assum:score_control_L2} and \eqref{eq:s_norm_control} we have
    \begin{align}
      \expeLigne{\normLigne{\bm{s}(T-t_k, Y_k)}^2} &\leq 4\expeLigne{\Delta_{T-t_k}(Y_k)^2} + 4 \expeLigne{\normLigne{Y_{k}}^2}/\sigma_{T-t_k}^4 + 4 m_{T-t_k}^2 \diam(\M)^2/\sigma_{T-t_k}^4 \\
                                                   & \leq  4\Mtt^2 (1 + \expeLigne{\normLigne{Y_k}^2})/\sigma_{T-t_k}^4 + 4 \expeLigne{\normLigne{Y_{k}}^2}/\sigma_{T-t_k}^4 + 4 m_{T-t_k}^2 \diam(\M)^2/\sigma_{T-t_k}^4 \\
      & \leq  4 (1 + \Mtt^2) \expeLigne{\normLigne{Y_k}^2})/\sigma_{T-t_k}^4 + 4 (\Mtt^2 + m_{T-t_k}^2 \diam(\M)^2)/\sigma_{T-t_k}^4 \eqsp . \label{eq:s_norm_control_esperance}
    \end{align}
    
    Combining \eqref{eq:discretization_improved_deet_duo},
    \eqref{eq:s_scalar_product_esperance} and \eqref{eq:s_norm_control_esperance} we have for any
    $k \in \{0, \dots, K-1\}$
    \begin{align}
      \expeLigne{\normLigne{Y_{k+1}}^2} &= (1 + \bar{\gamma}_{1,k})^2 \expeLigne{\normLigne{Y_{k}}^2} + 4 \bar{\gamma}_{1,k}^2 \expeLigne{\normLigne{\bm{s}(T-t_k, Y_k)}^2} \\
      & \qquad +4 \bar{\gamma}_{1,k} (1 + \bar{\gamma}_{1,k}) \expeLigne{\langle Y_k, \bm{s}(T-t_k, Y_k)\rangle} + 2\bar{\gamma}_{2,k}d \\
                                        &\leq (1 + 2\bar{\gamma}_{1,k} + \bar{\gamma}_{1,k}^2) \expeLigne{\normLigne{Y_k}^2} + 16 (\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
                                        & \qquad + 16(\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (\Mtt^2 + m_{T-t_k}^2 \diam(\M)^2 ) \\
      &\qquad + 4 \bar{\gamma}_{1,k} (1 + \bar{\gamma}_{1,k}) \expeLigne{\langle Y_k, \bm{s}(T-t_k, Y_k)\rangle} + 4\bar{\gamma}_{1,k}d\\
                                        &\leq (1 + 2\bar{\gamma}_{1,k} + \bar{\gamma}_{1,k}^2) \expeLigne{\normLigne{Y_k}^2} + 16 (\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
                                        & \qquad + 16(\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (\Mtt^2 + m_{T-t_k}^2 \diam(\M)^2 ) \\
      & \qquad + 4 (\bar{\gamma}_{1,k}/\sigma_{T-t_k}^2) (1 + \bar{\gamma}_{1,k}) (-1 + 2 \Mtt + \eta m_{T-t_k} \diam(\M))\expeLigne{\norm{Y_k}^2} \\
                                        & \qquad + (\bar{\gamma}_{1,k}/ \sigma_{T-t_k}^2 ) (1 + \bar{\gamma}_{1,k}) (m_{T-t_k} \diam(\M)/\eta + \Mtt) + 4 \bar{\gamma}_{1,k}d \eqsp . 
      %                                   &\leq (1 + 2\bar{\gamma}_{1,k} + \bar{\gamma}_{1,k}^2) \expeLigne{\normLigne{Y_k}^2} + 16 (\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
      %                                   & \qquad + 4(\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (\Mtt^2 + m_{T-t_k}^2 \diam(\M)^2 ) \\
      % & \qquad + 4 (\bar{\gamma}_{1,k}/\sigma_{T-t_k}^2) (1 + \bar{\gamma}_{1,k}) (-1 + 2 \Mtt + \vareps m_{T-t_k} \diam(\M))\expeLigne{\norm{Y_k}^2} \\
      % & \qquad + 2 (\bar{\gamma}_{1,k}/ \sigma_{T-t_k}^2 ) (1 + \bar{\gamma}_{1,k}) (m_{T-t_k} \diam(\M)/\vareps + \Mtt) + 4 \bar{\gamma}_{1,k} \eqsp . 
    \end{align}
    The rest of the proof is identical to the one of \Cref{lemma:control_growth_discrete_process}.
  \end{proof}

  Let $\zeta>0$. For any $k \in \{0, \dots, K\}$ we define $\msa_k$ such that
  \begin{equation}
    \msa_k = \ensembleLigne{y \in \rset^d}{\normLigne{\bm{s}(T-t_k, y) - \nabla \log p_{T-t_k}(y)} > (\Mtt/ \zeta) / \sigma_{T-t_k}^2} \eqsp .
  \end{equation}
  We define the process $(Y_k^\star)_{k \in \{0, \dots, K\}}$ such that
  $Y_0^\star = Y_0$ and for any $k \in \{0, \dots, K-1\}$, if $Y_k = Y_k^\star$
  and $Y_k \in \msa_k$  then $Y_{k+1}^\star = Y_{k+1}$. Otherwise, we define 
  \begin{equation}
    \label{eq:discretization_improved_inter}
    \textstyle{
      Y^\star_{k+1} = Y^\star_k + (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1) (Y^\star_{k} + 2 \nabla \log p_{T-t_k} (Y^\star_{k})) + (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)^{1/2} Z_k \eqsp .
      }
  \end{equation}
  This is similar to assuming that there exists $\bm{s}^\star$ such that for any $k \in \{0, \dots, K-1\}$
    \begin{equation}
    \label{eq:discretization_improved_inter}
    \textstyle{
      Y^\star_{k+1} = Y^\star_k + (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1) (Y^\star_{k} + 2 \bm{s}^\star (T-t_k, Y^\star_{k})) + (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)^{1/2} Z_k \eqsp ,
      }
  \end{equation}
  with $\bm{s}^\star$ which satisfies\footnote{Note that we slightly abuse since
    $\bm{s}^\star$ is random (depending on the behavior of $Y_k$) but one can
    check that all our proofs remain unchanged in this slightly larger setting}
  \rref{assum:score_control} with $\Mtt$ replaced by $\Mtt/\zeta$ and while $Y_k \in \msa_k$,
  $Y_{k+1}^\star = Y_{k+1}$.

  We have the following lemma which is an extension of \cite[Theorem
  4.1]{lee2022convergence} to the Wasserstein setting. Note that contrary to
  \cite[Theorem 4.1]{lee2022convergence} which states results in total variation
  we also need control on the moments of the distribution under a $\mathrm{L}^2$
  error, which is precisely \Cref{lemma:control_growth_discrete_process_weak}.

  \begin{lemma}
    \label{lemma:wasserstein_l2_linf}
    Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta} and
    \rref{assum:score_control_L2}. Assume that there exists $\delta >0$ such
    that for any $k \in \{0, \dots, K\}$,
    $\gamma_k \beta_{T-t_k} / \sigma_{T-t_k}^2 \leq \delta$ and that
    $\Mtt, \Mtt/\zeta, \delta \leq 1/32$.  Then, we have for any
    $k \in \{0, \dots, K\}$
    \begin{equation}
      \expeLigne{\normLigne{Y_k^\star - Y_k}} \leq 4 (1+ \Ktt_0) \zeta k \eqsp ,
    \end{equation}
    where $\Ktt_0$ is defined in \Cref{lemma:control_growth_discrete_process_weak}.
  \end{lemma}

  \begin{proof}
    Using the Cauchy-Schwarz inequality we have
    \begin{align}
      \expeLigne{\normLigne{Y_k^\star - Y_k}} &= \expeLigne{\normLigne{Y_k^\star - Y_k}\1_{Y_k \neq Y_k^\star}} \\
                                              &\leq \textstyle{ \sqrt{2}(\sqexpeLigne{\normLigne{Y_k^\star}^2} + \sqexpeLigne{\normLigne{Y_k}^2}) (\sum_{j=1}^k \probaLigne{Y_j \in \msa_j})^{1/2} } \\
                                              &\leq \textstyle{ \sqrt{2}(\sqexpeLigne{\normLigne{Y_k^\star}^2} + \sqexpeLigne{\normLigne{Y_k}^2})} \\
      & \qquad \times \textstyle{ (\sum_{j=1}^k \probaLigne{\normLigne{\bm{s}(T-t_j, Y_j) - \nabla \log p_{T-t_j}(Y_j)} > (\Mtt/ \zeta) / \sigma_{T-t_j}^2})^{1/2} } \eqsp . \label{eq:cauchy_schwarz_lee}
    \end{align}
    Using the Markov inequality, we have for any $j \in \{0, \dots, K\}$
    \begin{align}
      &\probaLigne{\normLigne{\bm{s}(T-t_j) - \nabla \log p_{T-t_j}(Y_j)} > (\Mtt/ \zeta)  / \sigma_{T-t_j}^2} \\
      & \qquad  \leq \expeLigne{\normLigne{\bm{s}(T-t_j, Y_j) - \nabla \log p_{T-t_j}(Y_j)}^2} \sigma_{T-t_j}^4 \zeta^2 / \Mtt^2 \leq \zeta^2 \expeLigne{1 +\normLigne{Y_j}^2} \eqsp . 
    \end{align}
    Therefore, combining this result, \eqref{eq:cauchy_schwarz_lee} and
    \Cref{lemma:control_growth_discrete_process_weak} we have
    $\expeLigne{\normLigne{Y_k^\star - Y_k}} \leq 4 (1 + \Ktt_0) \zeta k$.
  \end{proof}

We are now ready to complete the proof of \Cref{thm:convergence_general_L2}
  
\begin{proof}
  We have
  \begin{equation}
    \label{eq:ineq_triangle_l2_linf}
    \wassersteinD[1](\mathcal{L}(Y_K), \pi) \leq \wassersteinD[1](\mathcal{L}(Y_K), \mathcal{L}(Y_k^\star)) + \wassersteinD[1](\mathcal{L}(Y_k^\star), \pi) \eqsp . 
  \end{equation}
  Note that using \Cref{thm:convergence_general} we have
  \begin{equation}
   \wassersteinD[1](\mathcal{L}(Y_k^\star), \pi) \leq  \Dtt_0 (\exp[\kappa/\vareps] (\Mtt/ \zeta + \delta^{1/2})/ \vareps^2 + \exp[\kappa/\vareps]\exp[-T/\bar{\beta}] + \vareps^{1/2}) \eqsp .  \label{eq:convergence_Yk_star}
 \end{equation}
 In addition, using \Cref{lemma:wasserstein_l2_linf} we have
 \begin{equation}
   \wassersteinD[1](\mathcal{L}(Y_K), \mathcal{L}(Y_k^\star)) \leq 4 (1+ \Ktt_0) \zeta K \eqsp .
 \end{equation}
 Combining this result and \eqref{eq:convergence_Yk_star} in
 \eqref{eq:ineq_triangle_l2_linf} concludes the proof.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/ack.tex <==
\subsubsection*{Acknowledgements}
\label{sec:acknowledgement}

We thank Arnaud Doucet, \'Emile Mathieu and James Thornton for providing
feedback on an early version of the paper. We thank George Deligiannidis, Alain
Durmus and \'Eric Moulines for useful discussions. Finally, we are indebted to
Pierre Del Moral who pointed us toward his work on stochastic interpolation
formulae.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/backward_control.tex <==
\section{Control of the backward processes}
\label{sec:contr-backw-proc}

We start by introducing the different processes in \Cref{sec:intr-proc}. We
gather a few technical results in \Cref{sec:some-usef-techn}. Then, we turn to
the stability and Lipschitz properties of the backward processes in
\Cref{sec:stab-lipsch-prop}. Finally, we control the growth of the backward
tangent process in \Cref{sec:contr-tang-backw}.


\subsection{Introduction of the processes}
\label{sec:intr-proc}
In this section, we study the stability of the backward process given by
\begin{equation}
  \label{eq:continuous_exact_app}
  \textstyle{
    \rmd \bfY_t = \beta_{T-t} \{ \bfY_t + 2 \nabla \log q_{T-t}(\bfY_t) \} \rmd t + \sqrt{2 \beta_{T-t}} \rmd \bfB_t \eqsp ,
    }
\end{equation}
where $q_t$ is either $p_t$ or
$p_t^N$.  We are also going to
consider the following approximate
continuous-time process
\begin{equation}
  \label{eq:continuous_approximate_app}
  \textstyle{
    \rmd \bhfY_t = \beta_{T-t} \{ \bhfY_t + 2 \bm{s}(T-t, \bhfY_t) \} \rmd t + \sqrt{2 \beta_{T-t} } \rmd \bfB_t \eqsp ,
    }
\end{equation}
where $\bm{s}(t, \cdot)$ is an approximation of either $p_t$ or $p_t^N$. Note
that since $q_t > 0$ and
$q \in \rmc^\infty(\ocint{0, T} \times \rset^d, \rset^d)$ and that
$\bm{s} \in \rmc^1(\ocint{0,T} \times \rset^d, \rset^d)$ we have that
\eqref{eq:continuous_exact_app} and \eqref{eq:continuous_approximate_app} admit strong
solutions up to an explosion time.  Finally, we also consider the following
interpolating process: for any $t \in \coint{t_k, t_{k+1}}$
\begin{equation}
  \label{eq:OU_disc_app}
  \textstyle{
    \rmd \bbfY_t = \beta_{T-t} \{ \bbfY_{t} + 2 \bm{s}(T-t_k, \bbfY_{t_k}) \} \rmd t + \sqrt{2\beta_{T-t}} \rmd \bfB_t \eqsp .
    }
\end{equation}
This process is an interpolation of a modified Euler--Maruyama discretization of
\eqref{eq:continuous_approximate_app}.  Note that the classical Euler--Maruyama
discretization would be associated with the following interpolation
\begin{equation}
  \label{eq:classical_EM_app}
  \textstyle{
    \rmd \bbfY_t^{\EM} = \beta_{T-t_k} \{ \bbfY_{t_k}^{\EM} + 2 \bm{s}(T-t_k, \bbfY_{t_k}^{\EM}) \} \rmd t + \sqrt{2\beta_{T-t_k}} \rmd \bfB_t \eqsp .
    }
\end{equation}
In \eqref{eq:OU_disc_app}, we take advantage of the linear part of the drift. Indeed
on the interval $\ccint{t_k, t_{k+1}}$, the process \eqref{eq:OU_disc_app} is a
simple Ornstein--Ulhenbeck which can be integrated explicitly. In particular for
any $k \in \{0, \dots, N-1\}$ and $t \in \ccint{t_k, t_{k+1}}$ we have
\begin{equation}
  \textstyle{
    \bbfY_t = \bbfY_{t_k} + (\exp[\int_{T-t}^{T-t_k} \beta_s \rmd s] - 1) (\bbfY_{t_k} + 2 \bm{s}(T-t_k, \bbfY_{t_k})) + (\exp[2 \int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)^{1/2} Z \eqsp ,
    }
  \end{equation}
  where $Z$ is a Gaussian random variable with zero mean and identity covariance
  and the equality holds in distribution independent from
  $\bbfY_{t_k}$. Denoting $\{Y_k\}_{k \in \{0, \dots, N-1\}}$, we get that for
  any $k \in \{0, \dots, N-1\}$
  \begin{equation}
    \label{eq:discretization_improved_app}
    \textstyle{
      Y_{k+1} = Y_k + (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1) (Y_{k} + 2 \bm{s}(T-t_k, Y_{k})) + (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)^{1/2} Z_k \eqsp ,
      }
  \end{equation}
  where $\{Z_k\}_{k \in \nset}$ is a collection of independent Gaussian random
  variables with zero mean and identity covariance matrix.  Using this scheme
  instead of the classical Euler--Maruyama simplifies the analysis of the
  discretization. Up to the first order this scheme is equal to the classical
  Euler--Maruyama discretization. Once again, we emphasize that computing this
  scheme is as expensive as computing the classical Euler--Maruyama
  discretization provided that the integral $\int_s^t \beta_u \rmd u$ are
  available in close form for all $s, t \in \ccint{0,T}$ which is the case for
  all the discretization schemes used in practice. We refer to
  \Cref{tab:processes} for a list of all processes used in the proof. In what
  follows, we control the stability of these processes.


  \subsection{Some useful technical lemmas}
  \label{sec:some-usef-techn}
We gather in this section some technical results.

\begin{lemma}
  \label{lemma:integration_lemma}
  For any $s, t \in \ccint{0,T}$ we have
  \begin{align}
    &\textstyle{
      \int_s^t \beta_{T-u}/\sigma_{T-u}^2 \rmd u  = [(-1/2)\log(\exp[2\int_0^{T-u} \beta_v \rmd v] - 1)]_s^t
      } \eqsp ,\label{eq:integral_log} \\
    & \textstyle{
      \int_s^t \beta_{T-u}m_{T-u}^2/\sigma_{T-u}^4 \rmd u  = [(1/2)/(1 - \exp[-2\int_0^{T-u} \beta_v \rmd v])]_s^t \eqsp . 
      } \label{eq:integral_inverse}
  \end{align}
  In particular, if $\beta = \beta_0$ then
  \begin{align}
    &\textstyle{
      \int_s^t \beta_{T-u}/\sigma_{T-u}^2 \rmd u  = [(-1/2)\log(\exp[2\beta_0(T-u)] - 1)]_s^t
      } \eqsp , \\
    & \textstyle{
      \int_s^t \beta_{T-u}m_{T-u}^2/\sigma_{T-u}^4 \rmd u  = [(1/2)/(1 - \exp[-2\beta_0(T-u)])]_s^t \eqsp . 
      }
  \end{align}  
\end{lemma}
\begin{proof}
We have
\begin{align}
  \textstyle{
    \int_s^t \beta_{T-u}/\sigma_{T-u}^2 \rmd u} &= \textstyle{\int_s^t \beta_{T-u} / (1 - \exp[-2\int_0^{T-u} \beta_v \rmd v]) \rmd u 
                                                  } \\
  &= \textstyle{\int_s^t \beta_{T-u} \exp[2\int_0^{T-u} \beta_v \rmd v] / (\exp[2\int_0^{T-u} \beta_v \rmd v] - 1) \rmd u 
    } \\
    &= \textstyle{(-1/2)\int_s^t \partial_u \log(\exp[2\int_0^{T-u} \beta_v \rmd v] - 1) \rmd u 
    } \eqsp .
\end{align}
This concludes the proof of \eqref{eq:integral_log}. We have
\begin{align}
  \textstyle{
  \int_s^t \beta_{T-u}m_{T-u}^2/\sigma_{T-u}^4 \rmd u}  &= \textstyle{\int_s^t \beta_{T-u}m_{T-u}^2/ (1 - \exp[-2\int_0^{T-u} \beta_v \rmd v])^2 \rmd u} \\
                                                        &= \textstyle{\int_s^t \beta_{T-u}\exp[-2\int_0^{T-u} \beta_v \rmd v]/ (1 - \exp[-2\int_0^{T-u} \beta_v \rmd v])^2 \rmd u} \\
                                                            &= \textstyle{(1/2) \int_s^t \partial_u (1 - \exp[-2\int_0^{T-u} \beta_v \rmd v])^{-1} \rmd u} \eqsp .
\end{align}
This concludes the proof of \eqref{eq:integral_inverse}.
\end{proof}


\begin{lemma}
  \label{lemma:bound_sigma_t}
  Assume \rref{assum:assumption_beta}. We have
  $\sigma_{t}^2 \leq 2 t \bar{\beta}$ and
  $\sigma_t^{-2} \leq 1 + \bar{\beta}/(2t) $.
\end{lemma}

\begin{proof}
  First, using that for any $a \geq 0$, $\exp[-a] \geq 1 - a$ we have
  \begin{equation}
    \textstyle{
      \sigma_t^2 = 1 - \exp[-2 \int_0^t \beta_s \rmd s] \leq 1 - \exp[-2\bar{\beta} t] \leq 2 \bar{\beta} t \eqsp .
      }
    \end{equation}
    Second, using that for any $a \geq 0$, $1/(1+\exp[-a]) \leq 1 +1/a$ we have 
  \begin{equation}
    \textstyle{
      \sigma_t^{-2} = (1 - \exp[-2 \int_0^t \beta_s \rmd s])^{-1} \leq 1 + (2\int_0^t \beta_s \rmd s)^{-1} \leq    \eqsp ,
      }
    \end{equation}
    which concludes the proof.
  \end{proof}

  For any $k \in \{0, \dots, K\}$ we introduce $\kappa_k = \sup_{u \in \ccint{T-t_{k+1}, T-t_k}} \beta_u / \sigma_u^2$.
  \begin{lemma}
  \label{lemma:kappa_control}
  Assume \rref{assum:assumption_beta}.  Then, we have that for any
  $k \in \{0, \dots, N-1\}$
  \begin{equation}
    \kappa_k \leq \bar{\beta}(1 + \bar{\beta}/t) \eqsp . 
  \end{equation}
\end{lemma}

\begin{proof}
  Recall that for any $s \in \ccint{0,T}$,
  $\sigma_s^2 = 1 - \exp[-2\int_0^s \beta_u \rmd u]$. Using that for any
  $v \geq 0$, $(1 - \rme^{-2v})^{-1} \leq 1 + 1/(2v)$ we have for any
  $t \in \ocint{0,T}$
  \begin{equation}
    \textstyle{\beta_{t}/\sigma_t^2 \leq \beta_t + \beta_t (2\int_0^t \beta_s \rmd s )^{-1} \leq \beta_t (1 + \bar{\beta}/t)  \eqsp , }
  \end{equation}
  which concludes the proof.
\end{proof}


\subsection{Stability and Lipschitz properties of the backward processes}
\label{sec:stab-lipsch-prop}
The controls derived in \Cref{sec:grad-hess-contr} allow for uniform control of
the moments of the backward processes. Note that such Lyapunov techniques were
used in \citet{fontaine2021convergence} to control energy functionals in convex
optimization problems.  The following lemma is not used directly in our final
analysis but provides intuitive controls on the backward process.
  
  \begin{lemma}
    Assume \rref{assum:manifold_hyp}, \rref{assum:score_control} and that
    there exists $\eta >0$ such that
    $\Mtt + \eta \diam(\M) \leq 1/4$. Then, for any
    $t \in \ccint{0, T}$ we have
    \begin{equation}
      \expeLigne{\normLigne{\bhfY_t}^2} \leq d +  8(1 + \Mtt +  \diam(\M)/\eta)  \eqsp . 
    \end{equation}
    In particular if $\Mtt \leq 1/8$ then
for any
    $t \in \ccint{0, T}$ we have
    \begin{equation}
      \expeLigne{\normLigne{\bhfY_t}^2} \leq d +  8(1 + \Mtt +  8 \diam(\M)^2)  \eqsp . 
    \end{equation}    
  \end{lemma}

  \begin{proof}
    First, using \Cref{lemma:control_grad}, we have that for any
    $t \in \coint{0,T}$, $\expeLigne{\normLigne{\bhfY_t}^2} <+\infty$.  Hence,
    using It\^o's lemma, we have
    \begin{equation}
      \textstyle{
        \rmd (1/2) \normLigne{\bhfY_t}^2 =  \beta_{T-t} \{ \normLigne{\bhfY_t}^2 + 2\langle \bm{s}(T-t, \bhfY_t), \bhfY_t \rangle + 2 \} \rmd t  + \sqrt{2\beta_{T-t}} \langle \bhfY_t, \rmd \bfB_t \rangle \eqsp .
        }
    \end{equation}
    Therefore, using \rref{assum:score_control}, \Cref{lemma:control_grad} and
    that for any $a,b,\eta > 0$, $2ab \leq a^2\eta +b^2/\eta$ we get that for
    any $t \in \coint{0,T}$ we have that
    $(1/2) \expeLigne{\normLigne{\bhfY_t}^2} \leq u_t$, where $u_0 = d/2$ and
    \begin{align}
      \rmd u_t &= \beta_{T-t} (1 - 2/\sigma_{T-t}^2 + 2 (\Mtt + \eta m_{T-t} \diam(\M))/\sigma_{T-t}^2) u_t \\
      & \qquad \qquad + \beta_{T-t} (2 + 2\Mtt +  2m_{T-t} \diam(\M)/\eta)/\sigma_{T-t}^2 \\
               &= \beta_{T-t} (\sigma_{T-t}^2 - 2 + 2 (\Mtt + \eta m_{T-t} \diam(\M)))/\sigma_{T-t}^2 u_t \\
      & \qquad \qquad + \beta_{T-t} (2 + 2\Mtt +  2m_{T-t} \diam(\M)/\eta)/\sigma_{T-t}^2\eqsp . 
    \end{align}
    For any $t \in \ccint{0,T}$ and $x \in \rset$ define $F(t,x)$ given by 
    \begin{equation}
      F(t,x) = -(2 - \sigma_{T-t}^2 - 2 (\Mtt + m_{T-t} \eta \diam(\M)))/\sigma_{T-t}^2 x + (2 + 2\Mtt+2m_{T-t} \diam(\M)/\eta)/\sigma_{T-t}^2 \eqsp . 
    \end{equation}
    Using that for any $t \in \ccint{0,T}$, $m_t, \sigma_t^2 \in \ccint{0,1}$,
    we have that for any $t \in \ccint{0,T}$
    \begin{equation}
      2 - \sigma_{T-t}^2 - 2 (\Mtt + \eta m_{T-t} \diam(\M)) \geq 1 - 2 (\Mtt +  \eta\diam(\M)) \geq 1/2 \eqsp .
    \end{equation}
     % Note that
    % $2(1 + \Mtt + \diam(\M)/\eta)/(1 - 2(\Mtt + \eta \diam(\M)))\geq 1$.
    Using \cite[Lemma 3]{fontaine2021convergence}
    we get that for any $t \in \ccint{0,T}$
    \begin{equation}
      u_t\leq d/2 + 2(1 + \Mtt +  \diam(\M)/\eta)/(1 - 2(\Mtt + \eta \diam(\M)))\leq d/2 + 4(1 + \Mtt +  \diam(\M)/\eta) \eqsp ,
    \end{equation}
    which concludes the proof.
  \end{proof}
  
\begin{lemma}
  \label{lemma:control_growth_discrete_process}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta} and
  \rref{assum:score_control}. Assume that there exists $\delta >0$ such that for
  any $k \in \{0, \dots, K\}$,
  $\gamma_k \beta_{T-t_k} / \sigma_{T-t_k}^2 \leq \delta$. Assume that there
  exists $\eta >0$ such that $A(\delta, \Mtt, \eta, \diam(\M)) > 0$ with
    \begin{align}
      &A(\delta, \Mtt, \eta, \diam(\M)) = 2 - 2\delta - 32 \delta (1
    + \Mtt^2) - 8 \Mtt -
    4\eta \diam(\M) \eqsp , \\
     & B(\delta, \Mtt, \eta, \diam(\M)) = 32\delta (\Mtt^2 +
    \diam(\M)^2) + 2 
    (1+\delta)(\diam(\M)/\eta + \Mtt) + 4d \eqsp . 
    \end{align}
  Then, we have for any $k \in \{0, \dots, K\}$
  \begin{equation}
    \label{eq:Ktt_def}
      \expeLigne{\normLigne{Y_k}^2} \leq \Ktt = d + B(\delta, \Mtt, \eta, \diam(\M))(1/A(\delta, \Mtt, \eta, \diam(\M)) + \delta) \eqsp .
    \end{equation}
    In particular if $\Mtt \leq 1/32$ and $\delta \leq 1/32$ then for any $k \in \{0, \dots, K\}$
    \begin{equation}
      \expeLigne{\normLigne{Y_k}^2} \leq \Ktt_0 = 5d + 320 (1+ \diam(\M))^2 \eqsp . 
    \end{equation}
  \end{lemma}

  \begin{proof}
    Recall that using \eqref{eq:discretization_improved}, we have that for any $k \in \{0, \dots, K-1\}$
    \begin{equation}
      \label{eq:discretization_improved_deet_linf}
    \textstyle{
      Y_{k+1} = Y_k + (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1) (Y_{k} + 2 \bm{s}(T-t_k, Y_{k})) + (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)^{1/2} Z_k \eqsp ,
      }
    \end{equation}
    For simplicity, we denote
    \begin{equation}
      \textstyle{ \gamma_{1,k} = (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)/\beta_{T-t_k} \eqsp , \qquad \gamma_{2,k} = (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)/(2\beta_{T-t_k}) \eqsp . }
    \end{equation}
    Then, \eqref{eq:discretization_improved_deet_linf} can be rewritten for any $k \in \{0, \dots, K-1\}$ as
    \begin{equation}
      \label{eq:discretization_improved_deet_duo_linf}
          \textstyle{
      Y_{k+1} = Y_k + \gamma_{1,k} \beta_{T-t_k} (Y_{k} + 2 \bm{s}(T-t_k, Y_{k})) + \sqrt{2 \gamma_{2,k} \beta_{T-t_k}} Z_k \eqsp .
      }
    \end{equation}
    In what follows, we denote $\bar{\gamma}_{1,k} = \gamma_{1,k} \beta_{T-t_k}$
    and $\bar{\gamma}_{2,k} = \gamma_{2,k} \beta_{T-t_k}$. In addition, using
    that $\gamma_k \beta_{T-t_k} \leq \delta \leq 1/4$, we have that
    $\gamma_{1,k} \leq \gamma_{2,k} \leq 2 \gamma_{1,k}$.
    Indeed, we have that for any $k \in \{0, \dots, K-1\}$
    \begin{align}
      &\textstyle{\gamma_{2,k} / \gamma_{1,k} = (1/2) (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] + 1) \geq 1 \eqsp ,} \\ 
        &\textstyle{\gamma_{2,k} / \gamma_{1,k} = (1/2) (\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] + 1) \leq (1/2)(\exp[\gamma_k \beta_{T-t_k}] + 1) \leq 2 \eqsp ,}
    \end{align}
    Using \Cref{lemma:control_grad}, we have that for any $t \in \ccint{0,T}$,
    $x_t \in \rset^d$ and $\eta >0$
    \begin{align}
      \langle x_t, \bm{s}(t, x_t) \rangle &\leq -\normLigne{x_t}^2/\sigma_t^2 + m_t \diam(\M)\normLigne{x_t}/\sigma_t^2 + \Mtt (1 + \normLigne{x_t})\normLigne{x_t} /\sigma_t^2  \\
      &\leq (-1 + 2 \Mtt + \eta  m_t \diam(\M))\norm{x_t}^2/\sigma_t^2 + (m_t \diam(\M)/\eta + \Mtt) / \sigma_t^2 \eqsp , \label{eq:s_scalar_product_linf}
    \end{align}
    where we have used that for any $a,b \geq 0$, $2ab \leq \eta a^2 + b^2/\eta$
    in the last line.  In addition, using \Cref{lemma:control_grad}, for any
    $t \in \ccint{0,T}$ and $x_t \in \rset^d$ we have
    \begin{align}      
      \normLigne{\bm{s}(t, x_t)}^2 &\leq 2 \normLigne{\bm{s}(t, x_t) - \nabla \log p_t(x_t)}^2 + 2 \normLigne{\nabla \log p_t(x_t)}^2 \\
                                   &\leq 4\Mtt^2(1 + \normLigne{x_t}^2)/\sigma_t^4 + 4 \normLigne{x_t}^2/\sigma_t^4 + 4 m_t^2 \diam(\M)^2/\sigma_t^4 \\
      &\leq 4(1 + \Mtt^2)\normLigne{x_t}^2/\sigma_t^4 + 4(\Mtt^2 + m_t^2 \diam(\M)^2 ) / \sigma_t^4 \eqsp .  \label{eq:s_norm_control_linf}
    \end{align}
    Combining \eqref{eq:discretization_improved_deet_duo_linf},
    \eqref{eq:s_scalar_product_linf} and \eqref{eq:s_norm_control_linf} we have for any
    $k \in \{0, \dots, K-1\}$
    \begin{align}
      \expeLigne{\normLigne{Y_{k+1}}^2} &= (1 + \bar{\gamma}_{1,k})^2 \expeLigne{\normLigne{Y_{k}}^2} + 4 \bar{\gamma}_{1,k}^2 \expeLigne{\normLigne{\bm{s}(T-t_k, Y_k)}^2} \\
      & \qquad +4 \bar{\gamma}_{1,k} (1 + \bar{\gamma}_{1,k}) \expeLigne{\langle Y_k, \bm{s}(T-t_k, Y_k)\rangle} + 2\bar{\gamma}_{2,k}d \\
                                        &\leq (1 + 2\bar{\gamma}_{1,k} + \bar{\gamma}_{1,k}^2) \expeLigne{\normLigne{Y_k}^2} + 16 (\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
                                        & \qquad + 16(\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (\Mtt^2 + m_{T-t_k}^2 \diam(\M)^2 ) \\
      &\qquad + 4 \bar{\gamma}_{1,k} (1 + \bar{\gamma}_{1,k}) \expeLigne{\langle Y_k, \bm{s}(T-t_k, Y_k)\rangle} + 4\bar{\gamma}_{1,k}d\\
                                        &\leq (1 + 2\bar{\gamma}_{1,k} + \bar{\gamma}_{1,k}^2) \expeLigne{\normLigne{Y_k}^2} + 16 (\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
                                        & \qquad + 16(\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (\Mtt^2 + m_{T-t_k}^2 \diam(\M)^2 ) \\
      & \qquad + 4 (\bar{\gamma}_{1,k}/\sigma_{T-t_k}^2) (1 + \bar{\gamma}_{1,k}) (-1 + 2 \Mtt + \eta m_{T-t_k} \diam(\M))\expeLigne{\norm{Y_k}^2} \\
                                        & \qquad + (\bar{\gamma}_{1,k}/ \sigma_{T-t_k}^2 ) (1 + \bar{\gamma}_{1,k}) (m_{T-t_k} \diam(\M)/\eta + \Mtt) + 4 \bar{\gamma}_{1,k} d \eqsp . 
      %                                   &\leq (1 + 2\bar{\gamma}_{1,k} + \bar{\gamma}_{1,k}^2) \expeLigne{\normLigne{Y_k}^2} + 16 (\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
      %                                   & \qquad + 4(\bar{\gamma}_{1,k} / \sigma_{T-t_k}^2)^2 (\Mtt^2 + m_{T-t_k}^2 \diam(\M)^2 ) \\
      % & \qquad + 4 (\bar{\gamma}_{1,k}/\sigma_{T-t_k}^2) (1 + \bar{\gamma}_{1,k}) (-1 + 2 \Mtt + \vareps m_{T-t_k} \diam(\M))\expeLigne{\norm{Y_k}^2} \\
      % & \qquad + 2 (\bar{\gamma}_{1,k}/ \sigma_{T-t_k}^2 ) (1 + \bar{\gamma}_{1,k}) (m_{T-t_k} \diam(\M)/\vareps + \Mtt) + 4 \bar{\gamma}_{1,k} \eqsp . 
    \end{align}
    In what follows, we let 
    $\delta_k = \bar{\gamma}_{1,k} /
    \sigma_{T-t_k}^2$. Using
    that for any
    $t \in \ccint{0,T}$,
    $m_t, \sigma_t \in \ccint{0,1}$
    we have
    \begin{align}
      \expeLigne{\normLigne{Y_{k+1}}^2} & \leq (1 + 2\delta_k + \delta_k^2) \expeLigne{\normLigne{Y_k}^2} + 16 \delta_k^2 (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
                                        & \qquad + 16\delta_k^2 (\Mtt^2 + \diam(\M)^2 ) \\
      & \qquad + 4 \delta_k (1 + \delta_k) (-1 + 2 \Mtt +\eta \diam(\M))\expeLigne{\norm{Y_k}^2} \\
      & \qquad +  \delta_k (1 + \delta_k) (\diam(\M)/\eta + \Mtt) + 4 \delta_k d
    \end{align}
    Since $s \mapsto \beta_s$ is non-decreasing, that
    $\beta_{T-t_k} \gamma_k \leq  \delta \leq 1/4$ and that for any
    $w \in \ccint{0,1/2}$, $\rme^{w} -1 \leq 1 + 2 w$, we have 
    \begin{equation}
      \textstyle{ \exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1 \leq \exp[\beta_{T-t_k} \gamma_k] - 1 \leq 2 \beta_{T-t_k} \gamma_k \eqsp . }
    \end{equation}
    Therefore, we get that
    $\delta_k \leq 2 \gamma_k \beta_{T-t_k} /\sigma_{T-t_k}^2 \leq 2 \delta$.
    Since $\delta_k \leq 2\delta$ we have
    \begin{align}
      \expeLigne{\normLigne{Y_{k+1}}^2} & \leq (1 + 2\delta_k +2 \delta_k \delta) \expeLigne{\normLigne{Y_k}^2} + 32 \delta_k \delta (1 + \Mtt^2)\expeLigne{\normLigne{Y_k}^2}  \\
                                        & \qquad + 4 \delta_k  (-1 + 2 \Mtt + \eta \diam(\M))\expeLigne{\norm{Y_k}^2} \\
                                        & \qquad + 32\delta_k \delta (\Mtt^2 + \diam(\M)^2 ) \\      
                                        & \qquad + 2\delta_k (1 + \delta) (\diam(\M)/\eta  + \Mtt) + 4 \delta_k d \eqsp .
    \end{align}
    Hence, we have that
    \begin{align}
      \expeLigne{\normLigne{Y_{k+1}}^2} &\leq (1 + \delta_k[-2 + 2\delta + 32 \delta (1 + \Mtt^2) + 8 \Mtt + 4\eta \diam(\M)]) \expeLigne{\normLigne{Y_k}^2} \\
      & \qquad + \delta_k [32\delta (\Mtt^2 + \diam(\M)^2) + 2(1+\delta)(\diam(\M)/\eta + \Mtt) + 4 d] \eqsp . 
    \end{align}
    Denote
    $A = 2 - 2\delta - 32 \delta (1
    + \Mtt^2) - 8 \Mtt -
    4\eta \diam(\M)$, 
    $B = 32\delta (\Mtt^2 +
    \diam(\M)^2) + 2 
    (1+\delta)(\diam(\M)/\eta + \Mtt) + 4d$. Then, we have
    \begin{equation}
      \expeLigne{\normLigne{Y_{k+1}}^2} \leq (1 - \delta_k A) \expeLigne{\normLigne{Y_k}^2} + \delta_k B \eqsp . 
    \end{equation}
    Hence, if
    $\expeLigne{\normLigne{Y_k}^2}
    \geq B / A$ we have that
    $\expeLigne{\normLigne{Y_{k+1}}^2}
    \leq
    \expeLigne{\normLigne{Y_{k}}^2}$. In
    addition, if
    $\expeLigne{\normLigne{Y_k}^2}
    \leq B / A$ then,
    $\expeLigne{\normLigne{Y_{k+1}}^2}
    \leq B/A + \delta B$. Therefore,
    we conclude by recursion that for any $k \in \{0, \dots, K\}$
    \begin{equation}
      \expeLigne{\normLigne{Y_k}^2} \leq d + B(1/A + \delta) \eqsp ,
    \end{equation}
    which concludes the first part of the proof. If $\delta, \Mtt \leq 1/32$
    then, $A(\delta, \Mtt, \eta, \diam(\M)) \geq 1/2 - 4 \eta \diam(\M)$. We
    conclude upon setting $\eta = 1/(16\diam(\M))$. In that case
    $A(\delta, \Mtt, \eta, \diam(\M)) \geq 1/4$ and
    \begin{align}
      B(\delta, \Mtt, \eta, \diam(\M)) &\leq 32\delta (\Mtt^2 +
    \diam(\M)^2) + 2 
                                         (1+\delta)(16\diam(\M) + \Mtt) + 4d \\
      &\leq 64(1 + \diam(\M) + \diam(\M)^2)+ 4d \eqsp ,
    \end{align}
    which concludes the proof.
  \end{proof}

  Note that the same result holds for $(\bbfY_t)_{t \in \ccint{0,t_K}}$.
  
  \begin{lemma}
    \label{lemma:lipschitz-behavior}
    Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta} and
    \rref{assum:score_control}. In addition, assume that for any
    $k \in \{0, \dots, K-1\}$,
    $\gamma_k \beta_{T-t_k} / \sigma_{T-t_k}^2 \leq \delta \leq 1/4$. Then, we
    have for any $k \in \{0, \dots, K-1\}$ and $t \in \ccint{t_k, t_{k+1}}$
    \begin{equation}
      \expeLigne{\normLigne{\bbfY_t - \bbfY_{t_k}}^2}
      \leq \Ltt \beta_{T-t_k} \gamma_k \eqsp ,
    \end{equation}
    with $\Ltt = 8 (1 + \delta) ( 16 (5 + \Mtt^2) \Ktt + 16 (4\diam(\M)^2 + \Mtt^2)) + 4$ and
    where $\Ktt$ is defined in \eqref{eq:Ktt_def}. In particular if $\Mtt \leq 1/32$ and $\delta \leq 1/32$
    \begin{equation}
      \expeLigne{\normLigne{\bbfY_t - \bbfY_{t_k}}^2} \leq \Ltt_0 \beta_{T-t_k} \gamma_k 
      = (64 d + 20544 (1 + \diam(\M))^2) \beta_{T-t_k} \gamma_k \eqsp .
    \end{equation}    
  \end{lemma}
  \begin{proof}
    Recall that
    \begin{equation}
  \textstyle{
    \bbfY_t = \bbfY_{t_k} + (\exp[\int_{T-t}^{T-t_k} \beta_s \rmd s] - 1) (\bbfY_{t_k} + 2 \bm{s}(T-t_k, \bbfY_{t_k})) + (\exp[2 \int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)^{1/2} Z \eqsp ,
    }
  \end{equation}
    where $Z$ is a Gaussian random variable with zero mean and identity covariance
    and the equality holds in distribution independent from $\bbfY_{t_k}$.
    Therefore, we get that
    \begin{align}
      \expeLigne{\normLigne{\bbfY_t - \bbfY_{t_k}}^2} &= 2\textstyle{(\exp[\int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)^2 (\expeLigne{\normLigne{\bbfY_{t_k}}^2} + 4 \expeLigne{\normLigne{\bm{s}(T-t_k, \bbfY_{t_k})}^2})} \\
      & \qquad \textstyle{+ (\exp[2 \int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)d \eqsp . \label{eq:easy_integration}}
    \end{align}
    In addition, using \Cref{assum:score_control}, \Cref{lemma:control_grad} and
    that for any $t \in \ccint{0,T}$, $m_t \in \ccint{0,1}$, we get that for any
    $u \in \ccint{0,T}$ and $x_u \in \rset^d$
    \begin{align}
      \normLigne{\bm{s}(u, x_u)} &\leq \Mtt(1 + \normLigne{x_u})/\sigma_u^2 + 2 \normLigne{x_u}/\sigma_u^2 + 2 \diam(\M)/\sigma_u^2 \\
      &\leq (1/\sigma_u^2)\{ (\Mtt + 2) \norm{x_u} + (\Mtt + 2 \diam(\M)) \} \eqsp .
    \end{align}
    Combining this result and \eqref{eq:easy_integration}, we get that
    \begin{align}
      \expeLigne{\normLigne{\bbfY_t - \bbfY_{t_k}}^2} &= 2\textstyle{(\exp[\int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)^2 (\expeLigne{\normLigne{\bbfY_{t_k}}^2} } \\
      & \qquad \textstyle{+ 4 \expeLigne{\normLigne{\bm{s}(T-t_k, \bbfY_{t_k})}^2}) + (\exp[2 \int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)d} \\
                                                      &\leq 2\textstyle{(\exp[\int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)^2} \expeLigne{\normLigne{\bbfY_{t_k}}^2 } \\
      & \qquad + 32 (4 + \Mtt^2) \textstyle{(\exp[\int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)^2} \expeLigne{\normLigne{\bbfY_{t_k}}^2}/\sigma_{T-t_k}^2 \\
      & \qquad  + 32 \textstyle{(\exp[\int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)^2} (4\diam(\M)^2 + \Mtt^2)/\sigma_{T-t_k}^2 \\
      & \qquad \textstyle{+ (\exp[2 \int_{T-t}^{T-t_k} \beta_s \rmd s] - 1)d} \eqsp . \label{eq:inter_bound_exp_time}
    \end{align}
    Since $s \mapsto \beta_s$ is non-decreasing, that
    $\beta_{T-t_k} \gamma_k \leq \delta \leq 1/4$ and that for any
    $w \in \ccint{0,1/2}$, $\rme^{2 w} -1 \leq 1 + 4 w$, we have for any $\alpha \in \{1,2\}$
    \begin{equation}
      \textstyle{ \exp[\alpha \int_{T-t}^{T-t_k} \beta_s \rmd s] - 1 \leq \exp[\alpha \beta_{T-t_k} \gamma_k] - 1 \leq 2 \alpha \beta_{T-t_k} \gamma_k \eqsp . }
    \end{equation}
    Combining this result and \eqref{eq:inter_bound_exp_time}, we get that
    \begin{align}
      \expeLigne{\normLigne{\bbfY_t - \bbfY_{t_k}}^2}  &\leq 8 \beta_{T-t_k}^2 \gamma_k^2 \expeLigne{\normLigne{\bbfY_{t_k}}^2 + 32 (4 + \Mtt^2) \normLigne{\bbfY_{t_k}}^2/\sigma_{T-t_k}^2 + 32 (4\diam(\M)^2 + \Mtt^2)/\sigma_{T-t_k}^2} \\
                                                       & \qquad + 4 \beta_{T-t_k} \gamma_k d \label{eq:inter_bound_exp_time} \\
                                                       &\leq 8 (\beta_{T-t_k}^2 \gamma_k^2/\sigma_{T-t_k}^2) ( 32 (5 + \Mtt^2) \expeLigne{\normLigne{\bbfY_{t_k}}^2} + 32 (4\diam(\M)^2 + \Mtt^2))  + 4 \beta_{T-t_k} \gamma_k d \eqsp .      
    \end{align}
    Therefore, using \Cref{lemma:control_growth_discrete_process} and \eqref{eq:Ktt_def}, we get that
    \begin{align}
      \expeLigne{\normLigne{\bbfY_t - \bbfY_{t_k}}^2} &\leq 8 (\beta_{T-t_k}^2 \gamma_k^2/\sigma_{T-t_k}^2) ( 32 (5 + \Mtt^2) \Ktt + 32 (4\diam(\M)^2 + \Mtt^2))  + 4 \beta_{T-t_k} \gamma_k d\\
      &\leq \{ 256 \delta ( (5 + \Mtt^2) \Ktt + 4\diam(\M)^2 + \Mtt^2)  + 4d\} \beta_{T-t_k}  \gamma_k 
    \end{align}
    which concludes the first part of the proof. Now assuming that $\delta, \Mtt \leq 1/32$ we have
    \begin{align}
      \expeLigne{\normLigne{\bbfY_t - \bbfY_{t_k}}^2} &\leq (64 \Ktt + 64 \diam(\M)^2 + 16d)\beta_{T-t_k} \gamma_k \\
      &\leq 64 d + 20544 (1 + \diam(\M))^2 \eqsp ,
    \end{align}
    which concludes the proof.
  \end{proof}

  \subsection{Control of the tangent backward process}
  \label{sec:contr-tang-backw}

We now introduce the tangent process associated with
$(\bfY_t)_{t \in \ccint{0,T}}$. We have
\begin{equation}
  \label{eq:stochastic_flow}
  \rmd \nabla \bfY_t = \beta_{T-t} (\Id + 2 \nabla^2 \log p_{T-t}(\bfY_t))\nabla \bfY_t \rmd t \eqsp , \qquad \nabla \bfY_0 = \Id \eqsp . 
\end{equation}
We recall that controlling the tangent process allows to control the Wasserstein
distance between the original process and its target measure. Indeed, let
$(\bfY_t^x)_{t\in\ccint{0,T}}$ and $(\bfY_t^y)_{t\in\ccint{0,T}}$ be the
processes given by \eqref{eq:continuous_exact_app} with initial condition $x$ and
$y$ respectively.  Then we have that for any $t \in \ccint{0,T}$
\begin{equation}
  \label{eq:pro_wasserstein}
  \textstyle{
    \normLigne{\bfY_t^x - \bfY_t^y} \leq \int_0^1 \normLigne{\nabla \bfY_t^{z_\lambda}} \rmd \lambda \normLigne{x-y} \eqsp ,
    }
\end{equation}
where $(\nabla \bfY_t^x)_{t \in \ccint{0,T}}$ is the tangent process given by
\eqref{eq:stochastic_flow} and associated with
$(\bfY_t^{z_\lambda})_{t\in \ccint{0,T}}$, where
$z_\lambda = \lambda x+(1-\lambda)y$. Before providing controls in the general
setting, we take a detour and focus on the case where $\diam(\M) = 0$, \ie
$\pi = \updelta_0$. In the following proposition, we show that in this case the
backward process converges in finite-time. This highlights the role of the
diameter of the manifold in the subsequent analysis.

\begin{proposition}
  \label{prop:convergence_dirac_zero}
  Assume \rref{assum:manifold_hyp} and that $\diam(\M) = 0$, \ie
  $\pi = \updelta_0$. Then, we have that for any $x,y \in \rset^d$ and
  $t \in \ccint{0,T}$
  \begin{equation}
    \wassersteinD[1](\updelta_x \Qker_t, \updelta_y \Qker_y) \leq \textstyle{ 2\exp[(1/2)\int_{T-t}^T \beta_{s} \rmd s] (\exp[2\int_0^{T} \beta_s \rmd s] -1)^{-1/2} (\exp[2\int_0^{T-t} \beta_s \rmd s] -1)^{1/2} \norm{x-y} } \eqsp . 
  \end{equation}
  In particular, we have that for any $x \in \rset^d$,
  $\updelta_x \Qker_T = \pi$, \ie the backward diffusion converges in finite
  time no matter the initialization distribution.
\end{proposition}

\begin{proof}
  Let $t \in \ccint{0,T}$. Using \Cref{lemma:control_hessian}, we have that for
  any $\mathrm{M} \in \mathcal{M}_d(\rset)$
  \begin{equation}
    \langle \mathrm{M}, \nabla^2 \log q_t(x_t) \mathrm{M} \rangle \leq - \sigma_t^{-2} \normLigne{\mathrm{M}}^2 \eqsp .
  \end{equation}
  In particular, we have that for
  any $\mathrm{M} \in \mathcal{M}_d(\rset)$
  \begin{equation}
    \label{eq:inequality_M}
   \beta_{T-t} \langle \mathrm{M}, \Id + 2 \nabla^2 \log q_{T-t}(x_t) \mathrm{M} \rangle \leq (\beta_{T-t} - 2 \beta_{T-t} \sigma_{T-t}^{-2}) \normLigne{\mathrm{M}}^2 \eqsp . 
 \end{equation}
 Using \Cref{lemma:integration_lemma}, we have
 \begin{align}
   &\textstyle{\int_0^t (\beta_{T-s} - 2 \beta_{T-s} \sigma_{T-s}^{-2}) \rmd s} \\
   & \qquad \textstyle{= \int_0^t \beta_{T-s} \rmd s + \log(\exp[2\int_0^{T-t} \beta_s \rmd s] -1) - \log(\exp[2\int_0^{T} \beta_s \rmd s] -1) } \\
   & \qquad \textstyle{= \int_{T-t}^T \beta_{s} \rmd s + \log(\exp[2\int_0^{T-t} \beta_s \rmd s] -1) - \log(\exp[2\int_0^{T} \beta_s \rmd s] -1) \eqsp . }     
 \end{align}
 Finally, we have that
 \begin{align}
   &\textstyle{\exp[\int_0^t (\beta_{T-s} - 2 \beta_{T-s} \sigma_{T-s}^{-2}) \rmd s]} \\
   & \qquad \leq \textstyle{ \exp[\int_{T-t}^T \beta_{s} \rmd s] (\exp[2\int_0^{T} \beta_s \rmd s] -1)^{-1} (\exp[2\int_0^{T-t} \beta_s \rmd s] -1) \eqsp . }
 \end{align}
 Hence, using this result, \eqref{eq:stochastic_flow} and \eqref{eq:inequality_M}, we get that
 \begin{equation}
  (1/2) \normLigne{\nabla \bfY_t}^2 \leq \textstyle{ \exp[\int_{T-t}^T \beta_{s} \rmd s] (\exp[2\int_0^{T} \beta_s \rmd s] -1)^{-1} (\exp[2\int_0^{T-t} \beta_s \rmd s] -1) \eqsp , }
 \end{equation}
 which concludes the first part of the proof, using
 \eqref{eq:pro_wasserstein}. For the second part of the proof, we first remark
 that for any $x, y \in \rset^d$,
 $\wassersteinD[1](\updelta_x \Qker_T, \updelta_y \Qker_T) = 0$. Therefore, for
 any probability measures $\mu, \nu$ such that
 $\int_{\rset^d} \normLigne{x} \rmd \mu(x) <+\infty$ and
 $\int_{\rset^d} \normLigne{x} \rmd \nu(x) <+\infty$, we have
 $\wassersteinD[1](\mu \Qker_T, \nu \Qker_T) = 0$ We conclude upon combining
 this result and that $(\updelta_x \Pker_T) \Qker_T = \updelta_x$.
\end{proof}

Note that it is also possible to explicitly write down the backward stochastic
process in this case since $\nabla \log p_t$ is available in close form. One can
remark that in this case we recover an Ornstein-Ulhenbeck bridge.

In the case where the diameter is non-zero, we cannot recover such a
contraction. However, it is possible to obtain a contraction up to a certain
point.  The following lemma will allow us to control the growth of the tangent
process.
\begin{lemma}
  \label{lemma:growth_tangent_process}
  Assume \rref{assum:assumption_beta} and that
  $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$. Let $t^\star \in \ccint{0,T}$
  given by
  \begin{equation}
    t^\star = T - 2\bar{\beta}(1 + \log(1+\diam(\M)) \eqsp . 
  \end{equation}
  Then, for any $t \in \ccint{0,t^\star}$ we have
  \begin{equation}
\textstyle{    \int_0^{t}\beta_{T-s} (1 -2/\sigma_{T-s}^2 + m_{T-s}^2\diam(\M)^2/\sigma_{T-s}^4) \rmd s  \leq -(1/2) \int_0^{t} \beta_{T-t} \rmd s  \eqsp . }
  \end{equation}
  In addition, for any $t \in \ccint{t^\star,T}$
  \begin{equation}
    \textstyle{    \int_{t^\star}^{t}\beta_{T-s} (1 -2/\sigma_{T-s}^2 + m_{T-s}^2\diam(\M)^2/\sigma_{T-s}^4) \rmd s}  \leq (\diam(\M)^2/2)(\sigma_{T-t}^{-2} - \sigma_{T-t^\star}^{-2}) \eqsp . 
  \end{equation}
\end{lemma}

\begin{proof}
  Let $s \in \ccint{0,T}$. Note that we have
  \begin{equation}
    \label{eq:upper_bound_neg}
    1 - 2/\sigma_{T-s}^2 + m_{T-s}^2 \diam(\M)^2/\sigma_{T-s}^4 \leq -1/2 \eqsp , 
  \end{equation}
  if and only if
  \begin{equation}
    3 \sigma_{T-t}^4 -4\sigma_{T-s}^2 + 2m_{T-s}^2 \diam(\M)^2 \leq 0 \eqsp . 
  \end{equation}
  Hence, using this result and the fact that $\sigma_{T-s}^2 = 1 - m_{T-s}^2$ we
  have that \eqref{eq:upper_bound_neg} is satisfied if and only if
  \begin{equation}
    3 m_{T-s}^4 +2 (\diam(\M)^2 - 1) m_{T-s}^2 -1 \leq 0 \eqsp . 
  \end{equation}
  Introduce $P(u) = 3 u^2 + 2(\diam(\M)^2 -1)u - 1$. We have that $P(u) \leq 0$
  for $u \in \ccint{0, u_0}$ with
  \begin{equation}
    u_0 = [-(\diam(\M)^2 -1) + ((\diam(\M)^2 -1)^2 + 3)^{1/2}]/3 = (\delta + (\delta^2 +3)^{1/2})/3\eqsp ,
  \end{equation}
  where $\delta = \diam(\M)^2 -1 \in \coint{-1, +\infty}$.  If
  $\diam(\M)^2 -1 \geq 1$ then, using this result and the fact that for any
  $a \in \coint{0,+\infty}$, $(1+a)^{1/2} \geq 1 + a/2 - a^2/8$ we have
  \begin{equation}
    \label{eq:u0_lower}
    u_0 \geq \delta(-1 + (1+3/\delta^2)^{1/2})/3 \geq \delta(1/(2\delta^2) - 3/(8\delta^4)) \geq (1/2 - 3/8)/\delta \geq 1/(8\delta) \eqsp . 
  \end{equation}
  In addition, if $\delta \leq 1$ then $\delta^2 \in \ccint{0,1}$. Using this
  result and the fact that for any $a \in \ccint{0,1}$,
  $\sqrt{3 +a} \geq (2 - \sqrt{3}) a + \sqrt{3}$ we have
  \begin{align}
    u_0 &\geq (-\delta + (3 + \delta^2)^{1/2})/3 \\
    &\geq (-\absLigne{\delta} + (3 + \absLigne{\delta}^2)^{1/2})/3 \geq ((1 - \sqrt{3})\absLigne{\delta} + \sqrt{3})/3 \geq 1/3 \eqsp . 
  \end{align}
  Combining this result and \eqref{eq:u0_lower}, we get that
  \begin{equation}
    u_0 \geq 1/(8(1 + \absLigne{\delta})) \eqsp . 
  \end{equation}
  Therefore, we get that for any $t \in \ccint{0,T}$ such that
  $m_{T-t}^2 \leq 1/(8(1 + \absLigne{\delta}))$
  \begin{equation}
    1 - 2/\sigma_{T-s}^2 + m_{T-s}^2 \diam(\M)^2/\sigma_{T-s}^4 \leq -1/2 \eqsp . 
  \end{equation}
  Hence, for any $t \in \ccint{0,T}$ such that
  $\exp[-2(T-t)/\bar{\beta}] \leq 1/(8(1 + \absLigne{\delta}))$
  \begin{equation}
    1 - 2/\sigma_{T-s}^2 + m_{T-s}^2 \diam(\M)^2/\sigma_{T-s}^4 \leq -1/2 \eqsp . 
  \end{equation}
  Let $t^\star_0$ such that
  $\exp[-2(T-t_0^\star)/\bar{\beta}] = 1/(8(1 + \absLigne{\delta}))$.
  We get that
  \begin{equation}
    t_0^\star = T - (\bar{\beta}/2)\log(8(1 + \absLigne{\delta})) \eqsp . 
  \end{equation}
  Using that for any $a \geq 0$, $1 + \absLigne{a^2 -1} \leq 2 (1 +a)^2$ and
  that $\log(16) \leq 4$, we get that
  \begin{equation}
    t_0^\star \geq T - (\bar{\beta}/2)(\log(16(1+\diam(\M))^2)) \geq t^\star = T - 2\bar{\beta}(1 + \log(1+\diam(\M))) \eqsp . 
  \end{equation}
  Hence, since $t \mapsto m_{T-t}$ is non-decreasing, we get that for any $t \in \ccint{0, t^\star}$, $m_{T-t} \leq 1/(8(1+\absLigne{\delta}))$ and therefore
    \begin{equation}
    1 - 2/\sigma_{T-s}^2 + m_{T-s}^2 \diam(\M)^2/\sigma_{T-s}^4 \leq -1/2 \eqsp ,
  \end{equation}
  which concludes the first part of the proof. The second part of the proof
  follows from \Cref{lemma:integration_lemma} and
  \begin{align}
    &\textstyle{    \int_{t^\star}^{t}\beta_{T-s} (1 -2/\sigma_{T-s}^2 + m_{T-s}^2\diam(\M)^2/\sigma_{T-s}^4) \rmd s}  \\
    & \qquad \leq \textstyle{ (\diam(\M)^2/2)[(1-\exp[-2\int_0^{T-t} \beta_s \rmd s])^{-1} - (1-\exp[-2\int_0^{T-t^\star} \beta_s \rmd s])^{-1}]  } \\
    & \qquad \leq (\diam(\M)^2/2)(\sigma_{T-t}^{-2} - \sigma_{T-t^\star}^{-2}) \eqsp ,
  \end{align}
  which concludes the proof.
\end{proof}

The control of the tangent process in the case where $\diam(\M) > 0$ is given in
\Cref{prop:control_gradient}.

  \begin{proposition}
    \label{prop:wasserstein_forward}
    Assume \rref{assum:manifold_hyp} and
    $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$. Then, for any
    $x, y \in \rset^d$ and $t \in \ccint{0,t_K}$
  \begin{equation}
    \textstyle{
      \wassersteinD[1](\updelta_x \Qker_{t}, \updelta_y \Qker_{t}) \leq  \exp[(\diam(\M)^2/2)\sigma_{T-t_K}^{-2}] \normLigne{x-y} \eqsp .
      }
    \end{equation}    
  \end{proposition}

  \begin{proof}
    This is a direct consequence of \eqref{eq:pro_wasserstein} and \Cref{prop:control_gradient}.
  \end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we have studied the convergence of diffusion models under the
manifold hypothesis and provided convergence guarantees w.r.t. the Wasserstein
distance of order one. Our theoretical results show that diffusion models are
able to recover target distributions defined on low-dimensional manifolds.
% One limitation of our current analysis resides in the error bound on the score
% which, while being more realistic than the uniform bound assumed in
% \cite{debortoli2021diffusion}, weaker conditions (like $\mathrm{L}^2$ bounds)
% are desirable. One possible avenue to bridge that gap is to rely on the
% framework introduce by \cite{lee2022convergence} to transfer $\mathrm{L}^2$
% bounds to uniform bounds.
% Another open question is to quantify the effect of the
% sample size when training the score and the associated error bounds.


These results can be extended in several directions. First, in this work we
focused on the Ornstein-Ulhenbeck process as a forward noising process. It would
be interesting to analyze other forward diffusions such as the critically-damped
one \citep{dockhorn2021score}. Another extension would be to study other
discretization frameworks such as predictor-corrector schemes
\citep{durkan2021maximum} and to extend our analysis to more realistic
statistical settings. Finally, it is a challenge to derive similar bounds for
target distributions with $\rset^d$ support and tail constraints.  From a
methodological point of view, we would like to analyze the convergence of
diffusion models defined in latent spaces, see \citep{vahdat2021score,cohen2022vqvae} for
instance, and characterize the dependency of the obtained bounds \wrt the latent
space dimension. Indeed, defining diffusion processes in latent spaces might
allow us to bypass some limitations of the manifold hypothesis. In particular,
by carefully choosing the latent space, it might be possible to alleviate the
score explosion at time $t \to 0$.

Finally, we would like to deepen our study of the relationship between the
geometry of the manifold $\M$ and the properties of the score
function. Preliminary results from \Cref{sec:non-conv-count} indicate that the
convexity of $\M$ can be recovered from the properties of the score but it
remains unclear if more can be said on the geometry of the manifold.



% \begin{itemize}
% \item Extension to discrete space ?
% \item Extension to Riemanian ?
% \item Extension to other diffusions ? --> avantage OU = kernel maybe critically damped 
% \item Extension to subgaussian targets ?
% \item Erreur L2 au lieu de Linfini
% \item Finally we note that our study could be extended to cover over discretization scheme   
% \end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/def.tex <==
\def\eps{\epsilon}
\def\erfc{\mathrm{erfc}}
\def\Vol{\mathrm{Vol}}
\def\softmin{\mathrm{softmin}}

\def\Ctt{\mathtt{C}}
\def\Dtt{\mathtt{D}}

\def\drifta{b^{(a)}}
\def\driftb{b^{(b)}}
\def\driftc{b^{(c)}}
\def\driftd{b^{(d)}}

\def\Deltaab{\Delta^{(a,b)} b}
\def\Deltabc{\Delta^{(b,c)} b}   
\def\Deltacd{\Delta^{(c,d)} b}   

\def\EM{\mathrm{EM}}
\def\volat{a}
\def\Cdeux{C_2}
\def\Ctrois{C_3}

\newcommand{\pdata}{p_{\mathrm{data}}}
\newcommand{\pref}{p_{\mathrm{ref}}}
\newcommand{\grad}{\mathrm{grad}}
\newcommand{\dive}{\mathrm{div}}

\newcommand{\bsde}[1]{\mathrm{BSDE}(#1)}
\newcommand{\pidata}{\pi_{\mathrm{data}}}
\newcommand{\pinoisy}{\pi_{\mathrm{noisy}}}
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\mail}[1]{\footnote{Email: \href{mailto:#1}{\textcolor{black}{#1}}}}
\newcommand{\schro}{Schr\"{o}dinger\xspace}
\newcommand{\Cweakapp}{\ttd}
\def\ttfp{\Cweakapp_{p}}
\def\ttfpun{\Cweakapp_{p,1}}
\def\ttfpdeux{\Cweakapp_{p,2}}
\def\ttfptrois{\Cweakapp_{p,3}}
\def\ttfpquatre{\Cweakapp_{p,4}}
\def\ttamin{\mathtt{a}}
\def\ttfun{\Cweakapp_4}
\def\ttfdeux{\Cweakapp_5}
\def\btta{\bar{\mathtt{A}}}
\def\bfb{\mathbf{b}}
\def\bfsigma{\pmb{\sigma}}
\def\KuLo{Kurdyka-\L ojasiewicz}
\def\Tnplusun{\mathcal{T}_{k+1}}
\def\contspace{\mathcal{C}}
\newcommand{\tta}{\mathtt{A}}
\newcommand{\ttb}{\mathtt{B}}
\newcommand{\ttc}{\mathtt{C}}
\newcommand{\ttd}{\mathtt{D}}
\def\tte{\mathtt{E}}
\newcommand{\ttM}{\mathtt{M}}
\def\boundLSig{\Lip\eta}

\newcommand{\Capprox}{\tta}
\newcommand{\Ctech}{\ttc}
\newcommand{\Cstrong}{\ttb}
\newcommand{\Cconv}{\ttc}
\newcommand{\Cweak}{C}

\def\conj{\varkappa}
\def\mtta{\mathtt{a}}
\def\explog{\vareps}
\newcommand{\note}[1]{\textcolor{red}{#1}}
\def\Cbeta{\Cweak_{\beta, \explog}}
\def\Aar{\Capprox_{\alpha, r}}
\def\xo{x_0}
\def\Db{\Ctech}
\def\intk{\int_{k\gua}^{(k+1)\gua}}
\newcommandx\ctun[1][1=T]{\Capprox_{#1,1}}
\def\btun{\mathtt{B}_1}
\def\btdeux{\mathtt{B}_2}
\def\dtun{\mathtt{D}_1}
\def\cttun{\tilde{\Capprox}_{T,1}}
\def\dtdeux{\mathtt{D}_2}
\def\ctdeux{\Capprox_{T,2}}
\def\cttrois{\Capprox_{T,3}}
\def\ctquatre{\Capprox_{T,4}}
\def\ctcinq{\Capprox_{T,5}}
\def\ctsix{\Capprox_{T,6}}
\def\ctsept{\Capprox_{T,7}}
\def\cthuit{\Capprox_{T,8}}
\def\ctneuf{\Capprox_{T,9}}
\def\gfun{\mathbb{G}}
\def\hash{\sharp}
\def\Cconvcontun{\Cconv_{1,\alpha}^{(c)}}
\def\Cconvcontdeux{\Cconv_{2,\alpha}^{(c)}}
\def\Cconvconttrois{\Cconv_{3,\alpha}^{(c)}}
\def\Cconvdiscun{\Cconv_{1,\alpha}^{(d)}}
\def\Cconvdiscdeux{\Cconv_{2,\alpha}^{(d)}}
\def\Cconvdisctrois{\Cconv_{3,\alpha}^{(d)}}
\def\Cconvcont{\Phibf_{\alpha}^{(c)}}
\def\Cconvdisc{\Phibf_{\alpha}^{(d)}}
\def\Csham{\Cconv_1}
\def\Cshamd{\Cconv_2}
\def\Cshama{\Cconv_{\alpha}}
\def\Cshamamoins{\Cshama^-}
\def\Cshamaplus{\Cshama^+}
\def\Ccont{\Cconv^{(c)}}
\def\Cdisc{\Cconv^{(d)}}
\def\Cconvk{{\Cconv^{(a)}_k}}
%\def\Cconvdun{\Cconv^{(b)}_1}
%\def\Cconvddeux{\Cconv^{(b)}_2}
\def\Cconvdtrois{\Cconv^{(b)}}
\def\Cconvdun{(\gamma\eta/2)}
\def\Cconvddeux{(\gamma/2)}
\def\Cshamdisc{\Cconv_{0}}
\def\Cshamt{\tilde{\Cconv}_{\alpha}}
\def\Psial{\Psibf_{\alpha}}
\def\Cstrongcont{\Cstrong_1}
\def\Cstrongcontf{\Cstrong_2}
\def\Cstrongdisc{\Cstrong_3}
\def\Cstrongdiscf{\Cstrong_4}
\def\Cstrongloj{\Cstrong_5}
\def\Cstronglojdisc{\Cstrong_6}
\def\Cstrongtilde{\tilde{\Cstrong}}
\def\maxnorm{C}
\newcommand{\pinv}{^{-1}}
\newcommand{\st}{^{\star}}
\newcommand{\gb}{\gamma^{\beta}}
\newcommand{\tr}{^{\top}}
\def\scrE{\mathscr{E}}
\def\scrV{\mathscr{V}}
\def\scrF{\mathscr{F}}
\newcommand{\rref}[1]{\tup{\Cref{#1}}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\LL}{\L ojasciewicz~}
\newcommand{\gua}{\gamma_{\alpha}}
\newcommand{\bgua}{\bgamma_{\alpha}}
\newcommand{\gda}{\gua^{1/2}}
\newcommand{\tgua}{(t+\gua)^{\alpha}}
\newcommand{\guac}{c}
\newcommand{\et}{\quad\mbox{and}\quad}
%\newcommand{\sigb}{\ttM_{\Sigma}}
\newcommand{\sigb}{\eta}
\newcommand{\phe}{\varphi_{\varepsilon}}
\newcommand{\feps}{f_{\varepsilon}}
\newcommand{\nfeps}{\nabla f_{\varepsilon}}
\newcommand{\intd}{\int_{\bR^{\dim}}}
\newcommandx{\expec}[2]{{\mathbb E}\left[#1 \middle \vert #2  \right]} %%%% esperance conditionnelle
\newcommand{\expek}[1]{\expec{#1}{\cF_k}}
\newcommand{\expen}[1]{\expec{#1}{\cF_n}}
\newcommand{\nn}{_{n+1}}
\newcommand{\kk}{_{k+1}}
\newcommand{\pal}{^{\alpha}}
\newcommand{\pmal}{^{-\alpha}}
\newcommand{\cH}{\mathcal{H}}

\def\En{\tilde{E}_n}
\def\varepsn{\tilde{\vareps}_n}
\def\pow{p}
\def\ntt{\mathtt{n}_0}
\def\tlambda{\tilde{\lambda}}
\def\dim{d}
\newcommand{\tb}{\tilde{b}}
\newcommand{\Time}{T}
\newcommand{\mttun}{\mathtt{k}_1}
\newcommand{\mttdeux}{\mathtt{k}_2}
\newcommand{\mtttrois}{\mtt_3^+}
\newcommand{\bvareps}{\bar{\vareps}}
\newcommand{\transference}{\mathbf{T}}
\newcommand{\esssup}{\mathrm{ess sup}}
\newcommand{\ring}{\mathcal{C}_{\varrho}}
\newcommand{\measx}{\mathcal{X}}
\newcommand{\bkappa}{\bar{\kappa}}
\newcommand{\probaspace}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\dTVdeux}{d_{\mathrm{TV}, 2}}
\newcommand{\dTVDeux}[1]{d_{\mathrm{TV}, 2}\left( #1 \right)}
\newcommand{\bgM}{b_{\gamma, n}}
\newcommand{\bbgM}{\bar{b}_{\gamma, M}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmE}{\mathrm{E}}
\newcommand{\Fdr}{\mathrm{f}}
\newcommand{\Gdr}{\mathrm{g}}
\newcommand{\alphastar}{\alpha_{\star}}
\newcommand{\LipVset}{\mathrm{Lip}_{V, \alpha}}
\newcommand{\Lip}{\mathtt{L}}
\newcommand{\Ltt}{\mathtt{L}}
\newcommand{\Mtt}{\mathtt{M}}
\newcommand{\Ktt}{\mathtt{K}}
\newcommand{\tLip}{\tilde{\mathtt{L}}}
\newcommand{\tell}{\tilde{\ell}}
\newcommand{\Lipb}{\mtt_b}
\newcommand{\step}{\ceil{1/\gamma}}
\newcommand{\bstep}{\ceil{1/\bgamma}}
\def\bdisc{b}
\def\bfDd{\mathbf{D}_{\mathrm{d}}}
\def\bfDc{\mathbf{D}_{\mathrm{c}}}
\newcommand{\SDE}{SDE}

\newcommand{\bbeta}{\bar{\beta}}
\newcommand{\measfun}{\mathbb{F}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bdeta}{\boldsymbol{\eta}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}

%\newcommand{\tau}{\boldsymbol{\tau}}
%\newcommand{\x}{\boldsymbol{x}}
%\newcommand{\X}{\boldsymbol{X}}
%\newcommand{\y}{\boldsymbol{y}}
%%\newcommand{\u}{\boldsymbol{u}}
%\newcommand{\w}{\boldsymbol{w}}
%\newcommand{\z}{\boldsymbol{z}}
%\newcommand{\p}{\boldsymbol{p}}
%\newcommand{\s}{\mathcal{S}}
%\newcommand{\ind}{\boldsymbol{1}}
%\newcommand{\dx}{\boldsymbol{\delta}\boldsymbol{x}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\newcommand{\prox}{\operatorname{prox}}
\def\x{{ \boldsymbol x}}
\def\u{{ \boldsymbol u}}
\def\y{{\boldsymbol y}}
\def\z{{\boldsymbol z}}
\def\w{{\boldsymbol w}}

\def\xt{ \boldsymbol x^t}
\newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
\newcommandx{\normLigne}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2\Vert^{#1}}}


\newcommand\mycomment[1]{\textcolor{red}{#1}}

%\theoremstyle{definition}
%\newtheorem{defn}{Definition}[section]
%\newtheorem{assump}{A}[paragraph]
%\newtheorem{prop}{Proposition}[section]
%\newtheorem{theo}{Theorem}[section]
%\newtheorem{coro}{Corollary}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{exmp}{Example}[section]

\def\xstart{x^{\star}_{\theta}}

%%%%%%%%%%%%%%%
%% mathbf

\def\bfn{\mathbf{n}}
\def\bfw{\mathbf{w}}
\def\bfc{\mathbf{c}}
\def\bfY{\mathbf{Y}}
\def\hbfY{\hat{\mathbf{Y}}}
\def\bhfY{\hat{\mathbf{Y}}}
\def\bbfY{\bar{\mathbf{Y}}}
\def\bfX{\mathbf{X}}
\def\bhfX{\hat{\mathbf{X}}}
\def\bbfX{\bar{\mathbf{X}}}
\def\bfV{\mathbf{V}} 
\def\bfU{\mathbf{U}}
\def\bfGamma{\bm{\Gamma}}
\def\bfQ{\mathbf{Q}}
\def\bfP{\mathbf{P}}
\def\bfZ{\mathbf{Z}}
\def\bfXt{\tilde{\mathbf{X}}}
\def\bfXd{\overline{\mathbf{X}}}
\def\bfYd{\overline{\mathbf{Y}}}
\def\bfZ{\mathbf{Z}}
\def\bbfX{\tilde{\mathbf{X}}}
\def\bfM{\mathbf{M}}
\def\bfB{\mathbf{B}}
\def\bfP{\mathbf{P}}
%%% mathsf
\def\msi{\mathsf{I}}
\def\msa{\mathsf{A}}
\def\msd{\mathsf{D}}
\def\msk{\mathsf{K}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\msat{\tilde{\mathsf{A}}}
\def\msb{\mathsf{B}}
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{o}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
\def\msx{\mathsf{X}}
\def\msz{\mathsf{Z}}
\def\msy{\mathsf{Y}}



%% mathcal
\def\mca{\mathcal{A}}
\def\mct{\mathcal{T}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcbb{\mathcal{B}}  %%% \mcb est déjà pris
\newcommand{\mcb}[1]{\mathcal{B}(#1)}
\def\mcc{\mathcal{C}}
\def\mcz{\mathcal{Z}}
\def\mcy{\mathcal{Y}}
\def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcs{\mathcal{S}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}

%% mathbb

\def\Qbb{\mathbb{Q}}
\def\Pbb{\mathbb{P}}
\def\Hbb{\mathbb{H}}
\newcommand{\Qit}[1]{\Qbb^{(#1)}}
\newcommand{\Pit}[1]{\Pbb^{(#1)}}

\def\rset{\mathbb{R}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^{\star}}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}

\def\bN{\mathbb{N}}
\def\bR{\mathbb{R}}
\def\bRd{\mathbb{R}^{\dim}}
\def\cF{\mathcal{F}}


%%%% mathrm

\def\rmP{\mathrm{P}}
\def\rmQ{\mathrm{Q}}
\def\rmR{\mathrm{R}}
\def\rmb{\mathrm{b}}
\def\mrb{\mathrm{b}}
\def\wrm{\mathrm{w}}
\def\rmw{\mathrm{w}}
\def\rmd{\mathrm{d}}
\def\rms{\mathrm{s}}
\def\rmZ{\mathrm{Z}}
\def\rmS{\mathrm{S}}
\def\mrd{\mathrm{d}}
\def\mre{\mathrm{e}}
\def\rme{\mathrm{e}}
\def\rmn{\mathrm{n}}
\def\mrn{\mathrm{n}}
\def\mrc{\mathrm{C}}
\def\mrcc{\mathrm{c}}
\def\rmc{\mathrm{C}}
\def\rmC{\mathrm{C}}
\def\GaStep{\Gamma}
\def\rmcc{\mathrm{c}}
\def\rma{\mathrm{a}}
\def\rmA{\mathrm{A}}
\def\rmL{\mathrm{L}}
\def\rmf{\mathrm{f}}
\def\rmg{\mathrm{g}}
\def\rmh{\mathrm{h}}
\def\rmv{\mathrm{v}}
\def\mra{\mathrm{a}}

\def\cov{\mathrm{Cov}}

\newcommand{\cco}{\llbracket}
\newcommand{\ccf}{\rrbracket}
\newcommand{\po}{\left(}
\newcommand{\pf}{\right)}
\newcommand{\co}{\left[}
\newcommand{\cf}{\right]}
\newcommand{\R}{\mathbb R}
\newcommand{\Z}{\mathbb Z}
\newcommand{\D}{\mathcal D}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\A}{\mathcal A}
\newcommand{\M}{\mathcal M}
\newcommand{\na}{\nabla}
\newcommand{\loiy}{\mu_{\mathrm{v}}}


\def\MeasFspace{\mathbb{M}}
\def\xstar{x^\star}
\def\Tr{\operatorname{T}}
\def\trace{\operatorname{Tr}}
\newcommandx{\functionspace}[2][1=+]{\mathbb{F}_{#1}(#2)}
%% argmin, argmax
\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\estimateur}[1]{\hat{\pi}_n^N(#1)}
\def\RichR{\operatorname{R}}
\def\piR{\hat{\pi}^{\RichR}}
\def\estimatorRR{\piR}
\newcommandx{\VarDeux}[3][3=]{\operatorname{Var}^{#3}_{#1}\left\{#2 \right\}}
\newcommand{\VarDeuxLigne}[2]{\operatorname{Var}_{#1}\{#2 \}}
\newcommand{\gramm}{\operatorname{Gramm}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\2}[1]{\mathbbm{1}_{\{#1\}}}




\newcommand{\LeftEqNo}{\let\veqno\@@leqno}

\newcommand{\lambdast}{\lambda^{s \rightarrow t}}
\newcommand{\etast}{\eta^{s \rightarrow t}}
\newcommand{\mst}{m^{s \rightarrow t}}
\newcommand{\mun}{m^{1 \rightarrow 2}}
\newcommand{\mdeux}{m^{2 \rightarrow 1}}
\newcommand{\lambdaun}{\lambda^{2 \rightarrow 1}}
\newcommand{\etaun}{\eta^{2 \rightarrow 1}}
\newcommand{\lambdadeux}{\lambda^{1 \rightarrow 2}}
\newcommand{\etadeux}{\eta^{1 \rightarrow 2}}
\newcommand{\mnun}{m^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\etanun}{\eta^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\lambdanun}{\lambda^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\xpinun}{x_{\pi(n+1)}}
\newcommand{\xnun}{x_{n+1}}
\newcommand{\mpinun}{m^{\pi(n+1) \rightarrow n+1}}
\newcommand{\etapinun}{\eta^{\pi(n+1) \rightarrow n+1}}
\newcommand{\lambdapinun}{\lambda^{\pi(n+1) \rightarrow n+1}}
\newcommand{\pinun}{\pi(n+1)}
\newcommand{\vois}{\mathcal{N}}
\newcommand{\mpii}{m^{i \rightarrow \pi(n+1)}}
\newcommand{\etapii}{\eta^{i \rightarrow \pi(n+1)}}
\newcommand{\lambdapii}{\lambda^{i \rightarrow \pi(n+1)}}
\newcommand{\alphahat}{\widehat{\alpha}}
\newcommand{\betahat}{\widehat{\beta}}
\newcommand{\tildegamma}{\widetilde{\gamma}}
\newcommand{\tildeP}{\widetilde{P}}

\newcommand{\myeqref}[1]{Eq.~\eqref{#1}}



%%%% Floating Points Notation

\newcommand{\fpround}[1]{\lfloor #1 \rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\floorLigne}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}



%voc
\newcommand{\pth}{\ensuremath{p^{\text{th}}}}
\newcommand{\qth}{\ensuremath{q^{\text{th}}}}
\newcommand{\nth}{\ensuremath{n^{\text{th}}}}

%order
\newcommand{\ord}{\ensuremath{\operatorname{ord}}}
\newcommand{\rad}{\ensuremath{\operatorname{rad}}}



% Sets
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

%\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\primes}{\ensuremath{\mathcal P}}

\newcommand{\sfi}{\ensuremath{\mathcal{S}\!\mathcal{F}}}
\newcommand{\sfibt}{\ensuremath{\mathcal{S}\!\mathcal{F}'}}

\newcommand{\reghat}{\widehat{R}}

\newcommand{\reghatn}{\widehat{R}_n}

\newcommand{\arm}{\mathcal{A}}

\newcommand{\mX}{\widehat{X}}
\newcommand{\PE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\Ft}{\mathcal{F}}

\newcommand{\Sy}{\mathbf{S}}

\newcommand{\Kfrac}{\mathscr{K}}
\newcommand{\Pens}{\mathscr{P}}
\newcommand{\Fun}{\mathscr{F}}

% Operands
\newcommand{\absolute}[1]{\left\vert #1 \right\vert}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\absLigne}[1]{\vert #1 \vert}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathrm{TV}}}
\newcommand{\tvnormLigne}[1]{\| #1 \|_{\mathrm{TV}}}
\newcommand{\tvnormEq}[1]{\left \| #1 \right \|_{\mathrm{TV}}}
\newcommandx{\Vnorm}[2][1=V]{\| #2 \|_{#1}}
\newcommandx{\VnormEq}[2][1=V]{\left\| #2 \right\|_{#1}}
% \newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
% \newcommandx{\normLigne}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2\Vert^{#1}}}
\newcommand{\crochet}[1]{\left\langle#1 \right\rangle}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\newcommand{\parentheseLigne}[1]{(#1 )}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\newcommand{\parentheseDeuxLigne}[1]{[ #1 ]}
\newcommand{\defEns}[1]{\left\lbrace #1 \right\rbrace }
\newcommand{\defEnsLigne}[1]{\lbrace #1 \rbrace }
\newcommand{\defEnsPoint}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsPointDeux}[1]{\left. #1 \right  \rbrace }
\newcommand{\defEnsL}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsR}[1]{\left. #1 \right  \rbrace }

%\newcommand{\defSystem}[1]{\left\lbrace #1 \right. }

\newcommand{\ps}[2]{\left\langle#1,#2 \right\rangle}
\newcommand{\eqdef}{=}
\newcommand{\defeq}{=}

% Relations
\newcommand{\divid}{\mid}
\newcommand{\ndivide}{\nmid}

% Proba
\newcommand{\proba}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\probaCond}[2]{\mathbb{P}\left( \left. #1  \middle\vert #2 \right.\right)}
\newcommand{\probaLigne}[1]{\mathbb{P}( #1 )}
\newcommandx\probaMarkovTilde[2][2=]
{\ifthenelse{\equal{#2}{}}{{\widetilde{\mathbb{P}}_{#1}}}{\widetilde{\mathbb{P}}_{#1}\left[ #2\right]}}
\newcommand{\probaMarkov}[2]{\mathbb{P}_{#1}\left[ #2\right]}
\newcommand{\probaMarkovDD}[1]{\mathbb{P}_{#1}}
\newcommand{\expe}[1]{\PE \left[ #1 \right]}
\newcommand{\expesq}[1]{\PE^{1/2} \left[ #1 \right]}
\newcommand{\expeExpo}[2]{\PE^{#1} \left[ #2 \right]}
\newcommand{\expeLigne}[1]{\PE [ #1 ]}
\newcommand{\sqexpeLigne}[1]{\PE^{1/2} [ #1 ]}
\newcommand{\expeLignesqrt}[1]{\PE^{1/2} [ #1 ]}
\newcommand{\expeLignesqrtt}[1]{\PE^{1/4} [ #1 ]}
\newcommand{\expeLine}[1]{\PE [ #1 ]}
\newcommand{\expeMarkov}[2]{\PE_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovD}[3]{\PE_{#1}^{#3} \left[ #2 \right]}
\newcommand{\expeMarkovDD}[1]{\PE_{#1}}
\newcommand{\expeMarkovLigne}[2]{\PE_{#1} [ #2 ]}
\newcommand{\expeMarkovExpo}[3]{\PE_{#1}^{#2} \left[ #3 \right]}
\newcommand{\probaMarkovTildeDeux}[2]{\widetilde{\mathbb{P}}_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovTilde}[2]{\widetilde{\PE}_{#1} \left[ #2 \right]}

% Landau notation (big O)
\newcommand{\bigO}{\ensuremath{\mathcal O}}
\newcommand{\softO}{\Tilde{\ensuremath{\mathcal O}}}

% Environments

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}



%fleche limite
\newcommand{\flecheLimite}{\underset{n\to+\infty}{\longrightarrow}}
\newcommand{\flecheLimiteOption}[2]{\underset{#1\to#2}{\longrightarrow}}
\newcommand{\flecheLimiteHaut}{\overset{n\to+\infty}{\longrightarrow}}


%notation infini
\newcommand{\plusinfty}{+\infty}

%notation egale
\newcommand{\egale}[1]{\ensuremath{\underset{#1}{=}}}

%plusieurs ligne indice
%\sum\limits_{\substack{i=0 \\ i \neq i_0}}^{n}{A_



\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


\newcommand{\hilbert}{\mathcal{H}}


\def\ie{\textit{i.e.}}
\def\as{\textit{a.s}}
\def\cadlag{càdlàg}
\def\eqsp{}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}

\def\primr{f_r}
\def\primrO{f_{r_0}}




\newcommand{\indi}[1]{\1_{#1}}
\newcommandx{\weight}[2][2=n]{\omega_{#1,#2}^N}
\newcommand{\loi}{\mathcal{L}}
\newcommand{\boule}[2]{\operatorname{B}(#1,#2)}
\newcommand{\ball}[2]{\operatorname{B}(#1,#2)}
\newcommand{\boulefermee}[2]{\bar{B}(#1,#2)}
\newcommand{\cball}[2]{\bar{\operatorname{B}}(#1,#2)}
\newcommand{\diameter}{\operatorname{diam}}
\newcommand{\deta}{d_{\eta}}

\def\TV{\mathrm{TV}}



\newcommand{\alain}[1]{\todo[color=blue!20]{{\bf AD:} #1}}
\newcommand{\alaini}[1]{\todo[color=blue!20,inline]{{\bf AL:} #1}}
\newcommand{\valentin}[1]{\todo[color=blue!20]{{\bf VDB:} #1}}
 \newcommand{\valentini}[1]{\todo[color=blue!20,inline]{{\bf VDB:} #1}}
\newcommand{\xavier}[1]{\todo[color=blue!20]{{\bf XF:} #1}}
 \newcommand{\xavieri}[1]{\todo[color=blue!20,inline]{{\bf XF:} #1}}

% \newcommand{\aymeric}[1]{\todo[color=blue!20]{{\bf AD:} #1}}
% \newcommand{\francis}[1]{\todo[color=black!20]{{\bf FB:} #1}}
 \newcommand{\tcr}[1]{\textcolor{red}{#1}}
% \newcommand{\tcb}[1]{\textcolor{blue}{#1}}


\def\as{\ensuremath{\text{a.s.}}}
\def\dist{\operatorname{dist}}

\newcommandx\sequence[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2}, \eqsp #2 \in #3 \}}}}

\newcommandx\sequenceD[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{( #1)_{ #2 \in #3} }}}

\newcommandx{\sequencen}[2][2=n\in\N]{\ensuremath{\{ #1_n, \eqsp #2 \}}}
\newcommandx\sequenceDouble[4][3=,4=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ (#1_{#3},#2_{#3}) \}}}{\ensuremath{\{  (#1_{#3},#2_{#3}), \eqsp #3 \in #4 \}}}}
\newcommandx{\sequencenDouble}[3][3=n\in\N]{\ensuremath{\{ (#1_{n},#2_{n}), \eqsp #3 \}}}


\newcommand{\wrt}{w.r.t.}
\newcommand{\Withoutlog}{w.l.o.g.}
\def\iid{i.i.d.}
\def\ifof{if and only if}
\def\eg{\textit{e.g.}}


\newcommand{\notered}[1]{{\textbf{\color{red}#1}}}


\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}



%\def\Lip{\operatorname{Lip}}
\def\generator{\mathcal{A}}
\def\generatorsp{\generator^{\sphere^d}}
\def\generatorr{\generator^{\rset^d}}

\def\momentNoise{\mathrm{m}}
\def\bfe{\mathbf{e}}

\def\bfv{\mathbf{v}}
\def\ebf{\mathbf{e}}
\def\vbf{\mathbf{v}}


\def\Id{\operatorname{Id}}

\def\tildetheta{\tilde{\theta}}

\def\calC{\mathcal{C}}


\newcommandx{\CPE}[3][1=]{{\mathbb E}_{#1}\left[#2 \middle \vert #3  \right]} %%%% esperance conditionnelle
\newcommandx{\CPELigne}[3][1=]{{\mathbb E}_{#1}[#2  \vert #3  ]} %%%% esperance conditionnelle
\newcommandx{\CPEsq}[3][1=]{{\mathbb{E}^{1/2}}_{#1}\left[#2 \middle \vert #3  \right]} %%%% esperance conditionnelle
\newcommandx{\CPVar}[3][1=]{\mathrm{Var}^{#3}_{#1}\left\{ #2 \right\}}
\newcommand{\CPP}[3][]
{\ifthenelse{\equal{#1}{}}{{\mathbb P}\left(\left. #2 \, \right| #3 \right)}{{\mathbb P}_{#1}\left(\left. #2 \, \right | #3 \right)}}

\def\Ascr{\mathscr{A}}
\def\scrA{\mathscr{A}}
\def\scrB{\mathscr{B}}
\def\scrC{\mathscr{C}}

\def\barL{\bar{L}}

\def\YL{\mathbf{Y}}
\def\XEM{X}
\def\steps{\gamma}
\def\measSet{\mathbb{M}}

\newcommand\Ent[2]{\mathrm{Ent}_{#1}\left(#2\right)}
\newcommandx{\osc}[2][1=]{\mathrm{osc}_{#1}(#2)}

\def\Ybar{\bar{Y}}
\def\Id{\operatorname{Id}}
\def\IdM{\operatorname{I}_d}
\newcommand\EntDeux[2]{\Ent_{#1}\left[#2 \right]}
\def\Ltwo{\mathrm{L}^2}
\def\Lone{\mathrm{L}^1}
\newcommand\densityPi[1]{\frac{\rmd #1}{\rmd \pi}}
\newcommand\densityPiLigne[1]{\rmd #1 /\rmd \pi}
\newcommand\density[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand\densityLigne[2]{\rmd #1/\rmd #2}

\def\V{V}
\def\VD{V}
\def\Vsp{V^{\sphere^d}_{\b,\beta}}
\def\Vr{V^{\rset^d}_{\b,\c,\beta}}

\def\Prset{P^{\rset^d}}
\def\Psphere{P^{\sphere^d}}

\def\n{\mathrm{n}}
\def\Vpsi{\psi}
\def\Vkappa{\kappa}
\def\Vkappat{\tilde{\kappa}}
\def\Vchi{\chi}
\def\Vchit{\tilde{\chi}}
\def\Vphi{\phi}
\def\Vrho{\rho}
\def\psiV{\Vpsi}
\def\rhoV{\Vrho}
\def\phiV{\Vphi}
\def\fV{f}
\def\Vf{\fV}
\def\kappaVt{\tilde{\Vkappa}}
\def\kappaV{\Vkappa}
\def\chiV{\Vchi}
\def\chiVt{\Vchit}


\def\a{a}
\def\b{b}
\def\e{e}
\def\rU{\mathrm{r}}

\def\domain{\mathrm{D}}

\def\martfg{M^{f,g}}
\newcommand\Ddir[1]{D_{#1}}
\newcommand\maxplus[1]{\parenthese{#1}_+}
\def\Refl{\mathrm{R}}
\def\phibf{\pmb{\phi}}
\def\Gammabf{\mathbf{\Gamma}}


\def\transpose{\top}
\def\v{v}
\def\w{w}
\def\y{y}
\def\z{z}
%%%% bar
\def\bD{\bar{D}}
\def\bC{\bar{C}}
\def\brho{\bar{\rho}}
\def\bt{\bar{t}}
\def\bA{\bar{A}}
\def\bb{\overline{b}}
\def\bc{\bar{c}}
\def\bgamma{\bar{\gamma}}
\def\bU{\bar{U}}
\def\Ub{\bU}
\def\lambdab{\bar{\lambda}}
\def\blambda{\bar{\lambda}}
\def\blambdab{\bar{\lambda}}
\def\bv{\bar{v}}
\def\vb{\bv}
\def\yb{\bar{y}}
\def\by{\yb}
\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\taub{\bar{\tau}}

\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}

\def\pib{\bar{\pi}}
\def\bpi{\pib}

\def\S{S}

%%%% tilde
\def\tgamma{\tilde{\gamma}}
\def\tC{\tilde{C}}
\def\tB{\tilde{B}}
\def\tc{\tilde{c}}
\def\tvareps{\tilde{\vareps}}
\def\trho{\tilde{\rho}}
\def\tmsk{\tilde{\msk}}
\def\tW{\tilde{W}}
\def\tvarsigma{\tilde{\varsigma}}
\def\tv{\tilde{v}}
\def\vt{\tv}
\def\yt{\tilde{y}}
\def\ty{\yt}
\def\Mt{\tilde{M}}
\def\tM{\Mt}

\def\tx{\tilde{x}}
\def\xt{\tx}
\def\Xt{\tilde{X}}
\def\Yt{\tilde{Y}}
\def\Gt{\tilde{G}}
\def\Et{\tilde{E}}
\def\Tt{\tilde{T}}
\def\St{\tilde{S}}
\def\taut{\tilde{\tau}}

\def\tX{\tilde{X}}
\def\tY{\tilde{Y}}
\def\tG{\tilde{G}}
\def\tE{\tilde{E}}
\def\tT{\tilde{T}}
\def\tS{\tilde{S}}
\def\ttau{\tilde{\tau}}


\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\Sb{\bar{S}}
\def\taub{\bar{\tau}}
\def\Hb{\bar{H}}
\def\Nb{\bar{N}}


\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}
\def\bS{\bar{S}}
\def\bH{\bar{H}}
%\def\bN{\bar{N}}

%%%%%%%%

\def\mgU{\mathrm{m}_{\nabla U}}
\def\MintDrift{I}
\def\CU{C_U}
\def\RU{R_1}
\def\RV{R}
\def\Reps{R_{\epsilon}}
\def\Resp{\Reps}
\def\veps{\varepsilon}

\def\sphere{\mss}

\def\nablaUt{\overline{\nabla U}}
\def\measureSphere{\nu^d}

\def\etaU{\eta}
\def\epsilonU{\epsilon}

\def\Jac{\operatorname{Jac}}
\def\jac{\operatorname{Jac}}
\def\sign{\operatorname{sign}}
\def\rate{\lambda_{\mathrm{r}}}







\def\sigmaS{\sigma^2}

\newcommand{\ensemble}[2]{\left\{#1\,:\eqsp #2\right\}}
\newcommand{\ensembleLigne}[2]{\{#1\,:\eqsp #2\}}
\newcommand{\set}[2]{\ensemble{#1}{#2}}

\def\rmD{\mathrm{D}}%%rmd déjà pris
\def\mrd{\mathrm{D}}
\def\mrc{\mathrm{C}}

\def\diag{\Delta_{\rset^d}}

\def\lyap{W}
\newcommand\coupling[2]{\Gamma(\mu,\nu)}
\def\supp{\mathrm{supp}}
\def\tpi{\tilde{\pi}}
\newcommand\adh[1]{\overline{#1}}

\def\ACb{\mathrm{AC}_{\mathrm{b}}}

\def\opK{\mathrm{K}}

\newcommand{\fracm}[2]{\left. #1 \middle / #2 \right.}
\newcommand{\fraca}[2]{ #1  / #2 }
\newcommand{\fracaa}[2]{ #1  / (#2) }

\newcommand{\complementary}{\mathrm{c}}

% \renewcommand{\geq}{\geqslant}
% \renewcommand{\leq}{\leqslant}
\def\poty{H}
\def\diam{\mathrm{diam}}
\def\talpha{\tilde{\alpha}}
% \def\Leb{\mathrm{Leb}}
\def\Leb{\lambda}
\newcommand{\iintD}[2]{\{#1,\ldots,#2\}}
\def\interior{\mathrm{int}}
\def\iff{ if and only if }

\def\vareps{\varepsilon}
\def\bvareps{\bar{\varepsilon}}
\def\varespilon{\varepsilon}
\def\si{\text{ if } }
\def\proj{\operatorname{proj}}
\def\projd{\operatorname{proj}^{\msd}}
\def\Phibf{\mathbf{\Phi}}
\def\Psibf{\mathbf{\Psi}}

\def\rker{\mathrm{R}}
\def\kker{\mathrm{k}}

\def\VEa{V}
\def\KUa{K}
\newcommandx{\KL}[2]{\operatorname{KL}\left( #1 | #2 \right)}
\newcommandx{\KLLigne}[2]{\operatorname{KL}( #1 | #2 )}
\newcommandx{\KLLignesqrt}[2]{\operatorname{KL}^{1/2}( #1 | #2 )}

\def\gaStep
\def\QKer{Q}
\def\Tg{\mathcal{T}_{\gamma}}
\def\mcurb{m}
%\newcommand{\coupling}[1]{\Gamma\left( #1 \right)}
\newcommand{\couplingLine}[1]{\Gamma( #1 )}
\def\distance{\mathbf{d}}
\newcommandx{\wasserstein}[3][1=\distance,3=]{\mathbf{W}_{#1}^{#3}\left(#2\right)}
\newcommandx{\wassersteinLigne}[3][1=\distance,3=]{\mathbf{W}_{#1}^{#3}(#2)}
\newcommandx{\wassersteinD}[1][1=\distance]{\mathbf{W}_{#1}}
\newcommandx{\wassersteinDLigne}[1][1=\distance]{\mathbf{W}_{#1}}


\def\Rcoupling{\mathrm{R}}
\def\Qcoupling{\mathrm{Q}}
\def\Sker{\mathrm{S}}
\def\Kcoupling{\mathrm{K}}
\def\tKcoupling{\tilde{\mathrm{K}}}
\def\Lcoupling{\mathrm{L}}
\def\Kcouplingproj{\mathrm{K}^P}
\def\vepsilon{\varepsilon}


\newcommand{\defEnsE}[2]{\ensemble{#1}{#2}}
\newcommand{\expeMarkovTildeD}[3]{\widetilde{\PE}_{#1}^{#3} \left[ #2 \right]}
\newcommand{\probaMarkovTildeD}[3]{\widetilde{\PP}_{#1}^{#3} \left[ #2 \right]}
\def\coordtildex{\mathrm{w}}
\def\PPtilde{\widetilde{\PP}}
\def\PEtilde{\widetilde{\PE}}
\def\transfrr{\mathrm{F}}
\def\diagSet{\Delta_{\msx}}
\def\Deltar{\diagSet}
\def\complem{\operatorname{c}}
\def\alphar{\alpha}
\def\tildex{\tilde{x}}
\def\tildez{\tilde{z}}
\def\tildey{\tilde{y}}
\def\ar{\mathrm{a}}
\def\Kr{\mathsf{K}}
\def\Kar{K^{(\mathrm{a})}}
\def\Xr{\mathrm{X}}
\def\Yr{\mathrm{Y}}
\def\Xrd{\mathit{X}}
\def\Yrd{\mathit{Y}}
\def\Zr{\mathrm{Z}}
\def\Ur{\mathrm{U}}
\def\sigmaD{\sigma^2}
\def\sigmakD{\sigma^2_k}
\newcommandx{\phibfs}[1][1=]{\pmb{\varphi}_{\sigmaD_{#1}}}
\def\vphibf{\pmb{\varphi}}
\def\varphibf{\pmb{\varphi}}
\def\phibfvs{\pmb{\varphi}_{\varsigma^2}}
\def\funreg{\mct}
\def\kappar{\varpi}
\def\Pr{\mathsf{P}}
\def\Par{P^{(\mathrm{a})}}
\def\Qr{\mathsf{Q}}
\def\Qar{Q^{(\mathrm{a})}}
\def\eventA{\msa}

\def\borelSet{\B}
\def\Er{\mathrm{E}}
\def\er{\mathrm{e}}
\def\transp{\operatorname{T}}

\newcommandx\sequenceg[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{( #1_{#2})}}{\ensuremath{( #1_{#2})_{ #2 \geq #3}}}}


\def\indiar{\iota}
\def\rated{\chi}
\def\transar{\tau}
\def\filtrationTilde{\tilde{\mcf}}

\def\discrete{\mathrm{d}}
\def\continuous{\mathrm{c}}


\def\Xar{X^{(\mathrm{a})}}
\def\Yar{Y^{(\mathrm{a})}}
\def\War{W^{(\mathrm{a})}}
\def\Xiar{\Xi^{(\mathrm{a})}}
\def\mcfar{\mcf^{(\mathrm{a})}}

\def\Xart{\tilde{X}^{(\mathrm{a})}}
\def\Yart{\tilde{Y}^{(\mathrm{a})}}


\def\Kker{\Kcoupling}
\def\KkerD{\tilde{\Kcoupling}}
\def\Rker{\Rcoupling}
\def\tRker{\tilde{\Rker}}
\def\Pker{\mathrm{P}}
\def\Qker{\mathrm{Q}}
\def\Lker{\mathrm{L}}

\def\VlyapD{W}
\def\VlyapDun{W_1}
\def\VlyapDdeux{W_2}
\def\VlyapDtrois{W_3}
% \newcommandx{\distV}[1][1=W]{\mathbf{d}_{#1}}
\newcommandx{\distV}[1][1=\bfc]{\mathbf{W}_{#1}}
\newcommandx{\distVdeux}[1][1=W_2]{\mathbf{d}_{#1}}

\def\inv{\leftarrow}
\newcommand{\couplage}[2]{\Pi(#1,#2)}
\def\mtt{\mathtt{m}}
\def\mttzero{\mathtt{m}_0}
\def\tmtt{\tilde{\mathtt{m}}}
\def\ttm{\mathtt{m}}
\def\mttplus{\mathtt{m}^{+}}
\def\mttplusun{\mathtt{m}_1^{+}}
\def\mttplusdeux{\mathtt{m}_2^{+}}
\def\ttmplus{\mathtt{m}^{+}}
\def\cconst{\mathtt{a}}
\def\Run{R_1}
\def\Rdeux{R_2}
\def\Rtrois{R_3}
\def\Rquatre{R_4}
\def\tR{\tilde{R}}
\def\tmttplus{\tilde{\mtt}^+}
\newcommand{\tup}[1]{\textup{#1}}
\def\Fix{\operatorname{Fix}}
\newcommand{\stopping}[1]{\T_{\msc,\mathtt{n}_0}^{(#1)}}
\def\wass{\mathcal{W}}
\def\distY{\mathbf{d}}
\def\Xibf{\boldsymbol{\Xi}}
\def\rhomax{\rho_{\rm{max}}}
\def\familydrift{\mathscr{B}}

\def\wasscun{\mathbf{W}_{\bfc_1}}
\def\wasscdeux{\mathbf{W}_{\bfc_2}}
\def\wassctrois{\mathbf{W}_{\bfc_3}}

\def\loiz{\mu_{\msz}}
\def\muz{\loiz}
\def\funH{H}

\renewcommand{\doteq}{=}
\newcommand{\Idd}{\operatorname{I}_d}

\usepackage{xspace}

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


%\def\upsigma

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main
%%% End:



==> arxiv/discretization.tex <==
\section{Discretization of backward processes}
\label{sec:discr-backw-proc}

In \Cref{sec:link-with-euler}, we briefly describe the links between our
proposed discretization and the classical Euler-Maruyama discretization. In
\Cref{sec:equivalence-with-}, we show that the discretization
\eqref{eq:discretization_improved} is associated to the one of
\cite{ho2020denoising} under specific settings

\input{euler-maruyama}

\input{equivalence_ddpm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/equivalence_ddpm.tex <==
\subsection{Equivalence with \cite{ho2020denoising}}
\label{sec:equivalence-with-}

In this section, we show that the discretization scheme introduced in
\citet{ho2020denoising} and the one of \eqref{eq:discretization_improved} are
equivalent up to the first order in some parameter.

\paragraph{Setting of \cite{ho2020denoising}}
We start by recalling the setting of \citet{ho2020denoising}. Since, there is a
conflict between our notations and the ones of \citet{ho2020denoising}, we write
our constants in \rl{red} and the constants of \citet{ho2020denoising} in
\bl{blue}.  The forward process in \citet{ho2020denoising} is given for any
$\bl{t} \in \{1, \dots, \bl{T}\}$\footnote{Note that in \citet{ho2020denoising},
  $\bl{T}$ is a number of steps and not the total time of the forward.}
\begin{equation}
  \label{eq:reference_process}
  q(x_{\bl{t}}|x_0) = \mathrm{N}(x_{\bl{t}}; \sqrt{\bl{\bar{\alpha_t}}} x_0, (1 - \bl{\bar{\alpha}_t}) \Id) \eqsp ,
\end{equation}
and we define
\begin{equation}
  \label{eq:def_bar_alpha}
  \bl{\beta_t} = 1 - \bl{\alpha_t} \eqsp , \qquad \textstyle{\bl{\bar{\alpha}_t} = \prod_{\bl{s}=1}^{\bl{t}} \bl{\alpha_s} \eqsp .}
\end{equation}
In that case the loss function is given by
\begin{equation}
  \label{eq:loss_ddpm}
  \textstyle{
    \ell(\theta) = \sum_{\bl{t}=1}^{\bl{T}} \expeLigne{\normLigne{\eps_{\bl{t}} - \bm{\eps}_\theta(\sqrt{\bl{\bar{\alpha}_t}} x_0 + \sqrt{1 - \bl{\bar{\alpha}_t}} \eps_{\bl{t}}, \bl{t})}^2} \eqsp ,
    }
  \end{equation}  
  with $\{\eps_{\bl{t}}\}_{\bl{t}=1}^{\bl{T}}$ a collection of independent Gaussian random
  variables with zero mean and identity covariance matrix.  The backward
  sampling is given by the following recursion
  \begin{equation}
    \label{eq:backward_recursion}
    x_{\bl{t-1}} = \bl{\alpha_t}^{-1/2} (x_{\bl{t}} - (\bl{\beta_t}/\sqrt{1 - \bl{\bar{\alpha}_t}}) \bm{\eps}_\theta(x_{\bl{t}}, \bl{t})) + \bl{\beta_t} z_{\bl{t}} \eqsp ,
  \end{equation}
  with$\{z_{\bl{t}}\}_{\bl{t}=1}^{\bl{T}}$ a collection of independent Gaussian
  random variables with zero mean and identity covariance matrix\footnote{We
    consider the case where $\bl{\sigma_t} = \bl{\beta_t}$.}. Note that using
  these notations, there is a conflict of notation between the forward process
  and the backward process. To clarify our identification, we denote
  $y_{\bl{t}} = x_{\bl{t}}$ for any $t \in \{0, \dots, T\}$, with $x_{\bl{t}}$
  given by \eqref{eq:backward_recursion}, in what follows.

  \paragraph{Identification}
  In what follows, we set $\bl{t} = k+1$, $\bl{T} = K$ and for any
  $\bl{t} \in \{1, \dots, \bl{T}\}$
  \begin{equation}
    \textstyle{\bl{\alpha_t} = \exp[-2 \int_{\rl{T} - t_{K+1-k}}^{\rl{T} - t_{K+1-(k+1)}} \rl{\beta_s} \rmd s] = \exp[-2 \int_{\rl{T} - t_{K+1-k}}^{\rl{T} - t_{K-k}} \rl{\beta_s} \rmd s] \eqsp .}
  \end{equation}
  For instance, we have $\bl{\alpha_1} = \exp[-2\int_0^{\rl{T}-t_K} \rl{\beta_s} \rmd s ]$ and $\bl{\alpha_T} = \exp[-2\int_{\rl{T}-t_1}^{\rl{T}} \rl{\beta_s} \rmd s ]$. Note that in this case, using \eqref{eq:def_bar_alpha}, we have
  \begin{equation}
        \textstyle{\bl{\bar{\alpha}_t}^{1/2} = \exp[-\int_{0}^{\rl{T} - t_{K-k}} \rl{\beta_s} \rmd s] = \rl{m_{\rl{T}-t_{K-k}}} \eqsp .}
      \end{equation}
      Similarly, $\sqrt{1 - \bl{\bar{\alpha}_t}} = \rl{\sigma_{\rl{T} -t_{K-k}}}$.
      In what follows, we identify the distribution of the forward process
      \eqref{eq:reference_process} with the one of
      \eqref{eq:ornstein_ulhenbeck}, the loss function \eqref{eq:loss_ddpm} with
      the one of \eqref{eq:dsm_loss} and the time reversal
      \eqref{eq:backward_recursion} with the one of
      \eqref{eq:discretization_improved}.

      \begin{enumerate}[label=(\alph*)]
      \item The distribution $q(x_{\bl{t}}|x_0)$ given in
        \eqref{eq:reference_process} is the distribution of
        $\bfX_{\rl{T} - t_{K-k}} | \bfX_0$ where
        $(\bfX_{\rl{t}})_{\rl{t} \in \ccint{0,\rl{T}}}$ is given in
        \eqref{eq:ornstein_ulhenbeck}, since
        $\bfX_{\rl{T}-t_{K-k}} = \rl{m_{T-t_{K-k}}} \bfX_0 +
        \rl{\sigma_{T-t_{K-k}}} Z$ with $Z \sim \mathrm{N}(0, \Id)$. Therefore,
        we identify $x_{\bl{t}}$ and $\bfX_{\rl{T} - t_{K-k}}$ for any
        $\bl{t} \in \{1, \dots, \bl{T}\}$. Similarly, for any
        $\bl{t} \in \{1, \dots, \bl{T}\}$, we identify $\bl{t}$ and $\rl{T} - t_{K-k}$.
      \item Using that $\bfX_{\rl{t}} = \rl{m_t} \bfX_0 + \bfB_{\rl{\sigma_t}}$
        for any $\rl{t} \in \{0, \dots, \rl{T}\}$, the loss is given by
      \begin{align}
        \ell(\bm{s}) &= \textstyle{\int_0^{\rl{T}} \kappa(\rl{t}) \expeLigne{\normLigne{\bm{s}(\rl{t}, \bfX_{\rl{t}}) - \nabla \log p_{\rl{t}|0}(\bfX_{\rl{t}}|\bfX_0)}^2} \rmd t } \\
                     & = \textstyle{\int_0^{\rl{T}} \kappa(\rl{t}) \expeLigne{\normLigne{\bm{s}(\rl{t}, \bfX_{\rl{t}}) + \bfB_{\rl{\sigma_t}} /\rl{\sigma_{\rl{t}}}^2}^2} \rmd t } \\ 
                     & = \textstyle{\int_0^{\rl{T}} \kappa(\rl{t})/\rl{\sigma_{\rl{t}}}^2 \expeLigne{\normLigne{- \rl{\sigma_{\rl{t}}} \bm{s}(\rl{t}, \bfX_{\rl{t}}) - \bfB_{\rl{\sigma_t}} /\rl{\sigma_{\rl{t}}}}^2} \rmd t } \\
                                       & = \textstyle{\int_0^{\rl{T}} \kappa(\rl{T}-\rl{t})/\rl{\sigma_{\rl{T}-\rl{t}}}^2 \expeLigne{\normLigne{- \rl{\sigma_{\rl{T}-\rl{t}}} \bm{s}(\rl{T}-\rl{t}, \bfX_{\rl{T}-\rl{t}}) - \bfB_{\rl{\sigma_{T-t}}} /\rl{\sigma_{\rl{T}-\rl{t}}}}^2}} \rmd t \eqsp .
  \end{align}
  With a slight abuse of notation we assume that
  $\kappa(\rl{T}-\rl{t}) = \sum_{k=0}^{K} \updelta_{t_{K-k}}(\rl{t})
  \rl{\sigma_{T-t}}^2$ for any $\rl{t} \in \ccint{0,\rl{T}}$.  Hence, we get
  that
\begin{align}
  \ell(\bm{s}) &= \textstyle{ \sum_{k=0}^K \expeLigne{\normLigne{\eps_{\bl{t}} - (-\rl{\sigma_{\rl{T}-t_{K-k}}}\bm{s}(\rl{T}- t_{K-k}, \bfX_{\rl{T}-t_{K-k}}))}^2}} \\
               &= \textstyle{ \sum_{k=0}^K \expeLigne{\normLigne{\eps_{\bl{t}} - (-\sqrt{1 - \bl{\bar{\alpha_t}}} \bm{s}(\rl{T}- t_{K-k}, x_t))}^2}}\\
  &= \textstyle{ \sum_{\bl{t}=1}^{\bl{T}} \expeLigne{\normLigne{\eps_{\bl{t}} - (-\sqrt{1 - \bl{\bar{\alpha_t}}} \bm{s}(\bl{t}, \sqrt{\bl{\bar{\alpha}_t}} x_0 + \sqrt{1 - \bl{\bar{\alpha}_t}} \eps_{\bl{t}}))}^2}}
\end{align}
Hence, identifying $\bm{\eps}_\theta(\cdot, \bl{t})$ and
$-\sqrt{1 - \bl{\bar{\alpha_t}}} \bm{s}(\bl{t}, \cdot)$ for any
$\bl{t} \in \{1, \dots, \bl{T}\}$, we recover \eqref{eq:loss_ddpm}.
\item We now aim at recovering \eqref{eq:backward_recursion} from
  \eqref{eq:discretization_improved}. Using the change of variable $k \to K-k$
  and noting that for any $\rl{t} \in \ocint{0, \rl{T}}$,
  $\bfB_{\rl{\sigma_t}} / \rl{\sigma_t}$ is a Gaussian random variable with zero
  mean and identity covariance matrix we have
\begin{align}
  Y_{K-k+1} &=     \textstyle{Y_{K-k} + (\exp[\int_{\rl{T}-t_{K-k+1}}^{\rl{T}-t_{K-k}} \rl{\beta_s} \rmd s] - 1) (Y_{K-k} + 2 \bm{s}(\rl{T}-t_{K-k}, Y_{K-k}))} \\
            & \qquad \textstyle{+ (\exp[2 \int_{\rl{T}-t_{K-k+1}}^{\rl{T}-t_{K-k}} \rl{\beta_s} \rmd s] - 1)^{1/2} Z_{K-k} 
              } \\
            &=     \textstyle{Y_{K-k} + (\bl{\alpha_t}^{-1/2} - 1) (Y_{K-k} + 2 \bm{s}(\rl{T}-t_{K-k}, Y_{K-k})) + \sqrt{\bl{\beta_t}} Z_{K-k} 
              } \\
            &=     \textstyle{\bl{\alpha_t}^{-1/2} Y_{K-k} + 2 (\bl{\alpha_t}^{-1/2} - 1) \bm{s}(\rl{T}-t_{K-k}, Y_{K-k}) + \sqrt{\bl{\beta_t}} Z_{K-k} 
              }\\
            &=     \textstyle{\bl{\alpha_t}^{-1/2} Y_{K-k} - 2 ((\bl{\alpha_t}^{-1/2} - 1)/\sqrt{1-\bl{\bar{\alpha}_t}}) \bm{\eps}_\theta(Y_{K-k}, \bl{t}) + \sqrt{\bl{\beta_t}} Z_{K-k} \eqsp . 
              } \label{eq:almost_discrete}
\end{align}
Finally, since $\bl{\alpha_t} = 1 - \bl{\beta_t}$ we have
$\bl{\alpha_t}^{1/2} = 1 - \bl{\beta_t}/2 + o(\bl{\beta_t})$. This implies that
$2(\bl{\alpha_t}^{-1/2} -1) = -\bl{\beta_t}/\sqrt{\bl{\alpha_t}} +
o(\bl{\beta_t}/\sqrt{\bl{\alpha_t}})$. Therefore, combining this result and
\eqref{eq:almost_discrete}, we get that
\begin{equation}
  Y_{K-k+1} =     \textstyle{\bl{\alpha_t}^{-1/2} (Y_{K-k} + (\bl{\beta_t}/\sqrt{1-\bl{\bar{\alpha}_t}}) \bm{\eps}_\theta(\bl{t}, Y_{K-k})) + \sqrt{\bl{\beta_t}} Z_{K-k} + o(\bl{\beta_t}/\sqrt{\bl{\alpha_t}})\eqsp . }
\end{equation}
This corresponds to \eqref{eq:backward_recursion} up to a term of the form
$o(\bl{\beta_t}/\sqrt{\bl{\alpha_t}})$. 
\end{enumerate}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/euler-maruyama.tex <==
\subsection{Link with Euler-Maruyama discretization}
\label{sec:link-with-euler}

First, we recall the Euler-Maruyama discretization. Given a sequence of
stepsizes a discretization of \eqref{eq:approximate_time_reversal_continuous} is
given by the so-called Euler-Maruyama approximation, \ie we define for any
$k \in \{0, \dots, K\}$ and $t \in \ccint{t_k, t_{k+1}}$
  \begin{equation}
    \label{eq:classical_EM}
    \textstyle{
      \rmd \bbfY_t^{\EM} = \beta_{T-t_k} \{ \bbfY_{t_k}^{\EM} + 2 \bm{s}(T-t_k, \bbfY_{t_k}^{\EM}) \} \rmd t + \sqrt{2\beta_{T-t_k}} \rmd \bfB_t \eqsp , \qquad \bbfY_0^{\EM} \sim \pi_\infty \eqsp .
      }
\end{equation}
The associated discrete process $(Y_k^\EM)_{k \in \{0, \dots, K+1\}}$ is given for any
$k \in \{0, \dots, K+1\}$ by $Y_k^\EM = \bbfY_{t_k}^{\EM}$ and we have for any $k \in \{0, \dots, K\}$
\begin{equation}
  \label{eq:classical_EM_disc}
  \textstyle{
    Y_{k+1}^\EM = Y_k^\EM + \gamma_k  \beta_{T-t_k} \{ Y_k^{\EM} + 2 \bm{s}(T-t_k, Y_k^{\EM}) \} + \sqrt{2 \beta_{T-t_k} \gamma_k} Z_k \eqsp ,
    }
\end{equation}
where $\{Z_k\}_{k \in \nset}$ is a sequence of independent $d$-dimensional
Gaussian random variables with zero mean and identity covariance matrix.

Note that \eqref{eq:discretization_improved} describes the same update as
\eqref{eq:classical_EM} up to the first order \wrt $\gamma_k$. In practice,
there is no additional cost to replace the classical Euler-Maruyama
discretization with the discretization defined in
\eqref{eq:discretization_improved}, provided that the integral of the
temperature schedule $t \mapsto \beta_t$ can be computed in close form, which is
the case in all the cases considered experimentally, see
\Cref{sec:assumptions-schedule}.

However, in our theoretical analysis we found out that
\eqref{eq:discretization_improved} introduces less error than
\eqref{eq:classical_EM_disc} when compared to the approximate backward process
\eqref{eq:approximate_time_reversal_continuous}. In our study we only consider
the discretization scheme $(Y_k)_{k \in \{0, \dots, K+1\}}$ but emphasize that
our analysis could be readily extended to derive similar discretization errors
for the process $(Y_k^\EM)_{k \in \{0, \dots, K+1\}}$.





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/girsanov_easy.tex <==
\section{A short proof of the results of \cite{franzese2022much}}
\label{sec:short-proof}

In \cite[Equation (9)]{franzese2022much}, the authors show that (under mild
regularity assumptions\footnote{We assume that all probability measures admit
  densities \wrt the Lebesgue measure and that all the integrals we consider
  are well-defined.})
\begin{equation}
  \label{eq:franzese_res}
  \textstyle{
    \int_{\rset^d} \log p_{\theta,T}(x) p_0(x) \rmd x \geq \int_{\rset^d} \log p_{0}(x) p_0(x) \rmd  x - \mathcal{G}(\bm{s}_\theta,T) - \KLLigne{p_T}{p_\infty} \eqsp .
    }
  \end{equation}
  To do so, they rearrange the ELBO result from \cite{huang2021variational}. We
  have that \eqref{eq:franzese_res} is equivalent to
  \begin{equation}
    \label{eq:KL_ineq}
    \KLLigne{p_0}{p_{\theta, T}} \leq \mathcal{G}(\bm{s}_\theta,T) + \KLLigne{p_T}{p_\infty} \eqsp . 
  \end{equation}
  The definition of $\mathcal{G}(\bm{s}_\theta,T)$ is given by
  \begin{align}
    \textstyle{
      \mathcal{G}(\bm{s}_\theta,T)} &= \textstyle{(1/2) (\int_0^T  \beta_t^2 \expeLigne{\normLigne{\bm{s}_\theta(t,\bfX_t) - \nabla \log p_{t|0}(\bfX_t|\bfX_0)}^2 } \rmd t} \\
    & \qquad \textstyle{- \int_0^T  \beta_t^2 \expeLigne{\normLigne{\nabla \log p_t(\bfX_t) - \nabla \log p_{t|0}(\bfX_t|\bfX_0)}^2 })} \eqsp . 
  \end{align}
  Developing the square and using that
  $\CPELigne{\nabla \log p_{t|0}(\bfX_t|\bfX_0)}{\bfX_t} = \nabla \log
    p_t(\bfX_t)$, we get that
  \begin{equation}
    \textstyle{ \mathcal{G}(\bm{s}_\theta,T)} = \int_0^T \beta_t^2 \expeLigne{\normLigne{\bm{s}_\theta(t,\bfX_t) - \nabla \log p_{t}(\bfX_t)}^2} \rmd t  \eqsp .
  \end{equation}
  Hence, combining this result and \eqref{eq:KL_ineq}, we have that
  \eqref{eq:franzese_res} is equivalent to \cite[Theorem 1]{durkan2021maximum}
  which is obtained upon combining the data-processing inequality, the
  decomposition of the Kullback-Leibler via conditioning and the Girsanov
  theorem.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/gradient_hessian_control.tex <==
\section{Gradient and Hessian controls on the logarithmic density}
\label{sec:grad-hess-contr}

Let $\pi \in \Pens(\rset^d)$ be the target probability measure. We denote
$(p_t)_{t > 0}$ such that for any $t > 0$ the density \wrt the Lebesgue
measure of the distribution of $\bfX_t$ (with initialization
$\bfX_0^N \sim \pi$) is given by $p_t$. Similarly, $\pi^N \in \Pens(\rset^d)$ be
an empirical version of $\pi$, \ie  $\pi^N = (1/N) \sum_{k=1}^N X^k$, with
$\{X^k\}_{k=1}^N \sim \pi^{\otimes N}$. We denote $(p_t^N)_{t > 0}$ such that
for any $t > 0$ the density \wrt the Lebesgue measure of the distribution of
$\bfX_t^N$ (with initialization $\bfX_0^N \sim \pi^N$) is given by $p_t$.  In
order to show the stability and growth of the processes at hand we need to
control quantities related to the gradient and Hessian of $\log q_t$ where
$q_t = p_t$ or $p_t^N$. We first show a dissipativity condition on the
gradient. We recall that for any $t \in \ccint{0,T}$
\begin{equation}
  \textstyle{
    m_t = \exp[-\int_0^t\beta_s \rmd s] \eqsp , \qquad \sigma_t^2 = 1 - \exp[-2\int_0^t\beta_s \rmd s] \eqsp .
    }
  \end{equation}
  Such dissipativity conditions will allow us to control the moments of the
  introduced backward processes.
\begin{lemma}
  \label{lemma:control_grad}
    Assume \rref{assum:manifold_hyp}. Then for any $t \in \ocint{0,T}$ and $x_t \in \rset^d$ we have that
    \begin{equation}
      \langle \nabla \log q_t(x_t), x_t \rangle \leq -\norm{x_t}^2/\sigma_t^2 + m_t \diam(\M)\norm{x_t}/\sigma_t^2 \eqsp ,    \end{equation}
    with $q_t = p_t^N$ or $p_t$. In addition, we have
    \begin{equation}
      \label{eq:bound_norm}
      \normLigne{\nabla \log q_t(x_t)}^2 \leq 2\norm{x_t}^2/\sigma_t^4 + 2m_t^2 \diam(\M)^2/\sigma_t^4 \eqsp .
    \end{equation}
  \end{lemma}

  \begin{proof}
    Let $N \in \nset$. We have that for any $t \in \ccint{0,T}$ and $x_t \in \rset^d$
    \begin{equation}
      \textstyle{
        p_t^N(x_t) = (1/N) \sum_{k=1}^N \exp[-\normLigne{x_t - m_t X^k}^2/2\sigma_t^2] / (2 \uppi \sigma_t^2)^{d/2} \eqsp ,
        }
      \end{equation}
      Therefore, we get that for any $t \in \ccint{0,T}$ and $x_t \in \rset^d$
      \begin{align}
        \textstyle{
\nabla \log p_t^N(x_t) = (-1/N) \sum_{k=1}^N (x_t - m_t X^k) \exp[-\normLigne{x_t - m_t X^k}^2/2\sigma_t^2] / ((2 \uppi \sigma_t^2)^{d/2} \sigma_t^2 p_t^N(x_t)) \eqsp .} 
\end{align}
Hence, we have
\begin{equation}
  \langle \nabla \log p_t^N(x_t), x_t \rangle \leq -\norm{x_t}^2/\sigma_t^2 + m_t \diam(\M)\norm{x_t}/\sigma_t^2 \eqsp . 
\end{equation}
Therefore taking the limit $N \to +\infty$, the same conclusion holds for
$p_t$. The proof of \eqref{eq:bound_norm} follows the same lines and is left to
the reader.
\end{proof}


We now provide controls on the Hessian $\nabla^2 \log q_t$. Such bounds allow to
control the growth (or contraction) of the tangent process. This will also allow
us to control the growth (or contraction) of the distance between backward
processes \wrt the Wasserstein distance of order one.

  \begin{lemma}
    \label{lemma:control_hessian}
    Assume \rref{assum:manifold_hyp} then we have for any $t \in \ocint{0,T}$,
    $x_t \in \rset^d$ and $\mathrm{M} \in \mathcal{M}_d(\rset^d)$
  \begin{equation}
    \langle \mathrm{M}, \nabla^2 \log q_t(x_t) \mathrm{M} \rangle \leq - (1  -  m_t^2 \diam(\M)^2 / (2\sigma_t^2) )/\sigma_t^2 \normLigne{\mathrm{M}}^2 \eqsp .
  \end{equation}
  In addition, we have
  \begin{equation}    
    \normLigne{\nabla^2 \log q_t(x_t)} \leq (1 + \diam(\M)^2)/\sigma_t^4 \eqsp . 
  \end{equation}
  More generally, we have
  \begin{align}
    &\nabla^2 \log p_t(x_t) = -\Id/\sigma_t^2 \\
    &\qquad \textstyle{+ (2\sigma_t^4)^{-1} \int_{\M \times \M} (x_0 - x_0')^{\otimes 2} \exp[-\normLigne{x_t - m_t x_0}^2/(2\sigma_t^2)] \exp[-\normLigne{x_t - m_t x_0'}^2/(2\sigma_t^2)] \rmd \pi(x_0) \rmd \pi(x_0')} \\ 
    & \qquad \qquad \textstyle{/ (\int_\M \exp[-\normLigne{x_t - m_t x_0}^2/(2\sigma_t^2)] \rmd \pi(x_0))^2 \eqsp.}
  \end{align}
\end{lemma}

\begin{proof}
  Let $N \in \nset$. We have that for any $t \in \ocint{0,T}$ and $x \in \rset^d$, $p_t^N = \bar{p}_t^N  / (2 \uppi \sigma_t^2)^{d/2} $ with 
\begin{equation}
  \textstyle{
    \bar{p}_t^N(x) = (1/N) \sum_{k=1}^N \exp[-\normLigne{x - m_t X^k}^2/2\sigma_t^2] \eqsp ,
    }
  \end{equation}
  Hence, we have
  \begin{align}
    \textstyle{
    \nabla \log \bar{p}_t^N(x) = (-1/N) \sum_{k=1}^N (x - m_t X^k) \exp[-\normLigne{x - m_t X^k}^2/2\sigma_t^2] / (\sigma_t^2 \bar{p}_t^N(x)) \eqsp .
    }
\end{align}
Hence, we get that
\begin{align}
  &\textstyle{\nabla^2 \log \bar{p}_t^N(x) = - \Id / \sigma_t^2 }\\
  &\textstyle{\quad + (1/N) \sum_{k=1}^N (x - m_t X^k) \otimes (x - m_t X^k)  \exp[-\normLigne{x - m_t X^k}^2/2\sigma_t^2] / (\sigma_t^4 \bar{p}_t^N(x)) }\\
  &\quad \textstyle{- (1/N^2) (\sum_{k=1}^N (x - m_t X^k) \exp[-\normLigne{x - m_t X^k}^2/2\sigma_t^2]) }\\
  &\quad \qquad \textstyle{\otimes (\sum_{k=1}^N (x - m_t X^k) \exp[-\normLigne{x - m_t X^k}^2/2\sigma_t^2]) / (\sigma_t^2 \bar{p}_t^N(x))^2 } \eqsp . 
\end{align}
For any $k \in \{0, \dots, N-1\}$, denote $f_t^k = -(x - m_tX^k)/\sigma_t^2$
and $e_t^k = \exp[-\normLigne{f_t^k}^2]$. Using the previous result, we have
\begin{align}
  \nabla^2 \log \bar{p}_t^N(x) &\textstyle{= - \Id / \sigma_t^2 + \sum_{k=1}^N f_t^k \otimes f_t^k  e_t^k /  \sum_{k=1}^N e_t^k } \\
  & \qquad \textstyle{ - (\sum_{k=1}^N f_t^k  e_t^k /  \sum_{k=1}^N e_t^k) \otimes (\sum_{k=1}^N f_t^k  e_t^k /  \sum_{k=1}^N e_t^k) }\\
  &\textstyle{ = -\Id / \sigma_t^2 + (1/2) \sum_{j,k=1}^N (f_t^k - f_t^j) \otimes (f_t^k - f_t^j) e_t^k e_t^j / \sum_{k,j=1}^N e_t^k e_t^j \eqsp . }\label{eq:form_empirical_hessian}
\end{align}
In addition, using that for any $\ell \in \{1, \dots, N\}$, $X^\ell \in \M$ we have that
\begin{equation}
  \normLigne{f_t^k - f_t^j} = m_t \normLigne{X^k - X^j} / \sigma_t^2 \leq m_t \diam(\M) / \sigma_t^2 \eqsp . 
\end{equation}
Therefore, we get that
\begin{equation}
  \langle \mathrm{M}, \nabla^2 \log \bar{p}_t^N(x) \mathrm{M} \rangle \leq - (1  -  m_t^2 \diam(\M)^2 / (2\sigma_t^2) )/\sigma_t^2 \normLigne{\mathrm{M}}^2  \eqsp . 
\end{equation}
Using \eqref{eq:form_empirical_hessian}, the fact that $\M$ is compact and the
strong law of large numbers we have that
\begin{align}
  &\textstyle{ \lim_{N \to +\infty} \nabla^2 \log \bar{p}_t^N(x) = -\Id / \sigma_t^2 }\\
  &\textstyle{ + \int_{\rset^d} (x - m_t x_0) \otimes (x - m_t \bar{x}_0)  \exp[- \normLigne{x - m_t x_0}^2/(2\sigma_t^2) ] \exp[- \normLigne{x - m_t \bar{x}_0}^2/(2\sigma_t^2) ]  \rmd \pi(x_0) \rmd \pi(\bar{x}_0) }\\
  &\textstyle{ / (\int_{\rset^d} \exp[- \normLigne{x - m_t \bar{x}_0}^2/(2\sigma_t^2) ]  \rmd \pi(x_0))^2 \eqsp .}
\end{align}
Hence, we get that
$\lim_{N \to +\infty} \nabla^2 \log p_t^N(x) = \nabla^2 \log p_t$, which concludes the proof.
\end{proof}

% In the special case of the hypercube we can obtain tighter control on the
% Hessian of $\log p_t$.

%   \begin{lemma}
%     \label{lemma:control_hessian_hypercube}
%     Assume \rref{assum:manifold_hyp}. In addition assume that
%     $\M= \ccint{-1,1}^{r}$ and that $\pi$ admits a positive smooth density $p$ on
%     $\M$. Then we have for any $t \in \ocint{0,T}$, $x_t \in \rset^d$ and
%     $\mathrm{M} \in \mathcal{M}_d(\rset^d)$
%   \begin{equation}
%     \langle \mathrm{M}, \nabla^2 \log p_t(x_t) \mathrm{M} \rangle \leq - (1  -  m_t^2 \diam(\M)^2 / (2\sigma_t^2) )/\sigma_t^2 \normLigne{\mathrm{M}}^2 \eqsp .
%   \end{equation}
%   In addition, we have
%   \begin{equation}    
%     \normLigne{\nabla^2 \log p_t(x_t)} \leq (1 + \diam(\M)^2)/\sigma_t^4 \eqsp . 
%   \end{equation}
% \end{lemma}

% \begin{proof}
%   The first part of the proof is similar to the one of
%   \Cref{lemma:control_hessian}. Let $t \in \ocint{0,T}$ and $x \in \rset^d$. We
%   have that
%   \begin{equation}
%     \nabla^2 \log p_t(x) = \textstyle{-\Id/\sigma_t^2 + (m_t^2/\sigma_t^4) \tilde{I}_0 / \tilde{I}_1} \eqsp ,
%   \end{equation}
%   with
%   \begin{align}
%     &\tilde{I}_0 = \textstyle{\int_{\M^2} (z-z')\otimes(z-z') \exp[-\normLigne{m_t z - x}^2/(2\sigma_t^2)-\normLigne{m_t z' - x}^2/(2\sigma_t^2)]\rmd (\pi \otimes \pi)(z,z')}/(2\uppi\sigma_t^2/m_t^2)^p \eqsp ,\\
%         &\tilde{I}_1 = \textstyle{\int_{\M^2}  \exp[-\normLigne{m_t z - x}^2/(2\sigma_t^2)-\normLigne{m_t z' - x}^2/(2\sigma_t^2)]\rmd (\pi \otimes \pi)(z,z')}/(2\uppi\sigma_t^2/m_t^2)^p \eqsp .
%   \end{align}
%   Using the change of variable $z \mapsto m_t z$ we have
%   \begin{align}
%     &\tilde{I}_0 = m_t^{-2} \textstyle{\int_{\M^2} (z-z')\otimes(z-z') \exp[-\normLigne{ z - x}^2/(2\sigma_t^2)-\normLigne{z' - x}^2/(2\sigma_t^2)]\rmd (\pi \otimes \pi)(z,z')}/(2\uppi\sigma_t^2)^p \eqsp ,\\
%         &\tilde{I}_1 = \textstyle{\int_{\M^2}  \exp[-\normLigne{z - x}^2/(2\sigma_t^2)-\normLigne{z' - x}^2/(2\sigma_t^2)]\rmd (\pi \otimes \pi)(z,z')}/(2\uppi\sigma_t^2)^p \eqsp .
%   \end{align}
%   Hence, denoting $I_0 = \tilde{I}_0 m_t^2$ and $I_1 = \tilde{I}_1$ we have
%   \begin{equation}
%     \nabla^2 \log p_t(x) = \textstyle{-\Id/\sigma_t^2 + (1/\sigma_t^4) I_0 / I_1} \eqsp .
%   \end{equation}  
%   We now provide an upper-bound on $I_0$ and a lower bound on $I_1$. We have
%   that for any $x \in \M$, $(1/\bar{p}) \leq p(x) \leq \bar{p}$ for some constant
%   $p > 0$. Hence, we get that
%   \begin{equation}
%     I_0 \leq \bar{p} \expeLigne{\normLigne{Z-Z'}^2} \leq r \bar{p} \sigma_t^2 \eqsp ,
%   \end{equation}
%   where $Z,Z'$ are independent Gaussian random variable with mean $x$ and
%   variance $\sigma_t^2 \Id$. Similarly, we have
%   \begin{equation}
%     I_1 \geq (1/\bar{p}) \probaLigne{\normLigne{Z} \leq 1}^2 \geq (1/\bar{p})(1 - \expeLigne{\normLigne})
%   \end{equation}
% \end{proof}


Finally, in order to control the local error of the time discretization, we also
need to control the time derivative of the gradient, \ie
$\partial_t \nabla \log q_t$.

\begin{lemma}
  \label{lemma:control_time_space_der}
  Assume \rref{assum:manifold_hyp}. Then for any $t \in \ocint{0,T}$ and $x_t \in \rset^d$ we have that
  \begin{equation}
    \normLigne{\partial_t \nabla \log q_t(x_t)} \leq  (\beta_t /\sigma_t^6) (2 + \diam(\M)^2)(\diam(\M) + \normLigne{x})  \eqsp .
  \end{equation}
\end{lemma}

\begin{proof}
  Let $N \in \nset$ and $t \in \ocint{0,T}$. Recall that for any $x \in \rset^d$, $p_t^N(x) = \bar{p}_t^N(x)/(2\uppi \sigma_t^2)^{d/2}$ with 
  \begin{equation}
    \textstyle{\bar{p}_t^N(x) = (1/N) \sum_{k=1}^N e_t^k(x) \eqsp , \qquad e_t^k(x) = \exp[-\normLigne{x - m_t X^k}^2/(2\sigma_t^2)] \eqsp .}
  \end{equation}
  In what follows, we denote $f_t^k = \log e_t^k$ for any $k \in \{1, \dots,
  N\}$. For any $x \in \rset^d$ we have
  \begin{equation}
    \textstyle{ \partial_t \log \bar{p}_t^N(x) = \sum_{k=1}^N \partial_t f_t^k(x) e_t^k(x) / \sum_{k=1}^N e_t^k(x)  \eqsp .}
  \end{equation}
  Therefore, we have for any $x \in \rset^d$
  \begin{align}
    &\partial_t \nabla \log \bar{p}_t^N(x) = \textstyle{\sum_{k=1}^N \partial_t \nabla f_t^k(x) e_t^k(x) / \sum_{k=1}^N e_t^k(x) } \\
                                    & \qquad  \qquad \textstyle{ + \sum_{k=1}^N \partial_t f_t^k(x) \nabla f_t^k(x) e_t^k(x) / \sum_{k=1}^N e_t^k(x) } \\
                                    & \qquad  \qquad \textstyle{ - \sum_{k,j=1}^N \partial_t f_t^k(x) \nabla  f_t^j(x) e_t^k(x) e_t^j(x)  / \sum_{k,j=1}^N e_t^k(x)e_t^j(x) } \\
                                    & \qquad = \textstyle{\sum_{k=1}^N \partial_t \nabla f_t^k(x) e_t^k(x) / \sum_{k=1}^N e_t^k(x) } \\
                                    & \qquad  \qquad \textstyle{ + (1/2) \sum_{k,j=1}^N (\partial_t f_t^k(x) - \partial_t f_t^j(x)) (\nabla  f_t^k(x) - \nabla f_t^j(x)) e_t^k(x) e_t^j(x)  / \sum_{k,j=1}^N e_t^k(x)e_t^j(x) } \eqsp . \label{eq:general_decomposition}
  \end{align}
  In what follows, we fix $k, j \in \{1, \dots, N\}$ and provide upper bounds
  for $\absLigne{\partial_t f_t^k - \partial_t f_t^j}$,
  $\normLigne{\nabla f_t^k - \nabla f_t^j}$ and $\partial_t \nabla f_t^k$. First, we
  have that for any $x \in \rset^d$, $\nabla f_t^k(x) = -(x-m_t X^k)/\sigma_t^2$.
  Hence, using that $m_t \leq 1$, we get that for any $x\in \rset^d$
  \begin{equation}
    \label{eq:control_diff_grad_log}
    \normLigne{\nabla f_t^k(x) - \nabla f_t^j(x)} \leq m_t \diam(\M)/\sigma_t^2 \leq \diam(\M)/\sigma_t^2 \eqsp .
  \end{equation}
  In addition, we have that for any $x \in \rset^d$
  \begin{equation}
    \partial_t f_t^k(t) = \partial_t \sigma_t^2 /(2\sigma_t^4) \normLigne{x - m_t X^k}^2 + \partial_t m_t/\sigma_t^2 \langle X^k, x - m_t X^k \rangle \eqsp . 
  \end{equation}
  Combining this result, the fact that
  $\partial_t \sigma_t^2 = -2m_t \partial_t m_t$ and that
  $\partial_t m_t = -\beta_t m_t$, we get that
  \begin{align}
    \partial_t f_t^k(t) &= -\beta_t m_t/\sigma_t^2 [-(m_t/\sigma_t^2) \normLigne{x - m_t X^k}^2 + \langle x - m_t X^k, X^k \rangle] \\
                      &= -\beta_t m_t/\sigma_t^2 \langle x - m_t X^k, -(m_t /\sigma_t^2)(x- m_tX^k) + X^k \rangle \\
                        &= -\beta_t m_t/\sigma_t^4 \langle x - m_t X^k, - m_t x + X^k  \rangle \\
    &= \beta_t m_t/\sigma_t^4(m_t \normLigne{x}^2 + m_t \normLigne{X^k}^2 + (1+m_t^2)\langle x, X^k \rangle) \eqsp . \label{eq:partial_time_der}
  \end{align}
  Using this result and that $m_t \leq 1$, we have that for any $x \in \rset^d$
  \begin{align}
    \label{eq:control_diff_partial_log}
    \absLigne{\partial_t f_t^k(x) - \partial_t f_t^j(x)} &\leq 2 \beta_t m_t^2  \diam(\M)^2/\sigma_t^4 + \beta_t m_t (1 + m_t^2) \diam(\M)\normLigne{x}/\sigma_t^4 \\
    &\leq 2 (\beta_t/\sigma_t^4) \diam(\M) (\diam(\M)  + \normLigne{x})  \eqsp . 
  \end{align}
  Using \eqref{eq:partial_time_der}, we have for any $x \in \rset^d$
  \begin{equation}
    \nabla \partial_t f_t^k(x) = 2 \beta_t m_t^2 /\sigma_t^4 x +( \beta_t m_t/\sigma_t^4)(1+m_t^2)X^k \eqsp . 
  \end{equation}
  Therefore, combining this result and the fact that $m_t \leq 1$, we get that for any $x \in \rset^d$
  \begin{equation}
    \label{eq:control_cross_der}
    \normLigne{\partial_t \nabla f_t^k(x)} \leq 2 (\beta_t /\sigma_t^4)(\diam(\M) +  \normLigne{x}) \eqsp . 
  \end{equation}
  Combining \eqref{eq:control_diff_grad_log},
  \eqref{eq:control_diff_partial_log} and \eqref{eq:control_cross_der} in
  \eqref{eq:general_decomposition}, we get that for any $x \in \rset^d$
  \begin{align}
    \normLigne{\partial_t \nabla \log \bar{p}_t^N(x)} &\leq 2 (\beta_t /\sigma_t^4)(\diam(\M) +  \normLigne{x}) + (\beta_t/\sigma_t^6) \diam(\M)^2 (\diam(\M)  + \normLigne{x}) \\
    &\leq (\beta_t/\sigma_t^6) (2 + \diam(\M)^2)(\diam(\M)  + \normLigne{x}) \eqsp ,
  \end{align}
  which concludes the proof using that $\lim_{N \to +\infty} \partial_t \nabla \log p_t^N(x_t) = \partial_t \nabla \log p_t$.
\end{proof}

We conclude this section with bounds on the higher-order differentials of
$\log p_t$. To compute higher derivatives we will use the following lemma.
\begin{lemma}
  \label{sec:formal_derivative}
  Let $E = \{ e_i \}_{i=1}^M$ be a family of functions such that for any
  $i \in \{1, \dots, M\}$, $e_i \in \rmc^\infty(\rset^d, \rset)$. Similarly, let
  $G = \{ g_i \}_{i=1}^M$ be a family of functions such that for any
  $i \in \{1, \dots, M\}$, $g_i \in \rmc^\infty(\rset^d, \rset^p)$. Let $F(E,G)$
  such that for any $x \in \rset^d$
  \begin{equation}
    \textstyle{
      F(E,G) = \sum_{i=1}^M g_i e_i / \sum_{i=1}^M e_i \eqsp . 
      }
    \end{equation}
    Then, we have
    \begin{equation}
      \nabla F(E,G) = F(E, \nabla G) + (1/2) F(E \otimes E, (G \ominus G) \odot (\nabla \log E \ominus \nabla \log E)) \eqsp ,
    \end{equation}
    where $\otimes$ is the tensor product, $\odot$ the pointwise product and
    $\ominus$ the tensor substraction.
  \end{lemma}

  \begin{proof}
    We assume that $p =1$. The proof in the general case is similar and left to
    the reader.  We have that
    \begin{align}
      &\nabla F(E,G) = \textstyle{\sum_{i=1}^M \nabla g_i e_i / \sum_{i=1}^M e_i + \sum_{i,j=1}^M g_i \nabla \log(e_i) e_i e_j / \sum_{i,j=1}^M e_i e_j} \\
                    & \qquad \qquad - \textstyle{\sum_{i,j=1}^M  g_i \nabla \log(e_j) e_i e_j  / \sum_{i,j=1}^M e_i e_j} \\
                    &\qquad = \textstyle{\sum_{i=1}^M \nabla g_i e_i / \sum_{i=1}^M e_i} \\
      & \qquad \qquad \textstyle{+ (1/2) \sum_{i,j=1}^M (g_i \nabla \log(e_i) + g_j \nabla \log(e_j) - g_i \nabla \log(e_j) - g_j \nabla \log(e_i)) e_i e_j / \sum_{i,j=1}^M e_i e_j } \\
&\qquad = \textstyle{\sum_{i=1}^M \nabla g_i e_i / \sum_{i=1}^M e_i} \\
      & \qquad \qquad \textstyle{+ (1/2) \sum_{i,j=1}^M (g_i - g_j) (\nabla \log e_i - \nabla \log e_j) / \sum_{i,j=1}^M e_i e_j \eqsp ,}      
    \end{align}
    which concludes the proof.
  \end{proof}

\begin{lemma}
  \label{lemma:higher_order}
  Assume \rref{assum:manifold_hyp}. Then, there exists $C \geq 0$ such that for
  any $t \in \ocint{0,T}$ we have
  \begin{equation}
    \normLigne{\nabla^2 \log p_t(x)} + \normLigne{\nabla^3 \log p_t(x)} + \normLigne{\nabla^4 \log p_t(x)} \leq C / \sigma_t^8 \eqsp .
  \end{equation}
\end{lemma}

\begin{proof}
  Let $t \in \ocint{0,T}$. First, remark that for any $x \in \rset^d$
  \begin{equation}
    \nabla^2 \log p_t(x) = -\Id /\sigma_t^2 + F(E^{\otimes 2}, (\nabla \log E \ominus \nabla \log E)^{\odot 2}) \eqsp ,
  \end{equation}
  where $E = \{ e_i \}_{i=1}^N$ and for any $i \in \{1, \dots, N\}$,
  $e_i(x) = \exp[-\normLigne{x - m_t X^i}^2/(2\sigma_t^2)]$. Note that
  $\nabla \log E \ominus \nabla \log E$ does not depend on $x$ and there exists
  $C_0 \geq 0$ such that for any $i,j \in \{1, \dots, N\}$,
  $\normLigne{\nabla \log e_i(x) - \nabla \log e_j(x)} \leq C_0
  /\sigma_t^2$. Hence, using \Cref{sec:formal_derivative} we have
  \begin{equation}
    \nabla^3 \log p_t(x) = F(E^{\otimes 4}, (\nabla \log E \ominus \nabla \log E)^{\odot 2} \odot (\nabla \log(E \otimes E) \ominus \nabla \log(E \otimes E))) \eqsp . 
  \end{equation}
  Again, note that
  $G_1 = (\nabla \log E \ominus \nabla \log E)^{\odot 2} \odot (\nabla \log(E \otimes
  E) \ominus \nabla \log(E \otimes E))$ does not depend on $x$, upon remarking that
  \begin{equation}
    \nabla \log (E \otimes E) \ominus \nabla \log (E \otimes E) = (\nabla \log E \ominus \nabla \log E) \oplus (\nabla \log E \ominus \nabla \log E) \eqsp . 
  \end{equation}
  Finally, we have $\nabla^4 \log p_t(x) = F(E^{\otimes 8}, G_2)$, where
  \begin{align}
    G_2 &= [((\nabla \log E \ominus \nabla \log E)^{\odot 2} \odot (\nabla \log(E \otimes E) \ominus \nabla \log(E \otimes E))) \\
    & \qquad \ominus ((\nabla \log E \ominus \nabla \log E)^{\odot 2} \odot (\nabla \log(E \otimes E) \ominus \nabla \log(E \otimes E)))] \odot (\nabla \log(E^{\otimes 4}) \ominus \nabla \log(E^{\otimes 4})) 
        \eqsp . 
  \end{align}
  Therefore, we get that there exists $C \geq 0$ such that for any $x \in \rset^d$
  \begin{equation}
    \normLigne{\nabla \log p_t^3(x)} \leq C / \sigma_t^6 \eqsp , \qquad \normLigne{\nabla \log p_t^4(x)} \leq C / \sigma_t^8 \eqsp .
  \end{equation}
  We conclude the proof upon using that $\sigma_t \leq 1$.
\end{proof}


  

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/header.tex <==
\usepackage[utf8]{inputenc}   % LaTeX, comprends les accents !
\usepackage[T1]{fontenc}      % Police contenant les caractÃ¨res franÃ§ais
%\usepackage[french]{babel}  % Placez ici une liste de langues
%\usepackage{multicol}

%%%%%%%%%%%%%%
%% comment uncomment
%\usepackage[notref,notcite]{showkeys}
%%%%


 % \usepackage[notref,notcite]{showkeys}  %  comment out for final version
 % \renewcommand*\showkeyslabelformat[1]{\fbox{\normalfont\scriptsize\sffamily#1}}   % for showkeys

\usepackage{comment}
\usepackage{hyperref}
\usepackage{natbib}
%\setcitestyle{square}

\usepackage[tbtags]{amsmath}
\usepackage{amsthm}
\allowdisplaybreaks
\usepackage{amssymb,mathrsfs}
\usepackage{amsfonts}
\usepackage{upgreek}
\usepackage{xspace}

\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{thistle}{rgb}{0.85, 0.75, 0.85}
\definecolor{ticklemepink}{rgb}{0.99, 0.54, 0.67}
\definecolor{thulianpink}{rgb}{0.67, 0.24, 0.43}
\definecolor{tealblue}{rgb}{0.11, 0.36, 0.43}

\usepackage{color}
\newcommand{\bl}[1]{\textcolor{tealblue}{#1}}
\newcommand{\rl}[1]{\textcolor{thulianpink}{#1}}



% \usepackage{nicefrac}

%\usepackage[numbers]{natbib}
\usepackage{graphicx}
\usepackage{subfig}
%\usepackage[caption = false]{subfig} %package pour faire sous-figures
\usepackage{color}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{algpseudocode,algorithm,algorithmicx}
\usepackage{algorithm, algorithmic}

%###########
%\usepackage{manuColor}
\usepackage{stmaryrd}
\usepackage[inline]{enumitem}
%[wide, labelwidth=!, labelindent=0pt]
\usepackage{url}
\def\UrlBreaks{\do\/\do-}
\usepackage{tikz}
\usetikzlibrary{calc}
\newcommand\yBlock{1}
\newcommand\yNode{0.75}

\newcommand\xNodemoinstiny{-1}
\newcommand\xNodemoins{-1.5}
\newcommand\xNodemoinsint{-2.}
\newcommand\xNodeMoins{-3}
\newcommand\xNodeMOINS{-4.5}

\newcommand\xNodeplustiny{1}
\newcommand\xNodeplus{1.5}
\newcommand\xNodeplusint{2}
\newcommand\xNodePlus{3}
\newcommand\xNodePLUS{4.5}

\usepackage{pgfplots}
\usepackage{bbm}
\usepackage{ifthen}
\usepackage{xargs}
\usepackage[textwidth=1.8cm]{todonotes}

\usepackage{aliascnt}
\usepackage{cleveref}
\usepackage{autonum}
\makeatletter
\newtheorem{theorem}{Theorem}
\crefname{theorem}{theorem}{Theorems}
\Crefname{Theorem}{Theorem}{Theorems}


\newtheorem*{lemma_nonumber*}{Lemma}


\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}



\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\crefname{corollary}{corollary}{corollaries}
\Crefname{Corollary}{Corollary}{Corollaries}

\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\crefname{proposition}{proposition}{propositions}
\Crefname{Proposition}{Proposition}{Propositions}

\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\crefname{definition}{definition}{definitions}
\Crefname{Definition}{Definition}{Definitions}

\newaliascnt{remark}{theorem}
\newtheorem{remark}[remark]{Remark}
\aliascntresetthe{remark}
\crefname{remark}{remark}{remarks}
\Crefname{Remark}{Remark}{Remarks}


\newtheorem{example}[theorem]{Example}
\crefname{example}{example}{examples}
\Crefname{Example}{Example}{Examples}

\newtheorem{technique}{Technique}
\crefname{technique}{technique}{techniques}
\Crefname{Technique}{Technique}{Techniques}


\crefname{figure}{figure}{figures}
\Crefname{Figure}{Figure}{Figures}


%\newtheorem{assumption}{\textbf{A}\hspace{-3pt}}
%\Crefname{assumption}{\textbf{A}\hspace{-3pt}}{\textbf{A}\hspace{-3pt}}
%\crefname{assumption}{\textbf{A}}{\textbf{A}}
\newtheorem{assumption}{\textbf{A}\hspace{-3pt}}
\crefformat{assumption}{{\textbf{A}}#2#1#3}

\newtheorem{assumptionF}{\textbf{F}\hspace{-3pt}}
\crefformat{assumptionF}{{\textbf{F}}#2#1#3}

\newenvironment{assumptionbis}[1]
  {\renewcommand{\theassumptionF}{\ref*{#1}$\mathbf{b}$}%
   \addtocounter{assumptionF}{-1}%
   \begin{assumptionF}}
  {\end{assumptionF}}



\newtheorem{assumptionB}{\textbf{B}\hspace{-3pt}}
\Crefname{assumptionB}{\textbf{B}\hspace{-3pt}}{\textbf{B}\hspace{-3pt}}
\crefname{assumptionB}{\textbf{B}}{\textbf{B}}

\newtheorem{assumptionC}{\textbf{C}\hspace{-3pt}}
\Crefname{assumptionC}{\textbf{C}\hspace{-3pt}}{\textbf{C}\hspace{-3pt}}
\crefname{assumptionC}{\textbf{C}}{\textbf{C}}


\newtheorem{assumptionH}{\textbf{H}\hspace{-3pt}}
\Crefname{assumptionH}{\textbf{H}\hspace{-3pt}}{\textbf{H}\hspace{-3pt}}
\crefname{assumptionH}{\textbf{H}}{\textbf{H}}

\newtheorem{assumptionT}{\textbf{T}\hspace{-3pt}}
\Crefname{assumptionT}{\textbf{T}\hspace{-3pt}}{\textbf{T}\hspace{-3pt}}
\crefname{assumptionT}{\textbf{T}}{\textbf{T}}

\newtheorem{assumptionD}{\textbf{D}\hspace{-3pt}}
\Crefname{assumptionT}{\textbf{T}\hspace{-3pt}}{\textbf{T}\hspace{-3pt}}
\crefname{assumptionT}{\textbf{T}}{\textbf{T}}


\newtheorem{assumptionL}{\textbf{L}\hspace{-3pt}}
\Crefname{assumptionL}{\textbf{L}\hspace{-3pt}}{\textbf{L}\hspace{-3pt}}
\crefname{assumptionL}{\textbf{L}}{\textbf{L}}

\newtheorem{assumptionQ}{\textbf{Q}\hspace{-3pt}}
\Crefname{assumptionQ}{\textbf{Q}\hspace{-3pt}}{\textbf{Q}\hspace{-3pt}}
\crefname{assumptionQ}{\textbf{Q}}{\textbf{Q}}

% \newtheorem{assumptionD*}{\textbf{D}\hspace{-3pt}}
% \Crefname{assumptionD}{\textbf{D}\hspace{-3pt}}{\textbf{D}\hspace{-3pt}}
% \crefname{assumptionD}{\textbf{D}}{\textbf{D}}

\newtheorem{assumptionAR}{\textbf{AR}\hspace{-3pt}}
\Crefname{assumptionAR}{\textbf{AR}\hspace{-3pt}}{\textbf{AR}\hspace{-3pt}}
\crefname{assumptionAR}{\textbf{AR}}{\textbf{AR}}



\newcommand\diaW{11}
\newcommand\diaH{5}
\newcommand\diaJump{2.75}
\newcommand\nextRow{1.25}
\newcommand\imW{0.08}
\newcommand\imWB{0.1}
\newcommand\imOp{0.6}
\newcommand\bend{5}

\newcommand\offset{2}
\newcommand\offsety{2.3}
\newcommand\h{2.25}
\newcommand\hsmall{1.75}
\newcommand\ww{3.25}
\newcommand\www{1.8}
\newcommand\wwww{3.5}
\newcommand\wwwww{4.8}
\newcommand{\offsetsmall}{1.5}

\usepackage{bm}
\usepackage{wrapfig}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "La"
%%% End:


==> arxiv/improved_bounds.tex <==
\section{Improved bounds under Hessian conditions}
\label{sec:impr-bounds-under}

In \Cref{sec:proof-convergence-hessian}, we prove
\Cref{thm:convergence_bound_hessian} which is an improvement upon
\Cref{thm:convergence_general} under tighter conditions on the Hessian
$\nabla^2 \log p_t$. In \Cref{sec:hess-bounds-unif}, we show that this condition
is satisfied in the case of a uniform measure over $\ccint{-1/2, 1/2}^p$ for
some $p \in \{1, \dots, d\}$. Finally, in \Cref{sec:non-conv-count}, we show,
under appropriate smoothness conditions, that the condition is never satisfied
on non-convex sets.

\subsection{Proof of \Cref{thm:convergence_bound_hessian}}
\label{sec:proof-convergence-hessian}


In this section, we prove \Cref{thm:convergence_bound_hessian}. We start by
deriving an improvement on \Cref{prop:control_gradient}. The main difference
between \Cref{prop:control_gradient} and \Cref{prop:control_gradient_improved}
lies into the dependency \wrt $\sigma_{T-t_K}^{-2}$. In
\Cref{prop:control_gradient}, we have an exponential dependency
$\exp[(\diam(\M)^2/2)\sigma_{T-t_K}^{-2}]$ whereas in \Cref{prop:control_gradient_improved}, we
have a polynomial dependency $\sigma_{T-t_K}^{-2\Gamma}$.

For ease of notation we introduce the following assumption.

\begin{assumption}
  \label{assum:hessian_bound}
  There exists $\Gamma \geq 0$ such that for any $t \in \ocint{0,T}$ and $x_t \in \rset^d$, $\normLigne{\nabla^2 \log p_t(x_t)} \leq \Gamma / \sigma_t^2$.
\end{assumption}

We start with the following proposition.

\begin{proposition}
  \label{prop:control_gradient_improved}
  Assume \rref{assum:manifold_hyp}, \rref{assum:hessian_bound} and that
  $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$.  Let $t_K \in \coint{0,
    T}$. Then, for any $t\in \ccint{0,t_K}$ and $x \in \rset^d$ we have
  \begin{equation}
    \textstyle{
      \normLigne{\nabla \bfY_{t,t_K}^x} \leq \textstyle{ \exp[-(1/2) \int_{T-t^\star}^{T-t} \beta_s \rmd s \1_{\coint{0,t^\star}}(t)] \sigma_{T-t_K}^{-2\Gamma} \exp[(\Gamma +1) \int_{T -t_K}^{T-t^\star} \beta_{u} \rmd u]\eqsp . 
      }}
    \end{equation}
  \end{proposition}

  \begin{proof}
    Let $x\in \rset^d$. First, using \eqref{eq:tangent_process} and \Cref{lemma:control_hessian} we have that for any $s, t\in \ccint{0,T}$ with $s \leq t$
    \begin{equation}
      \rmd \normLigne{\nabla \bfY_{s,t}^x}^2 \leq 2\beta_{T-t}(\normLigne{\nabla \bfY_{s,t}^x }^2 - 2(1  -  m_{T-t}^2 \diam(\M)^2 / (2\sigma_{T-t}^2) )/\sigma_{T-t}^2 \normLigne{\nabla \bfY_{s,t}^x}^2) \rmd t  \eqsp . 
    \end{equation}
    First, assume that $s \leq t^\star$ and that $t \geq t^\star$. In that case, using
    \Cref{lemma:growth_tangent_process} we have that
      \begin{equation}
\textstyle{    \int_s^{t^\star}\beta_{T-u} (1 -2/\sigma_{T-u}^2 + m_{T-u}^2\diam(\M)^2/\sigma_{T-u}^4) \rmd u  \leq -(1/2) \int_s^{t^\star} \beta_{T-u} \rmd u  \eqsp . }
\end{equation}
Therefore, using that result and the fact that $\nabla \bfY_{s,s}^x = \Id$ we get that
\begin{equation}\label{eq:inter_s_lower_imp_i}
  \textstyle{\normLigne{\nabla \bfY_{s,t^\star}} \leq \exp[-(1/2)\int_{T-t^\star}^{T-s} \beta_u \rmd u] \eqsp . }
\end{equation}
In addition, using that for any $t \in \ocint{0,T}$ and $x_t \in \rset^d$, $\normLigne{\nabla^2 \log p_t(x_t)} \leq \Gamma /\sigma_t^2$ we have
\begin{equation}
  \rmd \normLigne{\nabla \bfY_{s,t}}^2 \leq 2 \beta_{T-t} (1 + 2 \Gamma / \sigma_{T-t}^2) \normLigne{\nabla \bfY_{s,t}^2} \rmd t \eqsp . 
\end{equation}
In addition, using \Cref{lemma:integration_lemma} we have that
\begin{align}
  \textstyle{    \int_{t^\star}^{t}\beta_{T-u} (1 + 2 \Gamma / \sigma_{T-u}^2) \rmd u}  & \textstyle{\leq \Gamma[\log(\exp[2\int_0^{T-t^\star} \beta_{T-u}\rmd u ] - 1)} \\ & \qquad  \textstyle{- \log(\exp[2\int_0^{T-t} \beta_{T-u} \rmd u ] - 1)] + \int_{T -t}^{T-t^\star} \beta_{u} \rmd u } \\
                                                                                        & \textstyle{\leq \Gamma[\log(\sigma_{T-t^\star}^2) - \log(\sigma_{T-t})] +(\Gamma +1) \int_{T -t}^{T-t^\star} \beta_{u} \rmd u  } \\
  & \textstyle{\leq  - \Gamma \log(\sigma_{T-t}^2) +(\Gamma +1)  \int_{T -t}^{T-t^\star} \beta_{u} \rmd u  \eqsp. }
  \end{align}
  Therefore, combining this result and \eqref{eq:inter_s_lower_imp_i}, we get
  that
  \begin{align}
    \normLigne{\nabla \bfY_{s,t}} &\leq \textstyle{ \sigma_{T-t}^{-2\Gamma} \exp[(\Gamma +1) \int_{T -t}^{T-t^\star} \beta_{u} \rmd u] \normLigne{\nabla \bfY_{s,t^\star}}} \\
                                  &\leq \textstyle{ \sigma_{T-t}^{-2\Gamma} \exp[(\Gamma +1) \int_{T -t}^{T-t^\star} \beta_{u} \rmd u] } \exp[-(1/2)\int_{T-t^\star}^{T-s} \beta_u \rmd u] \eqsp .
  \end{align}
        The proof in the cases where $s \geq t^\star$, $t \geq t^\star$ and
        $s \leq t^\star$, $t \leq t^\star$ are similar and left to the reader.
      \end{proof}

      The rest of the proof follows the proof of
      \Cref{sec:proof_theorem_one}. The following proposition is the counterpart
      of \Cref{prop:discretization_bound_final}. Again note that the exponential
      dependency \wrt $1/\vareps$ has been replaced by a polynomial dependency.

      \begin{proposition}
  \label{prop:discretization_bound_final_improved}.
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:score_control}, \rref{assum:step_size}, \rref{assum:hessian_bound} and $t_K = T - \vareps$. In
  addition, assume that $\vareps, \delta, \Mtt \leq 1/32$.  Then
  \begin{equation}
      \wassersteinD[1](\pi_\infty \rmQ_{t_K}, \pi_\infty \rmR_{K})  \leq  \Dtt_0 (\Mtt + \delta^{1/2})/ \vareps^{\Gamma +2}  \eqsp ,
  \end{equation}
  where
  \begin{equation}
    \Dtt_0 = 4 (4 + 256 d + 43664 (1+\diam(\M))^4)\exp[3(1+\bar{\beta})^2(\Gamma+2)(1+\log(1+\diam(\M))))] \eqsp . 
  \end{equation}
\end{proposition}

\begin{proof}
  Using \Cref{prop:pierre-extended}, we have
    \begin{equation}
\textstyle{    \normLigne{\bfY_{t_K} - Y_K} \leq \int_0^{t_K} \normLigne{\nabla \bfY_{u,t_K}(\bbfY_{0,u})} \normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})} \rmd u } \eqsp .
\end{equation}
Combining this result, recalling that $t^\star$ is defined in
\eqref{eq:def_t_star} and \Cref{prop:control_gradient_improved}, we get
    \begin{align}
      \textstyle{    \normLigne{\bfY_{t_K} - Y_K}} \leq & \textstyle{ \int_0^{t_K} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s \1_{\coint{0,t^\star}}(u)] \sigma_{T-t_K}^{-2\Gamma}} \\
      & \qquad \times \textstyle{\exp[(\Gamma+1)\int_{T-t_K}^{T-t^\star}\beta_s \rmd s]  \normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})} \rmd u } \\
                                                        &\leq \sigma_{T-t_k}^{-2\Gamma} \textstyle{\exp[(\Gamma+1)\int_{T-t_K}^{T-t^\star}\beta_s \rmd s]} ( \int_0^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s] \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}}) \rmd u \\
      & \qquad \textstyle{+ \int_{t^\star}^{t_K} \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})}\rmd u ) \eqsp .
\end{align}
Using this result and \Cref{prop:local-error-control} we get
\begin{align}
  &\wassersteinD[1](\pi_\infty \rmQ_{t_K}, \pi_\infty \rmR_{K}) \leq \expeLigne{\normLigne{\bfY_{t_K} - Y_K}} \\
  &\qquad \leq \textstyle{ \sigma_{T-t_K}^{-2\Gamma} \textstyle{\exp[(\Gamma+1)\int_{T-t_K}^{T-t^\star}\beta_s \rmd s]}(\int_{0}^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s] \expeLigne{\normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})}} \rmd u} \\
      & \qquad \qquad \textstyle{+ \int_{t^\star}^{t_K} \expeLigne{\normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})}} \rmd u ) \eqsp .  } \\
  &\qquad \leq \textstyle{ \sigma_{T-t_K}^{-2\Gamma} \textstyle{\exp[(\Gamma+1)\int_{T-t_K}^{T-t^\star}\beta_s \rmd s]} \Ctt_0 (T - t_K + \bar{\beta})^2 (\Mtt + \delta^{1/2}) /(T-t_K)^2 } \\
  & \qquad \qquad \textstyle{ \times (\int_0^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s]  \rmd u + t_K - t^\star)} \\
    &\qquad \leq \textstyle{ \sigma_{T-t_K}^{-2\Gamma} \textstyle{\exp[(\Gamma+1)\bar{\beta}(t_K - t^\star) \rmd s]} \Ctt_0 (T - t_K + \bar{\beta})^2 (\Mtt + \delta^{1/2}) /(T-t_K)^2 } \\
  & \qquad \qquad \textstyle{ \times (\int_0^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s]  \rmd u + t_K - t^\star)}\eqsp . \label{eq:bound_wasserstein_intermediate_improved}
\end{align}
We have that
\begin{equation}
  \textstyle{ \int_0^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s]  \rmd u \leq \int_0^{t^\star} \exp[-(t^\star -u)/(2\bar{\beta})]  \rmd u \leq 2 \bar{\beta} \eqsp . } \label{eq:bound_integration_improved}
\end{equation}
In addition, using \eqref{eq:def_t_star}  we have
\begin{equation}
  t_K - t^\star = T - \vareps - T +2 \bar{\beta} (1 + \log(1 + \diam(\M))) \leq 2 \bar{\beta} (1 + \log(1 + \diam(\M)))  \eqsp . \label{eq:bound_tk_tstar_improved}
\end{equation}
Finally, using \Cref{lemma:bound_sigma_t}, we have that
$\sigma_{T-t_K}^{-2} \leq (1 + \bar{\beta})/\vareps$. Combining this result,
\eqref{eq:bound_integration_improved} and \eqref{eq:bound_tk_tstar_improved} in
\eqref{eq:bound_wasserstein_intermediate_improved} and that for any $a \geq 0$,
$1+a \leq \exp[a]$, we get
\begin{align}
  \wassersteinD[1](\pi_\infty \rmQ_{t_K}, \pi_\infty \rmR_{K}) &\leq 4(1+ \bar{\beta})^{\Gamma+3} (1 + \log(1 + \diam(\M))) \\
   & \qquad \times \exp[2\bar{\beta}^2(\Gamma +1)(1 + \log(1+\diam(\M)))] 
     \Ctt_0 (\Mtt + \delta^{1/2})\vareps^{-(\Gamma+2)} \\
  &\leq 4(1+ \bar{\beta})^{\Gamma+3} (1 + \log(1 + \diam(\M))) \\
   & \qquad \times \exp[2\bar{\beta}^2(\Gamma +1)(1 + \log(1+\diam(\M)))] 
     \Ctt_0 (\Mtt + \delta^{1/2})\vareps^{-(\Gamma+2)} \\
  &\leq 4 \exp[3\bar{\beta}^2(\Gamma +2)(1 + \log(1+\diam(\M)))] 
     \Ctt_0 (\Mtt + \delta^{1/2})\vareps^{-(\Gamma+2)} \eqsp ,
\end{align}
which concludes the proof.
%   &\qquad \leq \textstyle{ \exp[(1/2)\sigma_{T-t_K}^{-2}] (1 + \Dtt) \Ctt (\Mtt + \delta^{1/2}) /(T-t_K)^2  (1 + t_K - t^\star)} \eqsp ,q:
% \end{align}
% where $\Dtt_0 = \int_0^{T} \exp[-(1/2) \int_0^{T-u} \beta_s \rmd s] \rmd u $. We conclude upon using that 
% \begin{equation}
%   t_K -t^\star \leq (\bar{\beta}/2) \log(2\{ -\diam(\M)^2/2 - 1/2 +(1 + \diam(\M)^2/2 +\diam(\M)^4/4)^{1/2}\}) \eqsp . 
% \end{equation}
\end{proof}

We now state the equivalent of \Cref{prop:wasserstein_forward}.

\begin{proposition}
    \label{prop:wasserstein_forward_improved}
    Assume \rref{assum:manifold_hyp}, \rref{assum:hessian_bound} and
    $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$. Then, for any
    $x, y \in \rset^d$ and $t \in \ccint{0,t_K}$
  \begin{equation}
    \textstyle{
      \wassersteinD[1](\updelta_x \Qker_{t}, \updelta_y \Qker_{t}) \leq  \exp[2(\Gamma+1)\bar{\beta}^2(1 + \log(1+\diam(\M)))]\sigma_{T-t_K}^{-2\Gamma} \normLigne{x-y} \eqsp .
      }
    \end{equation}    
  \end{proposition}

  \begin{proof}
    This is a direct consequence of \eqref{eq:pro_wasserstein},
    \Cref{prop:control_gradient_improved} and
    \eqref{eq:bound_tk_tstar_improved}.
  \end{proof}


  Finally, we control $\wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K})$. First, we have 
\begin{align}
\label{eq:convergence_bound_backward_inter_improved}  
  \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K}) &= \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T}  \Qker_{t_K}) \\
  &\leq \exp[2(\Gamma+1)\bar{\beta}^2(1 + \log(1+\diam(\M)))]\sigma_{T-t_K}^{-2\Gamma} \wassersteinD[1](\pi \Pker_T, \pi_\infty) \eqsp . 
\end{align}
To control $\wassersteinD[1](\pi \Pker_T, \pi_\infty)$, we use a
synchronous coupling, \ie we set $(\bfY_t, \bfZ_t)_{t \in \ccint{0,T}}$ such that
\begin{equation}
  \rmd \bfY_t = - \beta_t \bfY_t \rmd t + \sqrt{2 \beta_t} \rmd \bfB_t \eqsp , \qquad 
  \rmd \bfZ_t = - \beta_t \bfZ_t \rmd t + \sqrt{2 \beta_t} \rmd \bfB_t \eqsp ,
\end{equation}
where $(\bfB_t)_{t \in \ccint{0,T}}$ is a $d$-dimensional Brownian motion and
$\bfY_0 \sim \pi$, $\bfZ_0 \sim \pi_\infty$. We have that for any
$t \in \ccint{0,T}$, $\bfZ_t \sim \pi_\infty$. In addition, denoting
$u_t = \expeLigne{\normLigne{\bfY_t - \bfZ_t}}$ for any $t \in \ccint{0,T}$, we
have that
\begin{equation}
  \textstyle{\rmd u_t \leq u_0 \exp[-\int_0^t \beta_s \rmd s] \eqsp . }
\end{equation}
Therefore, combining this result and
\eqref{eq:convergence_bound_backward_inter_improved}, we get that
\begin{equation}
  \label{eq:convergence_bound_backward_improved}
  \textstyle{
    \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K}) \leq \exp[2(\Gamma+1)\bar{\beta}^2(1 + \log(1+\diam(\M)))]\sigma_{T-t_K}^{-2\Gamma} \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) \eqsp .
    }
  \end{equation}
Therefore, similarly as in the proof of \Cref{prop:discretization_bound_final}, we have
\begin{equation}
  \textstyle{
    \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K}) \leq \Dtt_1 \exp[-T/\bar{\beta}]/\vareps^{\Gamma} \eqsp , }
\end{equation}
with
\begin{equation}
  \Dtt_1 =  \exp[2(\Gamma+2)(1+\bar{\beta})^2(1 + \log(1+\diam(\M)))] (\sqrt{d} + \diam(\M)) \eqsp . 
\end{equation}
We conclude the proof of \Cref{thm:convergence_bound_hessian} upon combining
this result, \Cref{prop:discretization_bound_final_improved} and
\eqref{eq:control_noising}.

\subsection{Hessian bounds for the uniform distribution}
\label{sec:hess-bounds-unif}

The goal of this section is to prove the following result.

\begin{proposition}
  Assume that $\pi$ is the uniform distribution over $\ccint{-1/2, 1/2}^p$ for
  some $p \in \{1, \dots, d\}$. Then, there exists $\Gamma \geq 0$ such that for
  any $t \in \ocint{0,T}$ and $x \in \rset^d$,
  $\normLigne{\nabla^2 \log p_t(x_t)} \leq \Gamma / \sigma_t^2$.
\end{proposition}

\begin{proof}
  Let $t \in \ocint{0,T}$. We start by deriving a closed form expression for
  $p_t$. We have for any $x \in \rset^d$
  \begin{align}
    p_t(x) &= \textstyle{\int_{\M} \exp[-\normLigne{x-m_t z}^2/(2\sigma_t^2)]\rmd \pi(z)}(2\uppi \sigma_t)^{-d/2} \\
           &= \textstyle{\exp[-\sum_{i=p+1}^d x_i^2/(2\sigma_t^2)] \prod_{i=1}^p \int_{-1/2}^{1/2} \exp[-(x_i-m_t z_i)^2/(2\sigma_t^2)]\rmd z_i}(2\uppi \sigma_t)^{-d/2} \\
           &= \textstyle{\exp[-\sum_{i=p+1}^d x_i^2/(2\sigma_t^2)] \prod_{i=1}^p \int_{x_i-m_t/2}^{x_i + m_t/2} \exp[- z_i^2/(2\sigma_t^2)]\rmd z_i}(2\uppi \sigma_t)^{-d/2} m_t^{-p}   \\
           & = \textstyle{\exp[-\sum_{i=p+1}^d x_i^2/(2\sigma_t^2)] (2\uppi \sigma_t)^{-d/2}} \textstyle{\times \prod_{i=1}^p \int_{(x_i-m_t/2)/\sigma_t}^{(x_i + m_t/2)/\sigma_t} \exp[- z_i^2/2]\rmd z_i} (\sigma_t/m_t)^{p} \\ 
           & = (2\uppi)^{d/2} (2\uppi \sigma_t)^{-d/2} (\sigma_t/m_t)^{p} \textstyle{\prod_{i=p+1}^d \varphi(x_i /\sigma_t) } \\
    & \qquad \textstyle{\times \prod_{i=1}^p \{\Phi((x_i + m_t/2)/\sigma_t) - \Phi((x_i - m_t/2)/\sigma_t)\} }  \eqsp ,
  \end{align}
  where $\varphi(t) = \exp[-t^2/2]/\sqrt{2\uppi}$ and
  $\Phi(t) = \int_{-\infty}^t \varphi(s) \rmd s$. Note that from this
  expression, $\nabla^2 \log p_t$ is diagonal. Hence, we only need to compute
  $\partial_i^2 \log p_t(x)$ for any $x \in \rset^d$ and
  $i \in \{1, \dots, d\}$. Let $i \in \{p+1, \dots, d\}$. We have for any $x \in \rset^d$
  \begin{equation}
    \partial_i^2 \log p_t(x) = -\sigma_t^{-2} \eqsp .
  \end{equation}
  We now turn to the case where $i \in \{1, \dots, p\}$. In this case, we denote
  $F_t(\Phi, a, b) = \Phi(a + b) - \Phi(a - b) $ and we have
  \begin{equation}
    \label{eq:expression_hessienne}
    \partial_i^2 \log p_t(x) = (1/\sigma_t^2) \partial_2^2 \log F_t(\Phi, x_i/\sigma_t, m_t/\sigma_t) \eqsp . 
  \end{equation}
  We have that for any $a,b \in \rset$ with $a \neq b$
  \begin{equation}
    \label{eq:decomposition_der_second}
    \partial_2^2 \log F_t(\Phi, a, b) = F_t(\varphi', a, b)/F_t(\Phi, a, b) - F_t(\varphi, a, b)^2/F_t(\Phi, a, b)^2 \eqsp . 
  \end{equation}
  In what follows, we assume that $a >b$ and we define for any $t \in \rset$
  \begin{equation}
    \textstyle{\erfc(t) = 1 - (2/\sqrt{\uppi}) \int_0^t \exp[-s^2] \rmd s \eqsp . }
  \end{equation}
  Note that $F_t(\Phi, a, b) = (1/2)(\erfc((a-b)/2) - \erfc((a+b)/2))$. In addition, there exists $C > 0$ such that  for any $t \neq 0$ we have 
  \begin{equation}
    \erfc(t) \geq \exp[-t^2]/(\sqrt{\uppi}t) (1 + C/t^2) \eqsp , \qquad \erfc(t) \leq \exp[-t^2]/(\sqrt{\uppi}t) (1 - /(Ct^2)) \eqsp . 
  \end{equation}
  In particular, we have
  \begin{align}
    \label{eq:expansion_F_Phi}
    &\textstyle{F_t(\Phi, a, b) \leq  \exp[-(a-b)^2/2]/(\sqrt{2\uppi}(a-b)) (1 + R_0(a,b)) \eqsp , } \\
    &\textstyle{F_t(\Phi, a, b) \geq  \exp[-(a-b)^2/2]/(\sqrt{2\uppi}(a-b)) (1 - \bar{R_0}(a,b)) \eqsp , }
  \end{align}
  where
  \begin{align}
    R_0(a,b) &= C/(a-b)^2 + \exp[+(a-b)^2/2-(a+b)^2/2](a-b)/(a+b )(1 - /(C(a+b)^2)) \eqsp , \\
    \bar{R}_0(a,b) &= -C/(a-b)^2 + \exp[+(a-b)^2/2-(a+b)^2/2](a-b)/(a+b )(1 + C/(a+b)^2) \eqsp , \\
  \end{align}
  Note that there exists $C_0 \geq 0$ such that for any $a, b\in \rset$ with $a \geq b +1$
  \begin{equation}
    \label{eq:control_C0}
    (R_0(a,b) + \bar{R}_0(a,b))(a-b)^2 \leq C_0 \eqsp . 
  \end{equation}
  In particular, there exists $a_0 \geq 0$ such that if $a \geq b + a_0$, $\bar{R}_0(a,b) + R_0(a,b) \leq 1/2$.
  Similarly, we have
  \begin{equation}
    \label{eq:expansion_F_varphi}
    F_t(\varphi, a, b) = (2\uppi)^{-1/2} \exp[-(a-b)^2/2] (-1 + \exp[-((a+b)^2-(a-b)^2)/2]) \eqsp . 
  \end{equation}
  We denote $R_1(a,b) = \exp[-((a+b)^2-(a-b)^2)/2]$ and note that there exists
  $C_1 \geq 0$ such that for any $a, b\in \rset$ with $a \geq b +1$
  \begin{equation}
    \label{eq:control_C1}
    R_1(a,b)(a-b)^2 \leq C_1 \eqsp . 
  \end{equation}
  Finally, we have
  \begin{equation}
    \label{eq:expansion_F_varphi_prime}
    F_t(\varphi', a, b) = (2\uppi)^{-1/2} \exp[-(a-b)^2/2](a-b) (1 + (a+b)/(a-b)\exp[-((a+b)^2-(a-b)^2)/2]) \eqsp . 
  \end{equation}
  We denote $R_2(a,b) = (a+b)/(a-b) \exp[-((a+b)^2-(a-b)^2)/2]$ and note that there exists
  $C_2 \geq 0$ such that for any $a, b\in \rset$ with $a \geq b +1$
  \begin{equation}
    \label{eq:control_C2}
    R_2(a,b)(a-b)^2 \leq C_2 \eqsp . 
  \end{equation}
  Combining \eqref{eq:decomposition_der_second}, \eqref{eq:expansion_F_Phi},
  \eqref{eq:expansion_F_varphi} and \eqref{eq:expansion_F_varphi_prime}, we get
  that for any $a, b \in \rset$ with $a \geq b + 1$
  \begin{equation}
    \partial_2^2 \log F_t(\Phi, a, b) \leq (a-b)^2 [(1+R_2(a,b))/(1+\bar{R}_0(a,b)) - (1+R_1(a,b))^2/(1+R_0(a,b))^2] \eqsp . 
  \end{equation}
  In addition, we have for any $a, b \in \rset$ with $a \geq b + 1$
  \begin{align}
    &(1+R_2(a,b))/(1+\bar{R}_0(a,b)) - (1+R_1(a,b))^2/(1+R_0(a,b))^2 \\ &\qquad = (R_2(a,b)(1 +R_0(a,b))^2 -R_1(a,b)(1+\bar{R_0}(a,b) )) /[(1+\bar{R}_0(a,b))^2(1+\bar{R}_0(a,b))] \eqsp . 
  \end{align}
  Combining this result, \eqref{eq:control_C0}, \eqref{eq:control_C1} and
  \eqref{eq:control_C2}, we get that for any $a, b \in \rset$ with
  $a \geq b + a_0$
  \begin{equation}
    R_2(a,b)(1 +R_0(a,b))^2 -R_1(a,b)(1+\bar{R_0}(a,b) \leq 4(C_1 + C_2)/(a-b)^2 \eqsp . 
  \end{equation}
  Therefore, there exists $C_3 \geq 0$ such that for any $a \geq b +a_0$,
  $\absLigne{\partial_2^2 \log F_t(\Phi,a,b)} \leq C_3$. Similarly there exists
  $C_4 \geq 0$ such that if $a \leq - b -a_0$,
  $\absLigne{\partial_2^2 \log F_t(\Phi,a,b)} \leq C_4$. By symmetry, there
  exists $C_5 \geq 0$ such that for any $b \geq a + a_0$ or $-b \geq -a - a_0$,
  we have $\absLigne{\partial_2^2 \log F_t(\Phi,a,b)} \leq C_5$ and we conclude
  by continuity that there exists $C \geq 0$ such that for any $a, b \in \rset$,
  \begin{equation}
    \partial_2 \log F_t(\Phi, a, b) \leq C \eqsp ,
  \end{equation}
  which concludes the proof upon combining this result with \eqref{eq:expression_hessienne}.
\end{proof}

\subsection{The role of convexity}
\label{sec:non-conv-count}


In this section, for any $x \in \rset^d$, we define $f_x : \M \to \rset_+$ given
for any $y \in \M$ by $f_x(y) = \normLigne{x - y}^2$. Before giving our main
result we need to introduce a few useful tools.

For any subset $\msx \subset \rset^d$ and $x \in \rset^d$
we define $\rmP(x) = \ensembleLigne{y \in \msx}{d(x,\msx) = d(x,y)}$. Note that
$\rmP(x)$ can be empty. We say that a set $\msx$ is \emph{Chebyshev} if for all
$x \in \rset^d$, there exists $p(x) \in \msx$ such that $\rmP(x) = \{p(x)\}$,
\ie Chebyshev sets are the subsets of $\rset^d$ such that each point admits a
unique projection on $\msx$. It is clear that all closed and convex sets are
Chebyshev sets. Note that all Chebyshev sets are closed since for any Chebyshev
set $\msx$ and $x \in \partial \msx$ (the frontier of $\msx$) we have that there
exists $p(x) \in \msx$ such that $d(x,p(x)) = d(x, \msx) = 0$, \ie 
$x \in \msx$. In addition, Chebyshev sets are also convex, see
\citep{kritikos1938quelques,motzkin1935quelques,bundt1934chebyshev}. This result
implies the following proposition.

\begin{proposition}
  \label{prop:chebyshev_convex}
  Let $\msx \subset \rset^d$. $\msx$ is a closed convex set if and only if
  $\msx$ is a Chebyshev set.
\end{proposition}

In order to prove our main result, we introduce some basics on \emph{Morse
  theory}. Assume that $\M$ is a smooth manifold and
$f \in \rmc^\infty(\M, \rset)$. We say that $x\in \M$ is a non-degenerate
minimizer if $x \in \M$ is a minimizer of $f$ and the Hessian of $f$ at $x$ is
not singular. We then have the following proposition (see
\citep{matsumoto2002introduction} for instance).

\begin{proposition}
  \label{prop:morse}
  Let $f \in \rmc^\infty(\M, \rset)$ and $x \in \M$ a non degenerate minimizer
  of $f$. Then there exist $\msu \subset \M$ open and
  $\varphi: \msu \to \varphi(\msu) \subset \rset^p$ a local chart such that
  $\varphi(x) = 0$ and for any $\hat{y} \in \varphi(\msu)$
  \begin{equation}
    \textstyle{f(\varphi^{-1}(\hat{y})) = f(x) + \normLigne{\hat{y}}^2 \eqsp . }
  \end{equation}
  In addition, we have $\rmD \varphi(x) = \nabla^2 f(x)$.
\end{proposition}

Note that upon considering $\varphi^{-1}(\varphi(\msu)/2)$ instead of $\msu$ we
can always assume that $\varphi^{-1}$ has bounded derivatives.

Finally, we introduce the concept of \emph{shape operator} (also called
\emph{second fundamental form} or \emph{Weingarten form}), see
\citep{bishop2011geometry}. We assume that the metric on $\M$ is the induced
Euclidean metric. Let
$N \in \Gamma(\mathrm{T} \M^\top)$ a section on the normal bundle
$\mathrm{T} \M^\top$. We define
$\mathfrak{A}^N: \Gamma(\mathrm{T} \M)^2 \to \rmc^\infty(\M)$ such that for any
$V_1, V_2 \in \Gamma(\mathrm{T} \M)$
\begin{equation}
  \mathfrak{A}^N(V_1, V_2) = -\langle V_1, \nabla_{V_2} N \rangle \eqsp .
\end{equation}
Note that $\mathfrak{A}^N$ is symmetric, linear and the scalar product and
covariant derivative $\nabla$ are considered \wrt the ambient Euclidean metric. The shape
operator encodes the local geometry of $\M$. For example in the case of
$\mathbb{S}^{d-1}$, we have that for any $N \in \Gamma(\mathrm{T} \M^\top)$ and
$V_1, V_2 \in \Gamma(\mathrm{T} \M)$
\begin{equation}
  \label{eq:shape_operator_sphere}
  \mathfrak{A}^N(V_1, V_2) = - \langle V_1, V_2 \rangle \langle N_0, N\rangle \eqsp,
\end{equation}
where $N_0$ is the normal vector field pointing outward of the sphere, see
\citep{absil2013extrinsic}.  We have the following result, see \cite[Theorem
3]{bishop2011geometry} and \citep{bishop1974infinitesimal}.

\begin{proposition}
  If $\M$ is convex then for any $N \in \Gamma(\mathrm{T} \M^\top)$ such that
  for any $x, y \in \M$, $\langle y - x, N(x) \rangle \geq 0$, $\mathfrak{A}^N$
  is non-negative.
\end{proposition}

Finally, let $\bar{f} \in \rmc^\infty(\rset^d, \rset)$ and $f$ its restriction
to $\M$. Using \citep{absil2013extrinsic}, we have for any
$V_1, V_2 \in \Gamma(\mathrm{T} \M)$
\begin{equation}
  \label{eq:hessian_formula}
  \nabla^2 f(V_1, V_2) = \langle V_1, \Pi(\nabla^2 \bar{f}(V_2)) \rangle + \mathfrak{A}^{\Pi^\top(\nabla \bar{f})}(V_1, V_2) \eqsp ,
\end{equation}
where for any $x\in \M$, $\Pi_x$ is the orthogonal projection operator on
$\mathrm{T}_x\M$. We are now ready to state our main result.

\begin{theorem}
  \label{prop:non-convex-sets}
  Assume that $\M \subset \rset^d$ is a smooth manifold and that $\pi$ admits a
  smooth density \wrt the Hausdorff measure on $\M$. The following hold:
  \begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label=(\alph*)]
  \item \label{item:convex} If $\M$ is convex then for any $x \in \M$ we have $\limsup_{t \to 0} \sigma_t^2 \normLigne{\nabla^2 \log p_t(m_t x)} < +\infty$.     
  \item \label{item:non-convex} If there exists $x \in \rset^d$ such that
    $\absLigne{\rmP(x)} > 1$ and for any $p(x) \in \rmP(x)$,
    $\mathfrak{A}^{p(x) - x}_{p(x)} \succ -\Id$. Then, we have
    $\liminf_{t \to 0} \sigma_t^4 \normLigne{\nabla^2 \log p_t(m_t x)} > 0$.
  \end{enumerate}
\end{theorem}

\Cref{prop:non-convex-sets} implies that one can obtain information about the
geometry of $\M$ by computing the Hessian of the logarithmic gradient of the
densities of $(\mathcal{L}(\bfX_t))_{t \in \ccint{0,T}}$. In the convex case the scaling
\wrt $\sigma_t$ is of order $\sigma_t^{-2}$ whereas in the second scenario
the scaling is of order $\sigma_t^{-4}$. Note that the condition ``there exists
$x \in \rset^d$ such that $\absLigne{\rmP(x)} > 1$'' is equivalent to assuming
that $\M$ is not a Chebyshev set and hence a non convex set in virtue of
\Cref{prop:chebyshev_convex}. Therefore in
\Cref{prop:non-convex-sets}-\ref{item:non-convex}, we assume that $\M$ is non
convex and a curvature condition. The condition
$\mathfrak{A}^{p(x) - x}_x \succ -\Id$ implies that the manifold is not too
``negatively curved'' at the projection points.  The non-strict inequality is
always true, \ie for any $p(x) \in \rmP(x)$, $\mathfrak{A}^{p(x) - x}_x \succeq -\Id$
since $\nabla^2 f^x(p(x)) \succeq 0$. % Finally, we note that if $\M$ is non
% convex there exists $y \in \M$, $N \in \Gamma(\mathrm{T} \M^\top)$ and
% $V \in \Gamma(\mathrm{T}\M)$ such that $\mathfrak{A}_y^N(V,V) < 0$, see
% \cite{bishop1974infinitesimal}.

We conjecture that this curvature condition can be relaxed. Indeed, it is not
satisfied in the case where
$\M = \ensembleLigne{x \in \rset^d}{\normLigne{x}=1}$, since the only point
$x \in \rset^d$ such that $\absLigne{\rmP(x)} > 1$ is $x=0$ and in that case
$\rmP(x) = \M$ and therefore $\nabla^2 f^0 = 0$, which implies that for any
$x \in \M$, $\mathfrak{A}_{x}^{x} = -\Id$. This formula could also have been
obtained from \eqref{eq:shape_operator_sphere}. However, one can show that we
still have $\liminf_{t \to 0} \sigma_t^4 \normLigne{\nabla^2 \log p_t(0)} >
0$. In future works, we would like to relax these curvature conditions assuming
that the manifold has an analytic structure and using results from
\citep{combet2006integrales}.


Finally, we highlight that \Cref{prop:non-convex-sets}-\ref{item:convex} is
weaker than the condition \Cref{assum:hessian_bound}. To bridge the gap between
\Cref{prop:non-convex-sets}-\ref{item:convex} and \Cref{assum:hessian_bound} one
would need to strengthen \Cref{prop:non-convex-sets}-\ref{item:convex} to derive
\emph{uniform in space} bounds. This would require to use \emph{quantitative}
version of the Morse lemmas, see \citep{le2014numerical} for instance. We
postpone this study to future works. However,
\Cref{prop:non-convex-sets}-\ref{item:non-convex} implies that
\Cref{assum:hessian_bound} does not hold. Hence, any non convex set which is not
too ``negatively curved'' does not satisfy \Cref{assum:hessian_bound}.

% Pour comprendre le comportement asymptotique à
% haute fréquence d'intégrales exponentielles, il est nécessaire de faire appel à des théories
% mathématiques diverses (théorie des singularités, théorie des variétés lagrangiennes, etc.)
% HOMMAGE A EDMOND COMBET 17
% qui ne sont pas a priori présentes dans le problème. Il


\begin{proof}
  \begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label=(\alph*)]  
  \item First, we assume that $\M$ is convex. We show that for any
    $x \in \rset^d$ and $p(x) \in \mathrm{P}(x)$, $\nabla^2f^x(p(x)) \succ 0$,
    \ie the Hessian of $f^x$ is not degenerate. For any $x \in \rset^d$, we define
    $\bar{f}^x$ such that for any $y \in \rset^d$,
    $\bar{f}^x(y) = \normLigne{x-y}^2$. Using
    \eqref{eq:hessian_formula}, we have for any $x \in \rset^d$
    \begin{equation}
      \label{eq:hessian_invertible}
      \nabla^2 f^x(p(x)) = \Id + \mathfrak{A}^{p(x) - x} \succeq \Id \succ 0 \eqsp . 
    \end{equation}
    Since $\M$ is convex for any $x\in \rset^d$, $\rmP(x) = \{p(x)\}$ and note
    that $\rmP(x)$ is the set of minimizers of $f^x$. Let $x \in \rset^d$. Using
    \Cref{prop:morse} and \eqref{eq:hessian_invertible}, there exist $\msu \subset \M$ open and
    $\varphi: \msu \to \varphi(\msu) \subset \rset^p$ a local chart such that
    $\varphi(p(x)) = 0$ and for any $\hat{y} \in \varphi(\msu)$
    \begin{equation}
      \label{eq:changement_variable}
    \textstyle{\normLigne{x - \varphi^{-1}(\hat{y})}^2 = \normLigne{x - p(x)}^2 + \normLigne{\hat{y}}^2 \eqsp , }
  \end{equation}
  with $\varphi^{-1}(0) = p(x)$. Note that
  $\rmD \varphi^{-1}(0) = (\nabla^2 f^x(p(x)))^{-1}$. For any
  $t \in \ocint{0,T}$, denote $\lambda_t = m_t / \sigma_t$. Using
  \eqref{eq:changement_variable}, we have that
  \begin{align}
    &\textstyle{\int_{\msu^2} (y_0 - y_1)^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{x - y_1}^2/2] \rmd \pi(y_0) \rmd \pi(y_1)} \\
    &\textstyle{=\int_{\varphi^{-1}(\msu)^2} (\varphi^{-1}(\hat{y}_0) - \varphi^{-1}(\hat{y}_1))^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{\hat{y}_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{\hat{y}_1}^2/2] \rmd \hat{\pi}(\hat{y}_0) \rmd \hat{\pi}_1(\hat{y}_1)} \\
    & \qquad \times \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \\
    &\textstyle{=(1/\lambda_t)^{2p}\int_{\lambda_t \varphi^{-1}(\msu)^2} (\varphi^{-1}(\hat{y}_0/\lambda_t) - \varphi^{-1}(\hat{y}_1/\lambda_t))^{\otimes 2} \exp[-\normLigne{\hat{y}_0}^2/2]\exp[-\normLigne{\hat{y}_1}^2/2] \rmd \hat{\pi}(\hat{y}_0) \rmd \hat{\pi}_1(\hat{y}_1)} \\ 
      & \qquad \times \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \eqsp ,
  \end{align}
  where $\hat{\pi} = \varphi_{\#} \pi$ admits a positive density \wrt the
  Lebesgue measure.  Therefore, there exists $C_0 \geq 0$ such that for any
  $t \in \ocint{0,T}$
  \begin{align}
    &(2 \uppi/\lambda_t^2)^{-p}\normLigne{\textstyle{\int_{\msu^2} (y_0 - y_1)^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{x - y_1}^2/2] \rmd \pi(y_0) \rmd \pi(y_1)}} \\
    &\qquad \textstyle{\leq C_0 (2 \uppi)^{-p} \sigma_t^2 \int_{(\rset^p)^2} \normLigne{\hat{y}_0 - \hat{y}_1}^2  \exp[-\normLigne{\hat{y}_0}^2/2]\exp[-\normLigne{\hat{y}_1}^2/2] \rmd \hat{y}_0 \rmd \hat{y}_1}  \\
    &\qquad  \qquad \times \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \\
    &\qquad \leq 2C_0 p \sigma_t^2 \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \eqsp , \label{eq:inside_bound_convex}
  \end{align}
  where we have used that
  $\norm{a-b}^2 \leq 2(\normLigne{a}^2 + \normLigne{b}^2)$ for any
  $a, b \in \rset^p$ in the last line.  In addition, since $\msu$ is open we
  have that $\M \cap \msu^\complementary$ is compact and since for any
  $y \in \M \cap \msu^\complementary$,
  $\normLigne{y - x}^2 > \normLigne{p(x) - x}^2$, there exists $\vareps >0$ such
  that for any $y \in \M \cap \msu^\complementary$,
  $\normLigne{y - x}^2 \geq \normLigne{p(x) - x}^2 + \vareps$. Therefore, we
  have
  \begin{align}
    &\normLigne{\textstyle{\int_{(\M \cap \msu^\complementary)^2} (y_0 - y_1)^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{x - y_1}^2/2] \rmd \pi(y_0) \rmd \pi(y_1)}} \\
    &\qquad \leq \diam(\M)^2 \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \exp[-\vareps (m_t/\sigma_t)^2] \eqsp .  \label{eq:outside_bound_convex}
  \end{align}
  Combining \eqref{eq:inside_bound_convex} and \eqref{eq:outside_bound_convex}
  there exists $C_1 \geq 0$ such that for any $t \in \ocint{0,T}$
  \begin{align}
    &(2 \uppi/\lambda_t^2)^{-p}\normLigne{\textstyle{\int_{\M^2} (y_0 - y_1)^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{x - y_1}^2/2] \rmd \pi(y_0) \rmd \pi(y_1)}} \\
    & \qquad \qquad \leq C_1 \sigma_t^2 \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \eqsp . \label{eq:upper_bound_convex}
  \end{align}
  In addition, there exists $C_2 > 0$ such that for any $t \in \ocint{0,T}$
  \begin{align}
    (2 \uppi/\lambda_t^2)^{-p}\textstyle{\int_{\msu} \exp[-(m_t/\sigma_t)^2\normLigne{x - y}^2/2] \rmd \pi(y)} \geq (1/C_2) \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \eqsp . \label{eq:lower_bound_convex}
  \end{align}
  Therefore, combining \eqref{eq:upper_bound_convex} and
  \eqref{eq:lower_bound_convex}, we get that there exists $C_3 \geq 0$ such that
  for any $t \in \ocint{0,T}$
  \begin{align}
    &\normLigne{\textstyle{\int_{\M} (y_0 - y_1)^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{x - y_1}^2/2] \rmd \pi(y_0) \rmd \pi(y_1)}} \\
    & \qquad \qquad  \textstyle{/ (\int_{\M} \exp[-(m_t/\sigma_t)^2\normLigne{x - y}^2/2] \rmd \pi(y))^2 } \leq C_3 \sigma_t^2 \eqsp .
  \end{align}
  We conclude the proof in the convex case upon combining this result and  \Cref{lemma:control_hessian}.
\item Second, we assume that there exists $x \in \rset^d$ such that
  $\absLigne{\rmP(x)} > 1$ and for any $p(x) \in \rmP(x)$,
  $\mathfrak{A}^{p(x) - x} \succ -\Id$. Using \eqref{eq:hessian_formula}, we
  have for any $p(x) \in \rmP(x)$
    \begin{equation}
      \nabla^2 f^x(p(x)) = \Id + \mathfrak{A}^{p(x) - x}  \succ 0 \eqsp . 
    \end{equation}
    Using this fact and that $\rmP(x)$ is the set of minimizers of $f^x$ and is
    compact, we get that $\absLigne{\rmP(x)} < +\infty$. Hence, we assume that
    $\rmP(x) = \{p_i(x)\}_{i=1}^N$ with $N > 1$. Using \Cref{prop:morse}, for
    any $i \in \{1, \dots, N\}$, there exist $\msu_i \subset \M$ open and
    $\varphi_i: \msu_i \to \varphi_i(\msu_i) \subset \rset^p$ a local chart such that
    $\varphi_i(p_i(x)) = 0$ and for any $\hat{y} \in \varphi_i(\msu_i)$
  \begin{equation}
    \textstyle{\normLigne{x - \varphi_i^{-1}(\hat{y})}^2 = \normLigne{x - p_i(x)}^2 + \normLigne{\hat{y}}^2 \eqsp , }
  \end{equation}
  with $\varphi_i^{-1}(0) = p_i(x)$. Note that
  $\rmD \varphi_i^{-1}(0) = (\nabla^2 f^x(p_i(x)))^{-1}$. Without loss of
  generality we assume that for any $i, j \in \{1, \dots, N\}$,
  $\msu_i \cap \msu_j = \emptyset$.
  We have that
  \begin{align}
    &\textstyle{\int_{\msu_0 \times \msu_1} (y_0 - y_1)^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{x - y_1}^2/2] \rmd \pi(y_0) \rmd \pi(y_1)} \\
    &\textstyle{=\int_{\varphi_0^{-1}(\msu_0) \times \varphi_1^{-1}(\msu_1)} (\varphi_0^{-1}(\hat{y}_0) - \varphi_1^{-1}(\hat{y}_1))^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{\hat{y}_0}^2/2]}\\
    & \qquad \times \exp[-(m_t/\sigma_t)^2\normLigne{\hat{y}_1}^2/2] \rmd \hat{\pi}(\hat{y}_0) \rmd \hat{\pi}_1(\hat{y}_1) \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \\
    &\textstyle{=(1/\lambda_t)^{2p}\int_{\lambda_t \varphi_0^{-1}(\msu_0) \times \lambda_t \varphi_1^{-1}(\msu_1)} (\varphi_0^{-1}(\hat{y}_0/\lambda_t) - \varphi_1^{-1}(\hat{y}_1/\lambda_t))^{\otimes 2}} \\
    & \qquad \times \exp[-\normLigne{\hat{y}_0}^2/2]\exp[-\normLigne{\hat{y}_1}^2/2] \rmd \hat{\pi}(\hat{y}_0) \rmd \hat{\pi}_1(\hat{y}_1)  \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \eqsp . \label{eq:u0_u1_nonconvex}
  \end{align}
  In addition, using the dominated convergence theorem we have
  \begin{align}
    \label{eq:u0_u1_limit}
    &\lim_{t \to +\infty} \textstyle{(2\uppi)^{-p} \int_{\lambda_t \varphi_0^{-1}(\msu_0) \times \lambda_t \varphi_1^{-1}(\msu_1)} (\varphi_0^{-1}(\hat{y}_0/\lambda_t) - \varphi_1^{-1}(\hat{y}_1/\lambda_t))^{\otimes 2}} \\
    & \qquad \qquad \times \exp[-\normLigne{\hat{y}_0}^2/2]\exp[-\normLigne{\hat{y}_1}^2/2] \rmd \hat{\pi}(\hat{y}_0) \rmd \hat{\pi}_1(\hat{y}_1) = \hat{h}_0(p_0(x)) \hat{h}_1(p_1(x)) (p_0(x) - p_1(x))^{\otimes 2} \eqsp , 
  \end{align}
  where $\hat{h}_i$ is the density of $\hat{\pi}_i = (\varphi_i)_{\#} \pi$ \wrt the
  Lebesgue measure.  In addition, there exists $C_4 \geq 0$ such that for any
  $t \in \ocint{0,T}$
  \begin{align}
    &\textstyle{(2\uppi)^{-p/2} \int_{\msu_0} \exp[-(m_t / \sigma_t)^2\normLigne{x - y_0}^2/2] \rmd \pi(y_0)} \\
    & \qquad \qquad = \textstyle{(2\uppi)^{-p/2} \int_{\varphi_0^{-1}(\msu_0)} \exp[-(m_t / \sigma_t)^2\normLigne{\hat{y}_0}^2/2] \rmd \hat{\pi}(\hat{y}_0)} \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \\
    & \qquad \qquad \leq C_4 \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2] \lambda_t^{p/2} \eqsp . \label{eq:upper_bound_non_cvx}
  \end{align}
In addition, since $\msu_0$ is open we
  have that $\M \cap \msu_0^\complementary$ is compact and since for any
  $y \in \M \cap \msu_0^\complementary$,
  $\normLigne{y - x}^2 > \normLigne{p(x) - x}^2$, there exists $\vareps >0$ such
  that for any $y \in \M \cap \msu_0^\complementary$,
  $\normLigne{y - x}^2 \geq \normLigne{p(x) - x}^2 + \vareps$. Therefore, we
  have
  \begin{align}
    \textstyle{\int_{\M \cap \msu_0^\complementary} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2] \rmd \pi(y_0)}  \leq C_5 \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2/2] \exp[-\vareps (m_t/\sigma_t)^2] \eqsp .  \label{eq:outside_bound_non_convex}
  \end{align}
  Combining this result and \eqref{eq:upper_bound_non_cvx}, we get that there exists $C_6 > 0$ such that
  \begin{equation}
    (2 \uppi/\lambda_t^2)^{-p/2} \textstyle{\int_{\M} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2] \rmd \pi(y_0)} \leq C_6 \exp[-(m_t/\sigma_t)^2\normLigne{x-p(x)}^2/2] \eqsp . 
  \end{equation}
  Combining this result, \eqref{eq:u0_u1_nonconvex} and \eqref{eq:u0_u1_limit}, there exists $C_7 > 0$ such that
    \begin{align}
    &\liminf_{t \to 0} \textstyle{\int_{\M} (y_0 - y_1)^{\otimes 2} \exp[-(m_t/\sigma_t)^2\normLigne{x - y_0}^2/2]\exp[-(m_t/\sigma_t)^2\normLigne{x - y_1}^2/2] \rmd \pi(y_0) \rmd \pi(y_1)} \\
    & \qquad \qquad  \textstyle{/ (\int_{\M} \exp[-(m_t/\sigma_t)^2\normLigne{x - y}^2/2] \rmd \pi(y))^2 } \geq (x_0 - x_1)^{\otimes 2} / C_6 \eqsp .
  \end{align}
  We conclude upon combining this result and \Cref{lemma:control_hessian}.
  \end{enumerate}
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Diffusion modeling, also called score-based generative modeling, is a new
paradigm for generative modeling which exhibits state-of-the-art performance in
image and audio synthesis  
\citep{song2019generative,song2020score,ho2020denoising,nichol2021improved,nichol2021beatgans}. Such
models first consider a forward stochastic process, adding noise to the data until a
Gaussian distribution is reached. The model then approximates the
backward process associated with this forward noising process. It can be shown,
see \citep{haussmann1986time} for instance, that in order to compute the drift
of the backward trajectory, the gradient of the forward logarithmic density
(Stein score) must be estimated. Such an estimator is then obtained using score
matching techniques \citep{hyvarinen2005estimation,vincent2011connection} and
leveraging neural network techniques. At sampling time, the backward process is initialized
with a Gaussian and run backward in time using the approximation of the Stein
score. Despite impressive empirical results, theoretical understanding and convergence analysis of diffusion models remain limited. \citet{debortoli2021diffusion} establish the convergence of diffusion
models in total variation under the assumption that the target distribution
admits a density \wrt the Lebesgue measure and under dissipativity
conditions. More recently \citet{lee2022convergence}  obtained convergence
results for diffusion models, including predictor-corrector schemes,
under the assumption that the target distribution admits a density \wrt the
Lebesgue measure and satisfies a log-Sobolev inequality.

However, these works implicitly assume that the score does not explode as
$t \to 0$, by imposing that the score of the data distribution is Lipschitz
continuous or satisfies some growth property. This is not observed in practice and experimentally the norm of the score blows up when $t \to 0$, see
\citep{kim2021soft} for instance. Indeed, the assumptions that the target
distribution admits a density \wrt the Lebesgue measure and has a Lipschitz
logarithmic gradient does not hold if one assumes the \emph{manifold hypothesis}
\citep{tenenbaum2000global,fefferman2016testing,goodfellow2016deep} or if the
target measure is an empirical measure. In this setting, the target distribution
is supported on a lower dimensional compact set.  In the case of image
processing, this hypothesis is supported by empirical evidence
\citep{weinberger2006unsupervised,fefferman2016testing}.  Under this hypothesis,
even though the forward process admits a density for all $t >0$ its logarithmic
gradient explodes for small $t \rightarrow 0$. Consequently, previous
theoretical analyses of diffusion models do not apply to this setting. To our
knowledge, \citep{pidstrigach2022score} is the only existing work investigating
the convergence of diffusion models under such manifold assumptions by showing
that the limit of the continuous backward process with approximate score is
well-defined and that its distribution is equivalent to the one of the target
distribution under integrability conditions on the error of the score. In
particular, \cite{pidstrigach2022score} show that these distributions have the same
support.

In this work, we go one step further and study the convergence rate of diffusion
models under the manifold hypothesis. More precisely, we derive quantitative
convergence bounds in Wasserstein distance of order one between the target
distribution and the generative distribution of the diffusion model. The rest of the
paper is organized as follows. In \Cref{sec:diff-models-gener}, we recall the
basics of diffusion models. We present our main results and discuss links
with the existing literature in \Cref{sec:main-results}. The rest of the paper
is dedicated to the proof of \Cref{thm:convergence_general} in
\Cref{sec:proof_theorem_one}. We conclude and explore future avenues in
\Cref{sec:conclusion}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/main_results.tex <==
\section{Diffusion models for generative modeling }
\label{sec:diff-models-gener}

In this section, we recall the basics of diffusion models.
Henceforth, let $\pi \in \Pens(\rset^d)$ denote the target distribution, also known as the data distribution, and $\pi_\infty = \mathrm{N}(0, \Id)$ the $d$-dimensional Gaussian distribution with zero mean and identity covariance matrix. In what follows, we consider the forward noising process
$(\bfX_t)_{t \in \ccint{0,T}}$ given by an Ornstein--Ulhenbeck\footnote{Also
  called Variance Preserving Stochastic Differential Equation (VPSDE) in
  \cite{song2020score}.} process as follows
\begin{equation}
  \label{eq:ornstein_ulhenbeck}
  \rmd \bfX_t = - \beta_t \bfX_t \rmd t + \sqrt{2 \beta_t} \rmd \bfB_t \eqsp , \qquad \bfX_0 \sim \pi \eqsp . 
\end{equation}
where $(\bfB_t)_{t \geq 0}$ is a $d$-dimensional Brownian motion and
$t \mapsto \beta_t$ is an non-decreasing weighting function. In practice,
setting $\beta_0 \leq \beta_T$ allows for better control of the backward
diffusion near the target distribution, see \citep{nichol2021improved,song2020score} for instance. In what
follows, we assume that \eqref{eq:ornstein_ulhenbeck} admits a strong
solution. Under mild assumptions on the target distribution
\citep{haussmann1986time,cattiaux2021time}, the backward process
$(\bfY_t)_{t \in \ccint{0,T}} = (\bfX_{T-t})_{t \in \ccint{0,T}}$ satisfies
\begin{equation}
  \label{eq:time_reversal_sde}
  \textstyle{
    \rmd \bfY_t = \beta_{T-t} \{\bfY_t + 2 \nabla \log p_{T-t}(\bfY_t) \} \rmd t + \sqrt{2 \beta_{T-t}} \rmd \bfB_t \eqsp ,
    }
  \end{equation}
  where $\{p_t\}_{t \in \ocint{0,T}}$ the family of densities of
  $\{\mathcal{L}(\bfX_t)\}_{t \in \ocint{0,T}}$ \footnote{For any
    $\rset^d$-valued random variable $X$, $\mathcal{L}(X)$ is the distribution
    of $X$.} \wrt the Lebesgue measure. Note that in order to define
  \eqref{eq:time_reversal_sde} we do not need to assume that $\pi$ admits a
  density \wrt the Lebesgue measure. In practice, instead of sampling from
  $\bfY_0 \sim \mathcal{L}(\bfX_T)$ we sample from
  $\bfY_0 \sim \pi_\infty = \mathrm{N}(0, \Id)$. For large $T >0$ the mismatch
  between the distribution of $\bfX_T$ and $\pi_\infty$ is small due to
  geometric convergence of the Ornstein--Ulhenbeck process.

  In practice, $\{\nabla \log p_t\}_{t \in \ccint{0,T}}$ cannot be computed
  exactly and is approximated by a family of estimators
  $\{\bm{s}(t, \cdot)\}_{t \in \ccint{0,T}}$. Those estimators minimize
  the denoising score matching loss function $\ell$ given by
  \begin{equation}
    \label{eq:dsm_loss}
    \textstyle{
      \ell(\bm{s}) = \int_0^T \kappa(t) \expeLigne{\normLigne{\bm{s}(t, \bfX_t) - \nabla \log p_{t|0}(\bfX_t|\bfX_0)}^2} \rmd t \eqsp ,
      }
    \end{equation}
    with $p_{t|0}$ is the density of $\bfX_t$ given $\bfX_0$, \ie the density of
    the transition kernel associated with \eqref{eq:ornstein_ulhenbeck} and
    $\kappa: \ \ccint{0,T} \to \rset_+$ is a weighting function. In practice,
    \eqref{eq:dsm_loss} is approximated using Monte Carlo samples and the loss
    function is minimized over the parameters of a neural network.

    Once the score estimator $\bm{s}$ is learned, we introduce a continuous-time
    backward process $(\hat{\bfY}_t)_{t \in \ccint{0,T}}$ approximating
    $(\bfY_t)_{t \in \ccint{0,T}}$ and given by
    \begin{equation}
      \label{eq:approximate_time_reversal_continuous}
  \textstyle{
    \rmd \hat{\bfY}_t = \beta_{T-t} \{\hat{\bfY}_t + 2 \bm{s}(T-t, \hat{\bfY}_t) \} \rmd t + \sqrt{2 \beta_{T-t}} \rmd \bfB_t \eqsp , \qquad \hat{\bfY}_0 \sim \pi_\infty = \mathrm{N}(0, \Id) \eqsp . 
    }
  \end{equation}
  In practice, one needs to discretize
  \eqref{eq:approximate_time_reversal_continuous} in order to define an
  algorithm which can be implemented. We consider a sequence of stepsizes
  $\{\gamma_k\}_{k \in \{0, \dots, K\}}$ such that
  $\sum_{k=0}^{K} \gamma_k = T$. In what follows, for any
  $k \in \{0, \dots, K\}$ we denote $t_{k+1} = \sum_{j=0}^k \gamma_j$ and
  $t_0 =0$\footnote{Note that $t_{K+1} = T$.}.  Given this sequence of stepsizes,
  we consider the interpolation process $(\bbfY_t)_{t\in \ccint{0,T}}$ defined
  for any $k \in \{0, \dots, K\}$ and $t \in \ccint{t_k, t_{k+1}}$ by
\begin{equation}
  \label{eq:OU_disc}
  \textstyle{
    \rmd \bbfY_t = \beta_{T-t} \{ \bbfY_{t} + 2 \bm{s}(T-t_k, \bbfY_{t_k}) \} \rmd t + \sqrt{2\beta_{T-t}} \rmd \bfB_t \eqsp , \qquad \bbfY_0 \sim \pi_\infty \eqsp .
    }
  \end{equation}
  This process is an Ornstein--Ulhenbeck process on
  the interval $\ccint{t_k, t_{k+1}}$.  Denoting
  $(Y_k)_{k \in \{0, \dots, K+1\}}$ such that for any $k \in \{0, \dots, K+1\}$,
  $Y_k = \bbfY_{t_k}$, we have for any $k \in \{0, \dots, K\}$
  \begin{align}
    \label{eq:discretization_improved}
      Y_{k+1} &=     \textstyle{Y_k + \gamma_{1,k} (Y_{k} + 2 \bm{s}(T-t_k, Y_{k})) + \sqrt{2 \gamma_{2,k}} Z_k \eqsp ,
                } \\
    \gamma_{1,k} &= \textstyle{\exp[\int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1 \eqsp , \qquad \gamma_{2,k} = (\exp[2 \int_{T-t_{k+1}}^{T-t_k} \beta_s \rmd s] - 1)/2 \eqsp . }
    \end{align}
    where $\{Z_k\}_{k \in \nset}$ is a sequence of independent $d$-dimensional
    Gaussian random variables with zero mean and identity covariance matrix.
    The discretization \eqref{eq:discretization_improved} approximately
    corresponds to the discrete-time scheme introduced in
    \citep{ho2020denoising}, see \Cref{sec:equivalence-with-}. We call this
    discretization scheme the \emph{exponential integrator} (EI) discretization,
    similarly to \cite{zhang2022exponential} who introduced a similar scheme in
    accelerated deterministic diffusion models. \citet{lee2022convergence}
    analyze a slightly different scheme corresponding to replacing
    $\beta_{T-t} \bbfY_t$ by $\beta_{T-t} \bbfY_{t_k}$ in
    \eqref{eq:approximate_time_reversal_continuous}. We summarize the processes
    we have introduced in \Cref{tab:processes} and discuss the links between
    \eqref{eq:discretization_improved} and the classical Euler--Maruyama
    discretization in \Cref{sec:link-with-euler}.
    \begin{table}[h]
\small
\centering
\renewcommand*{\arraystretch}{1.2}
\caption{\small Different processes considered in this paper.}
\begin{tabular}{ll}
  \toprule 
  Description  &     Evolution equation 
  \\ \hline \\
  Forward process    & $\rmd \bfX_t = - \beta_t \bfX_t \rmd t + \sqrt{2 \beta_t} \rmd \bfB_t$  \\
  Backward process (BP) & $\rmd \bfY_t = \beta_{T-t} \{\bfY_t + 2 \nabla \log p_{T-t}(\bfY_t) \} \rmd t + \sqrt{2 \beta_{T-t}} \rmd \bfB_t$ \\ 
  Score approximate BP (SBP) & $\rmd \hat{\bfY}_t = \beta_{T-t} \{\hat{\bfY}_t + 2 \bm{s}(T-t, \hat{\bfY}_t) \} \rmd t + \sqrt{2 \beta_{T-t}}$ \\
  % EM interpolation of $(\hat{\bfY}_t)_{t \in \ccint{0,T}}$ & $\rmd \bbfY_t^{\EM} = \beta_{T-t_k} \{ \bbfY_{t_k}^{\EM} + 2 \bm{s}(T-t_k, \bbfY_{t_k}^{\EM}) \} \rmd t + \sqrt{2\beta_{T-t_k}} \rmd \bfB_t$ \\
  % EM discretization of $(\hat{\bfY}_t)_{t \in \ccint{0,T}}$ & $Y_{k+1}^\EM = Y_k^\EM + \gamma_k  \beta_{T-t_k} \{ Y_k^{\EM} + 2 \bm{s}(T-t_k, Y_k^{\EM}) \} + \sqrt{2 \beta_{T-t_k} \gamma_k} Z_k$ \\
        EI interpolation of SBP      & $\rmd \bbfY_t = \beta_{T-t} \{ \bbfY_{t} + 2 \bm{s}(T-t_k, \bbfY_{t_k}) \} \rmd t + \sqrt{2\beta_{T-t}} \rmd \bfB_t $ \\
  EI discretization of SBP  &
$ Y_{k+1} = \textstyle{Y_k + \gamma_{1,k} (Y_{k} + 2 \bm{s}(T-t_k, Y_{k})) + \sqrt{2 \gamma_{2,k}}} Z_k$ \\ 
  \bottomrule
\end{tabular}
\vspace{.2cm}
\label{tab:processes}
\end{table}
As emphasized in the introduction, under the manifold hypothesis or in the case
where the target distribution is an empirical measure, the true score
$\nabla \log p_t$ explodes when $t \to 0$. This behavior has been observed in
practice for image synthesis \citep{kim2021soft, song2020improved}. One way to
deal with this explosive behavior is to truncate the integration of the backward
diffusion, \ie instead of running $(\bfY_t)_{t \in \ccint{0,T}}$ we consider
$(\bfY_t)_{t \in \ccint{0, T - \vareps}}$ for a small hyperparameter
$\vareps >0$, \citep{vahdat2021score, song2020improved}. Translating this
condition on the associated discretized process, we assume that
$t_{K} = T - \vareps$ and study $\{Y_k\}_{k \in \{0, \dots, K\}}$ by
disregarding the last sample $Y_{K+1}$. We note that versions of diffusion
models defined in discrete time do not suffer from such shortcomings as the
truncation is embedded in the discretization scheme, see
\citep{song2020score,song2020improved,song2019generative,ho2020denoising} for
instance. Recently \citet{kim2021soft} have proposed a soft probabilistic
truncation to replace the proposed hard threshold.

In the next section, we state our main results providing upper bounds on the
distance between the distribution of $Y_{K}$ and $\pi$ \wrt the Wasserstein
distance of order one under the manifold hypothesis.
    
\section{Main results}
\label{sec:main-results}

We first start by introducing and discussing our main assumptions. First, the
only assumption that we make on the data distribution $\pi$ is that it is
supported on a compact set $\M \subset \rset^d$ (\ie a bounded and closed
subset of $\rset^d$).
\begin{assumption}
  \label{assum:manifold_hyp}
  $\pi$ is supported on a compact set $\M$ and $0 \in \M$.
\end{assumption}
The assumption $0 \in \M$ can be omitted but is kept to simplify the proofs. We
denote $\mathrm{diam}(\M)$ the diameter of the manifold defined by $  \mathrm{diam}(\M) = \sup \ensembleLigne{\normLigne{x-y}}{x, y \in \M}$.

An assumption of compactness is natural as images are encoded on a finite range
(typically $\ccint{0, 255}$ for each channel). We emphasize that this assumption
encompasses not only all distributions which admit a continuous density on a
lower dimensional manifolds but also all empirical densities of the form
$(1/N)\sum_{i=1}^N \updelta_{X^i}$. Next, we turn to the temperature schedule
$t \mapsto \beta_t$ and make the following assumption.

\begin{assumption}
  \label{assum:assumption_beta}
  $t \mapsto \beta_t$ is continuous, non-decreasing and there exists
  $\bar{\beta} > 0$ such that for any $t \in \ccint{0,T}$,
  $1/\bar{\beta} \leq \beta_t \leq \bar{\beta}$.
\end{assumption}
Under this assumption, the integral of $t \mapsto \beta_t$ is well-defined and for any $t \in \ccint{0,T}$ we have that 
\begin{equation}
  \textstyle{
  \bfX_t = m_t \bfX_0 + \sigma_t Z \eqsp , \qquad m_t = \exp[-\int_0^t \beta_s \rmd s] \eqsp , \qquad \sigma_t^2 = 1 - \exp[-2\int_0^t\beta_s \rmd s] \eqsp , }
\end{equation}
where the first equality holds in distribution and $Z$ is a Gaussian random
variable with zero mean and identity covariance. Note that
\rref{assum:assumption_beta} is satisfied for every schedule used in practice,
see \Cref{sec:assumptions-schedule}. Finally, we make the following assumption
on the score network.
  \begin{assumption}
    \label{assum:score_control}
    There exist $\bm{s} \in \rmc(\ccint{0,T} \times \rset^d, \rset^d)$ and
    $\Mtt \geq 0$ such that for any $t \in \ccint{0,T}$ and $x_t \in \rset^d$,
  \begin{equation}
    \normLigne{\bm{s}(t, x_t) - \nabla \log p_t(x_t)} \leq \Mtt (1+\normLigne{x_t})/\sigma_{t}^2 \eqsp . 
  \end{equation}
\end{assumption}

Contrary to \citet{debortoli2021diffusion}, we do not assume a uniform bound in
time and space as we allow growth as $t \to 0$ and $\normLigne{x} \to 0$. This
assumption is more realistic as
$\norm{\nabla \log p_t(x_t)} \sim_{t\to 0}c_0(x_t)/\sigma_t^2$ and
$\norm{\nabla \log p_t(x_t)} \sim_{\normLigne{x_t}\to
  +\infty}c_1(t)\normLigne{x_t}$ as we will show in
\Cref{sec:grad-hess-contr}. This explosive behavior as $t\to0$ is accounted for
in practical implementations. For example \citet{song2020score} used a
parameterization of the score of the form $\bm{s}(t,x) = \bm{n}(t,x)/\sigma_t$,
where $\bm{n}$ is a neural network with learnable parameters.  Our assumption is
notably different from the one of \citet{lee2022convergence} which assume a
uniform in time $\mathrm{L}^2$ bound between the score estimator and the true
score. Nevertheless, in \Cref{sec:wass-contr-under} we derive
\Cref{thm:convergence_general_L2} which is the counterpart to our main result
under a $\mathrm{L}^2$ error assumption, extending the theory of
\citet{lee2022convergence} to derive an $\mathrm{L}^\infty$ error from a
$\mathrm{L}^2$ one. Note that $\mathrm{L}^2$ bounds are more realistic than
$\mathrm{L}^\infty$ as the score is estimated on the data.

Finally, we make the following assumption on the sequence of stepsizes. Recall
that for any $k \in \{0, \dots, N\}$ we have $t_{k+1} =\sum_{j=0}^k \gamma_j$
and $t_0 = 0$.

\begin{assumption}
  \label{assum:step_size}
  For any $k \in \{0, \dots, K-1\}$, we have 
  $\gamma_k \sup_{v \in \ccint{T-t_{k+1}, T-t_k}} \beta_v / \sigma_v^2 \leq
  \delta \leq 1/2$.
\end{assumption}

In the case where $\beta_t = \beta_0$ for any $t\in \ccint{0,T}$, \rref{assum:step_size} is
implied by the following condition: for any $k \in \{0, \dots, K-1\}$
\begin{equation}
  \label{eq:gamma_ineq}
  \textstyle{\gamma_k (\beta_0 + (2 \sum_{j=k+1}^K \gamma_j)^{-1}) \leq \delta \eqsp .}
\end{equation}
In the next section, we fix $\gamma_K = \vareps$ and in this case, the condition
\eqref{eq:gamma_ineq} is satisfied if for any $k \in \{0, \dots, K-1\}$,
$\gamma_k \leq \delta \vareps /(2 + \beta_0 \vareps)$.
% In the next section, we set $\gamma_K = \vareps$ and \eqref{eq:gamma_ineq}
% implies that $\gamma_{K-1} \leq \delta\vareps/(2 + \beta_0 \vareps)$.  We
% consider the recursion for any $k \in \{0, \dots, K-1\}$,
% $\gamma_{k} = c \sum_{j=k+1}^K \gamma_j$, which gives
% $\gamma_k = c \vareps (1 - c^{K-k})/(1 - c)$. This sequence is non-decreasing
% for $c \in \ooint{0,1}$ and we have $\gamma_0 \leq c\vareps/(1-c)$. Hence,
% \eqref{eq:gamma_ineq} is satisfied if
% $c(\vareps \beta_0 / (1-c) + (1/2)) \leq \delta$. More generally,
% \Cref{assum:step_size} suggests to set
% $\gamma_k \propto \inf_{v \in \ccint{T-t_{k+1}, T-t_k}} \sigma_v^2 / \beta_v^2$.

\subsection{Convergence bounds}
\label{sec:convergence-bounds}

% In the result We have a condition on the diameter of the data. Quite natural
% We consider the Ornstein-Ulhenbeck
% \begin{equation}
%   \label{eq:ornstein-ulhenbeck}
%   \rmd \bfX_t = - \beta_t \bfX_t \rmd t + \sqrt{2 \beta_t} \rmd \bfB_t \eqsp . 
% \end{equation}
% Note that 

% The last condition ensures that $t \mapsto \int_0^t \beta_s \rmd s$ has at least
% a linear growth near $0$ which is a technical condition necessary to our
% analysis.  \valentin{do we have another interpretation??} This assumption is
% satisfied in all the settings considered in practice, see
% \Cref{sec:assumptions-schedule}.

% This assumption is less restrictive
% than the one considered in
% \cite{debortoli2021diffusion}
% (DISCUTER ASSUMPTION HUAWEI AUSSI),
% since we do not assume uniform
% control both \wrt the time and the
% space variable. Instead the error
% bound can blow up around $0$ with
% rate $\bigO(t^{-1})$. Spatially, we
% also allow for a blow-up of order
% $\bigO(\normLigne{x})$. COMMENT ON THE L2 ERROR

We are now ready to state our main result.
%\valentin{do not forget the assumption on the discretization stepsize}
\begin{theorem}
  \label{thm:convergence_general}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:score_control}, \rref{assum:step_size} that
  $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$, $\gamma_K = \vareps$ and
  $\vareps, \Mtt, \delta \leq 1/32$.
  % \begin{equation}
  %   \textstyle{
  %     t_N = \sum_{k=0}^{N-1} \gamma_k = T - (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps)) \eqsp . 
  %     }
  % \end{equation}
   Then, there exists $\Dtt_0 \geq 0$ such that
   \begin{equation}
         \wassersteinD[1](\mathcal{L}(Y_K), \pi) \leq \Dtt_0 (\exp[\kappa/\vareps] (\Mtt + \delta^{1/2})/ \vareps^2 + \exp[\kappa/\vareps]\exp[-T/\bar{\beta}] + \vareps^{1/2}) \eqsp ,
       \end{equation}
       with $\kappa = \diam(\M)^2(1+\bar{\beta})/2$ and
       \begin{equation}
         \label{eq:constant_diam}         
         \Dtt_0 = D (1 + \bar{\beta})^7(1 + d + \diam(\M)^4) (1 + \log(1 + \diam(\M))) \eqsp ,
       \end{equation}
       and $D$ is a numerical constant.
\end{theorem}

First, we note that letting $\vareps \to 0$, $T \to +\infty$,
$\delta, \Mtt \to 0$ we get that
$\wassersteinD[1](\mathcal{L}(Y_{K}), \pi) \to 0$. More generally the error
bounds depend on four variables
\begin{enumerate*}[label=(\alph*)]  
\item $\vareps$ which corresponds to the truncation of the backward process,
\item $T$ the integration time of the forward process,
\item $\delta$ which is related to a condition on the stepsizes of the backward
  discretization, see \rref{assum:step_size}
\item $\Mtt$ which controls the score approximation, see \Cref{assum:score_control}.
\end{enumerate*}
The dependence \wrt $\delta^{1/2}$ and $\Mtt$ is linear, whereas the dependence
\wrt $T$ is of the form $\exp[-T/\bar{\beta}]$. These two terms are multiplied
by a quantity depending on the truncation bound $\vareps$ which is exponential
of the form $\exp[\kappa/\vareps]$. We conjecture that under additional
assumptions on $\M$ this dependence can be improved to also be polynomial, see
\Cref{thm:convergence_bound_hessian} for an extension of
\Cref{thm:convergence_general} under general Hessian assumptions.


\begin{proof}
  We provide a sketch of the proof. The detailed proof is postponed to
  \Cref{sec:proof_theorem_one}. The distribution of $Y_{K}$ is given by
  $\pi_\infty \Rker_{K}$, where $\Rker_{K}$ is the transition kernel
  associated with $Y_{K}|Y_0$. In order to control
  $\wassersteinD[1](\pi_\infty \Rker_{K}, \pi)$, we consider the following
  inequality
  \begin{equation}
    \label{eq:decomposition}
    \wassersteinD[1](\pi_\infty \Rker_{K}, \pi) \leq \wassersteinD[1](\pi_\infty \Rker_{K}, \pi_\infty \Qker_{t_{K}}) + \wassersteinD[1](\pi_\infty \Qker_{t_{K}}, \pi \Pker_{T - t_{K}}) + \wassersteinD[1](\pi \Pker_{T - t_K}, \pi) \eqsp ,
  \end{equation}
  where $(\Pker_t)_{t \in \ccint{0,T}}$ is the semi-group associated with
  $(\bfX_t)_{t \in \ccint{0,T}}$ and $(\Qker_t)_{t \in \ccint{0,T}}$ is the
  semi-group associated with $(\bhfY_t)_{t \in \ccint{0,T}}$.  We then control
  each one of these terms. The first term corresponds to the discretization
  error and the score approximation. It is upper bounded by a term of the form
  $\bigO(\exp[\kappa/\vareps](\Mtt + \delta)/\vareps^2)$. The second term
  correspond to the convergence of the continuous-time exact backward process
  and is of order $\bigO(\exp[\kappa/\vareps]\exp[-T/\bar{\beta}])$. The last
  term corresponds to the error between the data distribution and a slightly
  noisy version of this distribution and is of order $\bigO(\vareps^{1/2})$. We
  conclude the proof upon combining these results.
\end{proof}

As an immediate corollary of \Cref{thm:convergence_general}, we have the following result.

\begin{corollary}
  \label{coro:control_eta}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:score_control}, \rref{assum:step_size}. Let
  $\eta \in \ooint{0, 1/32}$, $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$ and
  \begin{equation}
    T \geq \bar{\beta} (\kappa + 1) / \eta^2 \eqsp , \quad \Mtt \leq \exp[-\kappa/\eta^2]\eta^4 \eqsp, \quad \delta \leq \exp[-\kappa/\eta^2]\eta^4 \eqsp , \quad \gamma_K = \eta^2 \eqsp .
  \end{equation}
  Then, 
   \begin{equation}
         \wassersteinD[1](\mathcal{L}(Y_K), \pi) \leq \Dtt_0 \eta  \eqsp ,
       \end{equation}
       with $\kappa = \diam(\M)^2(1+\bar{\beta})/2$ and $\Dtt_0$ given in
       \eqref{eq:constant_diam}.
\end{corollary}

The constant $\Dtt_0$ appearing in \Cref{thm:convergence_general} and
\Cref{coro:control_eta} does not depend on $\vareps$, $T$, $\delta$ and $\Mtt$
but only on $\bar{\beta}$, $\diam(\M)$ and $d$. In particular, we highlight that
the dependence of $\Dtt_0$ \wrt the dimension is $\bigO(d)$ and the dependence
\wrt the diameter of $\M$ is $\bigO(\diam(\M)^4)$ up to logarithmic term. Note
that the diameter might only depend on \textit{intrisic} dimension $p$ of $\M$
which satisfies $p \ll d$ in some settings. For example in the case of an
hypercube of dimension $p$ we have $\diam(\M) = \sqrt{p}$.

Contrary to
\citet{debortoli2021diffusion,lee2022convergence,pidstrigach2022score}, our
results are stated \wrt the Wasserstein distance and not the total variation
distance or the Kullback-Leibler divergence. We emphasize that studying the
total variation or Kullback-Leibler divergence between the distribution of
$Y_{K}$ and the one of $\pi$ under \rref{assum:manifold_hyp} with $\M$ lower
dimensional than $\rset^d$ lead to \emph{vacuous bounds} as these quantities are
lower bounded by $1$ in the case of the total variation and $+\infty$ in the
case of the Kullback-Leibler divergence since the densities we are comparing are
not supported on the same set. This is not the case with the Wasserstein
distance of order one. To the best of our knowledge
\Cref{thm:convergence_general} is the first convergence result for diffusion
models \wrt $\wassersteinD[1]$. We note that our result could be extended to
$\wassersteinD[p]$ for any $p \geq 1$.


We conclude this section, with an improvement upon
\Cref{thm:convergence_general} in the case where tighter bounds on the Hessian
$\nabla^2 \log p_t$ are available.

\begin{theorem}
  \label{thm:convergence_bound_hessian}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:score_control}, \rref{assum:step_size} that
  $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$, $\gamma_K = \vareps$ and
  $\vareps, \Mtt, \delta \leq 1/32$. In addition, assume that there exists
  $\Gamma \geq 0$ such that for any $t \in \ocint{0, T}$ and $x_t \in \rset^d$
  \begin{equation}
    \label{eq:bound_tight_nabla2}
    \normLigne{\nabla \log p_t^2(x_t)} \leq \Gamma / \sigma_t^2 \eqsp . 
  \end{equation}
  % \begin{equation}
  %   \textstyle{
  %     t_N = \sum_{k=0}^{N-1} \gamma_k = T - (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps)) \eqsp . 
  %     }
  % \end{equation}
   Then, there exists $\Dtt_0 \geq 0$ such that
   \begin{equation}
         \wassersteinD[1](\mathcal{L}(Y_K), \pi) \leq \Dtt_0 ((\Mtt + \delta^{1/2})/ \vareps^{\Gamma+2} + \exp[-T/\bar{\beta}]/\vareps^{\Gamma} + \vareps^{1/2}) \eqsp ,
       \end{equation}
       with 
       \begin{equation}
         \label{eq:constant_diam_urg}
         \Dtt_0 = D (1 + d + (1+\diam(\M))^4)\exp[3(1+\bar{\beta})^2(\Gamma+2)(1+\log(1+\diam(\M)))] \eqsp . 
       \end{equation}
       and $D$ is a numerical constant.
\end{theorem}

     \begin{proof}
       The complete proof is postponed to \Cref{sec:proof-convergence-hessian}. The crux
       of the proof is to derive an improved version of
       \Cref{prop:control_gradient} which provides controls on some tangent
       process. Indeed, in \Cref{prop:control_gradient}, we use an upper bound
       of the form $\normLigne{\nabla^2 \log p_t(x_t)} \leq \Gamma / \sigma_t^4$
       which is a loose upper bound derived under \rref{assum:manifold_hyp}.
     \end{proof}

     \Cref{thm:convergence_bound_hessian} improves the bounds of
     \Cref{thm:convergence_general}, since the \emph{exponential} dependency
     \wrt $\vareps$ is replaced by a \emph{polynomial} dependency with exponent
     $\Gamma$. At first sight, it is not clear when
     \eqref{eq:bound_tight_nabla2} is satisfied. However, in special cases we
     can verify this condition explicitly. For example, in
     \Cref{sec:hess-bounds-unif}, we show that this condition is satisfied if
     $\pi$ is the uniform distribution on the hypercube, with
     $p \in \{1, \dots, d\}$. The condition \eqref{eq:bound_tight_nabla2} has
     strong geometrical implications on $\M$. In particular, under appropriate
     smoothness assumptions on $\M$, it implies that $\M$ is convex,
     \Cref{sec:non-conv-count}. Finally, we note that the proof can also be
     extended to work with $\mathrm{L}^2$ errors following the lines of
     \Cref{sec:wass-contr-under}.
     
% We conclude this section with an improvement of \Cref{thm:convergence_general}
% in the case where $\M$ is an hypercube.

% \begin{theorem}
%   \label{thm:convergence_sev}
%   Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
%   \rref{assum:score_control}, \rref{assum:step_size} that
%   $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$, $t_K = T - \vareps$ and
%   $\Mtt, \delta \leq 1/32$. In addition, assume that $\M = \ccint{-1,1}^p$ with
%   $p \leq d$ and that $\pi$ admits a smooth positive density \wrt the uniform
%   distribution on $\M$.  Then, there exist $A \geq 0$ such that
%   \begin{equation}
%     \wassersteinD[1](\pi_\infty \Rker_K, \pi) \leq A (\exp[1/\vareps](\Mtt + \delta)/\vareps^2 + \exp[1/\vareps]\exp[-T/\bar{\beta}] + \vareps )\eqsp . 
%   \end{equation}
% \end{theorem}

% \valentin{pour ce resultat il faut simplement mettre le meilleur controle dans
%   la Hessienne puis dans le controle du processus tangent (deux lemmes)}

% \begin{proof}
%   The proof is similar to the one of \Cref{thm:convergence_general} and only
%   differs in the control of $\nabla^2 \log p_t$. In particular, we derive a
%   tighter bound for the covariance term appearing in $\nabla^2 \log p_t$ given
%   by $I_1/I_0$ where
%   $I_1 = \int_{\M \times \M} \normLigne{z_0 - z_1}^2 \exp[-\normLigne{z_0 -
%     x_t}^2/(2\sigma_t^2) -\normLigne{z_1 - x_t}^2/(2\sigma_t^2) ] \rmd (\pi
%   \otimes \pi)(z_0, z_1)$ and $I_0 = \int_{\M \times \M}  \exp[-\normLigne{z_0 -
%     x_t}^2/(2\sigma_t^2) -\normLigne{z_1 - x_t}^2/(2\sigma_t^2) ] \rmd (\pi
%   \otimes \pi)(z_0, z_1)$.
% \end{proof}

% \valentin{actually do the proof}

% In \Cref{thm:convergence_sev}, contrary to \Cref{thm:convergence_general}, the
% dependence \wrt $1/\vareps$ is polynomial and not exponential. The current
% theorem can readily be extended to cover any $\M$ of the form
% $\ensembleLigne{ \sum_{i=1}^p \alpha_i e_i}{\alpha_i \in \ccint{a_i, b_i}}$
% where $\{e_i\}_{i=1}^p$ is a family of independent vectors of $\rset^d$. We
% conjecture that \Cref{thm:convergence_sev} can also be extended to the case of
% analytic manifolds using quantitative versions of the Morse lemma and Laplace
% expansions, see \cite{le2014numerical}.

\subsection{Generalization results and empirical measure targets}

We emphasize that the results of \Cref{thm:convergence_general} hold under the
general assumption \Cref{assum:manifold_hyp} which only requires the target
measure to be supported on a compact set. This includes measures which are
supported on a smooth manifold of dimension $p \leq d$ but also all empirical
measures of the form $(1/N) \sum_{i=1}^N \updelta_{X^i}$ with
$\{X^i\}_{i=1}^N \sim \pi^{\otimes N}$. In particular if we assume that the
underlying target measure $\pi$ is supported on a manifold of dimension
$p \leq d$ and that the diffusion models are trained \wrt some empirical
measure associated with $\pi$ then we have the following generalization result.

\begin{proposition}
  \label{prop:gener-results}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:score_control}, \rref{assum:step_size} that
  $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$, $\gamma_K = \vareps$ and
  $\vareps, \Mtt, \delta \leq 1/32$.
  % \begin{equation}
  %   \textstyle{
  %     t_N = \sum_{k=0}^{N-1} \gamma_k = T - (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps)) \eqsp . 
  %     }
  % \end{equation}
   Then, for any $\eta >0$ there exist $\Dtt_0, \Dtt_1 \geq 0$ such that
   \begin{equation}
         \expeLigne{\wassersteinD[1](\mathcal{L}(Y_K), \pi)} \leq \Dtt_0 (\exp[\kappa/\vareps] (\Mtt + \delta^{1/2})/ \vareps^2 + \exp[\kappa/\vareps]\exp[-T/\bar{\beta}] + \vareps) + \Dtt_1N^{-1/(\dim_M(\M)+\eta)} \eqsp ,
       \end{equation}
       with $\dim_M(\M)$ the Minkowski dimension of $\M$, see
       \eqref{eq:minkowski}, $\kappa = \diam(\M)^2(1+\bar{\beta})/2$, $\Dtt_1$
       given in \cite[Theorem 1]{weed2019sharp} and
       \begin{equation}
         \Dtt_0 = D (1 + \bar{\beta})^7(1 + d + \diam(\M)^4) (1 + \log(1 + \diam(\M))) \eqsp ,
       \end{equation}
       and $D$ is a numerical constant.
     \end{proposition}

     Note that in \Cref{prop:gener-results}, the expectation in
     $\expeLigne{\wassersteinD[1](\mathcal{L}(Y_K), \pi)}$ is taken \wrt
     $\pi^{\otimes N}$. More precisely, the diffusion model
     $(Y_k)_{k \in \{0, \dots, K\}}$ is trained \wrt
     $\pi^N= (1/N)\sum_{i=1}^N \updelta_{X^i}$ and therefore
     $\wassersteinD[1](\mathcal{L}(Y_K), \pi)$ is a random variable depending on
     $\{X^i\}_{i=1}^N \sim \pi^{\otimes N}$. In \Cref{prop:gener-results}, we
     provide generalization results in \emph{expectation} but note that
     generalization results in \emph{high probability} are also available using
     similar techniques from \cite[Section 6]{weed2019sharp}.
     
     \begin{proof}
       For any $N \in \nset$, we denote $\pi^N = (1/N) \sum_{i=1}^N
       \updelta_{X^i}$. Using \Cref{thm:convergence_general}, we have that for any $N \in \nset$
       \begin{equation}
         \wassersteinD[1](\mathcal{L}(Y_K), \pi^N) \leq \Dtt_0 (\exp[\kappa/\vareps] (\Mtt + \delta^{1/2})/ \vareps^2 + \exp[\kappa/\vareps]\exp[-T/\bar{\beta}] + \vareps) \eqsp ,
       \end{equation}
       with a constant $\Dtt_0$ which does not depend on $\{X^i\}_{i=1}^N$ and
       $N$. Therefore, we have that for any $N \in \nset$
       \begin{equation}
         \label{eq:wasserstein_target_empirique}
         \expeLigne{\wassersteinD[1](\mathcal{L}(Y_K), \pi^N)} \leq \Dtt_0 (\exp[\kappa/\vareps] (\Mtt + \delta^{1/2})/ \vareps^2 + \exp[\kappa/\vareps]\exp[-T/\bar{\beta}] + \vareps) \eqsp .
       \end{equation}
       Using \cite[Theorem 1]{weed2019sharp} and \cite[Proposition
       2]{weed2019sharp}, for any $\eta >0$, there exists $\Dtt_1 \geq 0$ such
       that
       \begin{equation}
         \expeLigne{\wassersteinD[1](\pi^N, \pi)} \leq \Dtt_1 N^{-1/(\dim_M(\M) + \eta)}\eqsp ,
       \end{equation}
       which concludes the proof upon combining this result,
       \eqref{eq:wasserstein_target_empirique} and the triangle inequality. 
     \end{proof}

     The Minkowski dimension $\dim(\M)$ is defined as follows:
     \begin{equation}
       \label{eq:minkowski}
       \textstyle{\dim(\M) = d - \liminf_{\vareps \to 0} \log(\Vol(\M_{\vareps}))/\log(1/\vareps)\eqsp , }
     \end{equation}
     with $\Vol(\msa)$ the volume of a (measurable) set $\msa$ and $\M_\vareps$
     the $\vareps$-fattening of $\M$, \ie for any $ \vareps >0$,
     $\M_\vareps = \ensembleLigne{x \in \rset^d}{d(x, \M) \leq \vareps}$.  For
     example if $\M$ is a topological manifold of dimension $p \leq d$ then its
     Minkowski dimension is $p$, \ie $\dim_M(\M) = p$. Hence, in this case the
     error term in \Cref{prop:gener-results} depends \emph{exponentially} on the
     dimension of $\M$ and on its diameter but depends only \emph{linearly} on
     $d$, the dimension of the ambient space. Note again that $\diam(\M)$ might
     depend on the dimension of $\M$. For example in the case of the hypercube
     $\M = [-1/2,1/2]^p$, we have $\diam(\M) = \sqrt{p}$. Hence, the results of
     \Cref{prop:gener-results} show that diffusion models take advantage of the
     lower-dimensional structure of the target. 
%      We conclude this section, with a study on the effect of the sample size
%      $N$. We show that bias induced by the empirical measure is mitigated by the
%      diffusive behavior of the forward process. \cite{peluchetti2021non}
     
% \begin{itemize}
% \item Faire la meme experience mais avec des reseaux entraines
% \item Faire l'experience avec les distances de Wasserstein
% \end{itemize}

% \begin{tikzpicture}
% \node[inner sep=0pt] (generalization) at (0,0)
% {\includegraphics[width=.59\textwidth]{fisher_score}};
% \node[inner sep=0pt] (generalization) at (-4.5,-2)
% {\includegraphics[width=.15\textwidth]{forward_process_time_1}};
% \node[inner sep=0pt] (generalization) at (-0.95,-2)
%     {\includegraphics[width=.15\textwidth]{forward_process_time_2}};
% \node[inner sep=0pt] (generalization) at (2.2,-2)
% {\includegraphics[width=.15\textwidth]{forward_process_time_3}};
% \end{tikzpicture}

\subsection{Related works}
\label{sec:related-works}

To the best of our knowledge, \citep{debortoli2021diffusion} provided the first quantitative
convergence results for denoising diffusion models. More precisely,  \citet{debortoli2021diffusion} show a bound in total
variation between the distribution of the diffusion model and the target
distribution of the form
\begin{equation}
  \label{eq:earlier_tv}
  \tvnorm{\mathcal{L}(Y_{K+1}) - \pi} \leq A( \exp[-T] + \exp[T] (\Mtt^{1/2} + \delta^{1/2})) \eqsp . 
\end{equation}
This result holds under the assumption that $\pi$ admits a density \wrt Lebesgue
measure which satisfies some dissipativity conditions. Again we emphasize that
such results in total variation are vacuous under the manifold hypothesis. The
upper bound in \eqref{eq:earlier_tv} is obtained using a similar splitting of
the error as in \Cref{thm:convergence_general}. However the control of the
discretization error is handled using Girsanov formula in
\citep{debortoli2021diffusion} and relies on similar techniques as
\citep{dalalyan2017theoretical,durmus2017nonasymp}. In the present work, this
error is controlled using the interpolation formula from \citet{del2019backward}
which, combined with controls on stochastic flows, allows for tighter controls
of the discretization error \wrt $\wassersteinD[1]$.

% \cite{lee2022convergence} investigate the convergence of the original diffusion
% model of \cite{song2019generative}, \ie a warm-start version of annealing with
% estimation of the score. 
% In our setting this amounts to replacing the forward
% process with a simple Brownian motion.
% Similar results to the ones of
% \Cref{thm:convergence_general} could be derived in this setting upon replacing
% $\bigO(\exp[-T/\bar{\beta}])$ in the bound with $\bigO(1/T)$ and replacing
% $\pi_\infty$ with $\mathrm{N}(0, T\Id)$.
% Contrary to our study 
\citet{lee2022convergence} study the convergence of diffusion models under
(uniform in time) $\mathrm{L}^2$ controls on the score approximation. Their
result is given \wrt the total variation and therefore suffers from the same
shortcoming as the ones of \citet{debortoli2021diffusion}. In particular it is
assumed that the data distribution admits a density \wrt the Lebesgue measure
which satisfies some regularity conditions as well as a logarithmic Sobolev
inequality. Additionally, it is required that $\nabla^2 \log p_t$ is bounded
uniformly in time and in space which is not true under the manifold hypothesis
and is hard to verify in practice even in simple cases.

Closer to our line of work are the results of \citet{pidstrigach2022score} who
proves that the approximate backward process
\eqref{eq:approximate_time_reversal_continuous} converges to a random variable
whose distribution is supported on the manifold of interest. In this work, we go
one step further by studying the discretization scheme and providing
quantitative bounds between the output of the diffusion model and the target
distribution.

Related to the manifold hypothesis and the study of convergence of diffusion
models is the work of \citet{de2022riemannian} who study the convergence of a
Riemannian counterpart of diffusion models. Result are given \wrt the total
variation (defined on the manifold of interest). Even though such diffusion
models directly incorporate the manifold information they require the knowledge
of the geodesics and the Riemannian metric of the manifold. In the case of the
manifold hypothesis these quantities are not known and therefore cannot be used
in practice. In particular, \citet{de2022riemannian} focus on manifolds which
have a well-known structure such as $\mathbb{S}^1$, $\mathbb{T}^2$ or
$\mathbb{SO}_3(\rset)$.

\citet{franzese2022much} show that there exists a trade-off between long and
short time horizons $T$. Their analysis is based on a rearrangement of the
Evidence Lower Bound (ELBO) obtained by \citet{huang2021variational}. This ELBO
can be decomposed in the sum of two terms: one which decreases with $T$
(controlling the bias between $\mathcal{L}(\bfX_T)$ and $\pi_\infty$) and one
which increases with $T$ (corresponding to the loss term
\eqref{eq:dsm_loss}). Their decomposition of the ELBO is in fact equivalent to
\cite[Theorem 1]{durkan2021maximum}. In \Cref{sec:short-proof} we include a
short derivation of this result.

Finally, we highlight the earlier results of \citet{block2020generative}. In
this work, the authors study a version of the Langevin algorithm in which the
score term is approximated. This is different from the diffusion model
\footnote{Note however that the authors provide a discussion on an annealed
  version of the algorithm they study which corresponds to the original
  framework of \citet{song2019generative}.} setting and is closer to the setting
of Plug-and-Play approaches
\citep{venkatakrishnan2013plug,arridge2019solving,zhang2017learning}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/proof.tex <==
% \section{Stability and growth of the backward process}
% \label{sec:stab-backw-proc}







%   \section{Backward interpolation error}
% \label{sec:backw-interp-error}

% In this section, we focus on the following error
% $\wassersteinD[1](\pi_\infty \rmQ_{t_1}, \pi_\infty \rmR_{N})$. To control
% this term, we use \Cref{prop:pierre-extended} together with the controls derived
% in \Cref{sec:stab-backw-proc}.

% \subsection{Drift controls}
% \label{sec:drift-decomp-contr}

% We start with the following useful lemma.

% % \begin{lemma}
% %   \label{lemma:condition_beta_integral}
% %   Assume \rref{assum:assumption_beta}. Then for any $t \in \ccint{0,T}$, $\textstyle{\int_0^t \beta_s \rmd s \geq t \beta_t / (1 + C)}$.
% % \end{lemma}

% % \begin{proof}
% %   We have that for any $t \in \ocint{0,T}$, $\beta_t' \leq C \beta_t /t$ using
% %   \rref{assum:assumption_beta}. Hence, we get that for any $t \in \ocint{0,T}$,
% %   $C \beta_t \geq t\beta_t'$ and hence $(1+C)\beta_t \geq
% %   (t\beta_t)'$. Therefore, we have that for any $t \in \ccint{0,T}$,
% %   $\textstyle{\int_0^t \beta_s \rmd s \geq t \beta_t / (1 + C)}$, which
% %   concludes the proof.
% % \end{proof}

% The following lemma controls the growth of $\kappa_k$ w.r.t. $k \in \{0, \dots, N-1\}$.


% \valentin{faire les changements plus haut t0 devient ta et t1 devient tb}

%   \section{Wasserstein approximation and conclusion}
% \label{sec:wass-appr-concl}

% In this section, we focus on the error $\wassersteinD[1](\pi, \pi\Pker_{T-t_b})$
% and conclude the proof.
% First, we have that
% \begin{equation}
%   \wassersteinD[1](\pi, \pi\Pker_{T-t_b}) \leq \expeLigne{\normLigne{X - m_{T-t_b} X + \sigma_{T-t_b} Z}} \eqsp ,
% \end{equation}
% with $X \sim \pi$ and $Z \sim \mathrm{N}(0, \Id)$. Hence, we have 
% \begin{equation}
%   \wassersteinD[1](\pi, \pi\Pker_{T-t_b}) \leq \diam(\M) (1 - m_{T-t_b}) + \sigma_{T-t_b} d \leq (\diam(\M) + d) \sigma_{T-t_b} \eqsp .
% \end{equation}
% Combining this result, \eqref{eq:convergence_bound_backward} and
% \Cref{prop:discretization_bound_final} we get that
% \begin{align}
%   \wassersteinD[1](\pi_\infty \Rker_N, \pi) &\leq \wassersteinD[1](\pi_\infty \Rker_N, \pi_\infty \Qker_{t_b}) + \wassersteinD[1](\pi_\infty \Qker_{t_b}, \pi \Pker_{t_b}) + \wassersteinD[1](\pi \Pker_{t_b}, \pi) \\
%                                             &\leq \textstyle{ \exp[(1/2)\sigma_{T-t_b}^{-2}]} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2) /((T-t_b)^2\beta_{T-t_b})  (1 + t_b - t_a) \\
%                                             & \qquad \textstyle{ + \exp[(1/2)\sigma_{T-t_b}^{-2}] \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\sigma_{T-t_b} \eqsp . } \label{eq:intermediate_bound_tb_ta}
% \end{align}

% In order to conclude, we now link $t$ and $\sigma_{T-t}^2$ with the following lemma.

% % \begin{lemma}
% %   \label{lemma:bound_sigma_t}
% %   Let $t = (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps))$ then $\sigma_{t}^2 \leq \vareps$ and $\sigma_t^2 \geq \vareps/\bar{\beta}^2$. We also have that $t \geq \vareps/(2\bar{\beta})$.
% % \end{lemma}

% % \begin{proof}
% %   First, we have that
% %   \begin{equation}
% %     \textstyle{\sigma_t^2 = 1 - \exp[-2\int_0^t \beta_s \rmd s] \leq 1 - \exp[-\log(1 + \vareps/(1-\vareps))]} \leq \vareps \eqsp . 
% %   \end{equation}
% %   Then, we have
% %   \begin{equation}
% %     \textstyle{\sigma_t^2 = 1 - \exp[-2\int_0^t \beta_s \rmd s] \geq 1 - \exp[-\bar{\beta}^{-2}\log(1 + \vareps/(1-\vareps))]} \geq 1 - (1-\vareps)^{\bar{\beta}^{-2}} \eqsp . 
% %   \end{equation}
% %   We conclude upon using that $(1-\vareps)^{\bar{\beta}^{-2}} \leq 1 - \vareps/\bar{\beta}^2$.
% % \end{proof}

% \valentin{modifier la suite en fonction !}

% In what follows, we set
% $t_b = T - (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps))$ and recall that
% using \eqref{eq:t_a_def}, we have
% \begin{equation}
%   t_a = T - (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \vareps +(1 + \vareps \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\vareps)) \eqsp . 
% \end{equation}
% \valentin{remove the eps dependency in ta}
% Therefore, we get that
% \begin{equation}
%   t_b -t_a \leq (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \vareps +(1 + \vareps \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\vareps)) \eqsp . 
% \end{equation}
% \valentin{this gives a natural condition on $T$ to be large enough so that everything is positive (when I say everything I am talking about ta)}
% Therefore, combining this result and \Cref{lemma:bound_sigma_t} in
% \eqref{eq:intermediate_bound_tb_ta}, we get that
% \begin{align}
%   &\wassersteinD[1](\pi_\infty \Rker_N, \pi)  \leq \textstyle{ \exp[(1/2)\sigma_{T-t_b}^{-2}]} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2) /((T-t_b)^2\beta_{T-t_b})  (1 + t_b - t_a) \\
%                                              & \qquad \textstyle{ + \exp[(1/2)\sigma_{T-t_b}^{-2}] \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\sigma_{T-t_b} \eqsp . } \\
%                                              &\leq \textstyle{ 4\bar{\beta}^3 \exp[\bar{\beta}/(2\vareps)]\vareps^{-2}} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2)  \\
%   & \qquad \times (1 +  (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \eta +(1 + \eta \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\eta))) \\
%                                             & \qquad \textstyle{ + \exp[\bar{\beta}/(2\vareps)] \exp[-T/\bar{\beta}] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\vareps \eqsp , }
% \end{align}
% which concludes the proof.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> arxiv/proof_sketch.tex <==
\section{Proof of \Cref{thm:convergence_general}}
\label{sec:proof_theorem_one}

In this section, we present a proof of \Cref{thm:convergence_general}. More
precisely, we control each term on the right hand side of
\eqref{eq:decomposition}. The bottleneck of the proof resides in the control of
the discretization and approximation error
$\wassersteinD[1](\pi_\infty \Rker_{K}, \pi_\infty \Qker_{t_K})$ which is
dealt with in \Cref{sec:discretization_approximation_error}. Then, we turn to
the convergence of the backward process
$\wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T - t_K})$ in
\Cref{sec:convergence_backward}. Finally, we control the noising error
$\wassersteinD[1](\pi \Pker_{T - t_K}, \pi)$ and conclude in
\Cref{sec:noising_error_conclusion}. Technical results are postponed to the
appendix.

\subsection{Control of $\wassersteinD[1](\pi_\infty \Rker_{K}, \pi_\infty \Qker_{t_K})$}
\label{sec:discretization_approximation_error}

In this section, we control
$\wassersteinD[1](\pi_\infty \Rker_{K}, \pi_\infty \Qker_{t_K})$. To do so we
are going to use the backward formula introduced in \citet{del2019backward}.
First, we recall the definition of the stochastic flows
$(\bfY_{s,t}^x)_{s, t \in \ccint{0,T}}$ and the interpolation of its
discretization $(\bbfY_{s,t}^x)_{s, t \in \ccint{0,T}}$, for any $x \in \rset^d$
and $s,t \in \ccint{0,T}$ with $t \geq s$
\begin{equation}
  \textstyle{
    \rmd \bfY_{s,t}^x = \beta_{T-t} \{ \bfY_{s,t}^x + 2 \nabla \log p_{T-t}(\bfY_{s,t}^x) \} \rmd t + \sqrt{2 \beta_{T-t}} \rmd \bfB_t \eqsp , \qquad \bfY_{s,s}^x = x \eqsp ,
    }
\end{equation}
and for any $k \in \{0, \dots, K\}$ and $t \in \coint{s_k, t_{k+1}}$
\begin{equation}
  \textstyle{
    \rmd \bbfY_{s,t}^x = \beta_{T-t} \{ \bbfY_{s, t}^x + 2 \bm{s}(T-s_k, \bbfY_{s, s_k}^x) \} \rmd t + \sqrt{2 \beta_{T-t}} \rmd \bfB_t  \eqsp , \qquad \bbfY_{s,s}^x = x \eqsp ,
    }
  \end{equation}
  where $s_k = \max(s, t_k)$.  We also introduce the tangent process
  \begin{equation}
      \label{eq:tangent_process}
  \textstyle{
    \rmd \nabla \bfY_{s,t}^x = \beta_{T-t} \{ \Id + 2 \nabla^2 \log p_{T-t}(\bfY_{s,t}^x) \} \nabla \bfY_{s,t}^x \rmd t  \eqsp , \qquad \nabla \bfY_{s,s}^x = \Id \eqsp .
  }
\end{equation}
The tangent process $(\nabla \bfY_{s,t}^x)_{s,t \in \ccint{0, T}}$ can also be
defined as follows. Under mild regularity assumption, for any
$s, t \in \ccint{0,T}$ with $t\geq s$, $x \mapsto \bfY_{s,t}^x$ is a
diffeomorphism, see \citep{kunita1981decomposition}, and we denote
$x \mapsto \nabla \bfY_{s,t}^x$ its differential. Then, \cite[Section
2]{kunita1981decomposition} shows under mild assumptions that
$(\nabla \bfY_{s,t}^x)_{s,t \in \ccint{0, T}}$ satisfies
\eqref{eq:tangent_process}. Hence,
$(\nabla \bfY_{s,t}^x)_{s,t \in \ccint{0, T}}$ encodes the local variation of
the process $(\bfY_{s,t}^x)_{s,t \in \ccint{0, T}}$ \wrt its initial
condition.  Our bound on the approximation/discretization error relies on the
following proposition which was first proven by \citet{del2019backward}.
\begin{proposition}
  \label{prop:pierre-extended}
  Assume \rref{assum:manifold_hyp}. Then, for any $s, t \in \coint{0,T}$ with $s<t$ and $x \in \rset^d$
  \begin{equation}
\textstyle{    \bfY_{s,t}^x - \bbfY_{s,t}^x = \int_s^t \nabla \bfY_{u,t}^x(\bbfY_{s,u}^x)^\top \Delta b_u((\bbfY_{s,v}^x)_{v\in \ccint{s,T}}) \rmd u } \eqsp , %+  \int_s^t \nabla \bfY_{u,t}(\bbfY_{s,u})^\top \Delta \volat_u((\bbfY_{s,v})_{v\in \ccint{s,u}}) \rmd \bfB_u \eqsp ,  }
\end{equation}
where for any $u \in \coint{0,T}$ such that $u \in \coint{s_k, t_{k+1}}$ for
some $k \in \{0, \dots, K\}$ and $(\omega_v)_{v \in \ccint{s,T}} \in \rmc(\ccint{s,T}, \rset^d)$ we have 
  \begin{align}
    &b_u(\omega) = \beta_{T-u}( \omega_u + 2 \nabla \log p_{T-u}(\omega_u)) \eqsp , \qquad \bar{b}_u(\omega) = \beta_{T-u}(\omega_{u} + 2 \bm{s}(T -s_k, \omega_{s_k})) \eqsp , \\
%    &\volat_u(\omega) = \sqrt{2 \beta_{T-u}} \eqsp , \qquad  \bar{\volat}_u(\omega) = \sqrt{2 \beta_{T-u}} \eqsp , \\
    &\Delta b_u(\omega) = b_u(\omega) - \bar{b}_u(\omega) \eqsp , %\qquad \Delta \volat_u(\omega) = \volat_u(\omega) - \bar{\volat}(\omega) = 0 \eqsp .
  \end{align}
  where $s_k = \max(s, t_k)$.
\end{proposition}

\begin{proof}
  The proof of this proposition and a discussion are postponed to
  \Cref{sec:stoch-interp-form}.
\end{proof}

Using \Cref{prop:pierre-extended} our goal is now to control
$\normLigne{\nabla \bfY_{s,t}^x}$ and $\normLigne{\Delta b_s((\bbfY_{s,t}^x)_{t \in \ccint{s,T}})}$
for any $s \in \ccint{0,T}$ and $x \in \rset^d$.  To do so, we introduce the
time $t^\star$ which is a lower bound on the supremum time so that the backward
process is contractive on $\ccint{0, t^\star}$
\begin{equation}
  \label{eq:def_t_star}
  t^\star =  T - 2\bar{\beta}(1 + \log(1+\diam(\M))) \eqsp . 
\end{equation}
We then obtain the following controls.

\begin{proposition}
  \label{prop:control_gradient}
  Assume \rref{assum:manifold_hyp} and
  $T \geq 2\bar{\beta}(1 + \log(1+\diam(\M))$.  Let
  $t_K \in \coint{0, T}$. Then, for any $s\in \ccint{0,t_K}$ and
  $x \in \rset^d$ we have
  \begin{equation}
    \textstyle{
      \normLigne{\nabla \bfY_{s,t_K}^x} \leq \exp[-(1/2) \int_{T-t^\star}^{T-s} \beta_u \rmd u \1_{\coint{0,t^\star}}(s)] \exp[(\diam(\M)^2/2)\sigma_{T-t_K}^{-2}] \eqsp .
      }
    \end{equation}
  \end{proposition}

  \begin{proof}
    Let $x\in \rset^d$. First, using \eqref{eq:tangent_process} and \Cref{lemma:control_hessian} we have that for any $s, t\in \ccint{0,T}$ with $s \leq t$
    \begin{equation}
      \rmd \normLigne{\nabla \bfY_{s,t}^x}^2 \leq 2\beta_{T-t}(\normLigne{\nabla \bfY_{s,t}^x }^2 - 2(1  -  m_{T-t}^2 \diam(\M)^2 / (2\sigma_{T-t}^2) )/\sigma_{T-t}^2 \normLigne{\nabla \bfY_{s,t}^x}^2) \rmd t  \eqsp . 
    \end{equation}
    First, assume that $s \leq t^\star$ and that $t \geq t^\star$. In that case, using
    \Cref{lemma:growth_tangent_process} we have that
      \begin{equation}
\textstyle{    \int_s^{t^\star}\beta_{T-u} (1 -2/\sigma_{T-u}^2 + m_{T-u}^2\diam(\M)^2/\sigma_{T-u}^4) \rmd u  \leq -(1/2) \int_s^{t^\star} \beta_{T-u} \rmd u  \eqsp . }
\end{equation}
Therefore, using that result and the fact that $\nabla \bfY_{s,s}^x = \Id$, we get that
\begin{equation}\label{eq:inter_s_lower}
  \textstyle{\normLigne{\nabla \bfY_{s,t^\star}} \leq \exp[-(1/2)\int_{T-t^\star}^{T-s} \beta_u \rmd u] \eqsp . }
\end{equation}
In addition, using \Cref{lemma:growth_tangent_process} we have that
\begin{equation}
    \textstyle{    \int_{t^\star}^{t}\beta_{T-u} (1 -2/\sigma_{T-u}^2 + m_{T-u}^2\diam(\M)^2/\sigma_{T-u}^4) \rmd u} 
    \leq (\diam(\M)^2/2)(\sigma_{T-t}^{-2} - \sigma_{T-t^\star}^{-2}) \eqsp . 
  \end{equation}
  Therefore, we get that
\begin{equation}
  \textstyle{\normLigne{\nabla \bfY_{s,t}} \leq \exp[(\diam(\M)^2/2)\sigma_{T-t}^{-2}] \normLigne{\nabla \bfY_{s,t^\star}} \eqsp . }
\end{equation}
  Hence, combining this result and \eqref{eq:inter_s_lower}, in the case where $s \leq t^\star$ we have
  \begin{equation}
          \textstyle{\normLigne{\nabla \bfY_{s,t}^x} \leq \exp[-(1/2) \int_{T-t^\star}^{T-s} \beta_s \rmd s ] \exp[(\diam(\M)^2/2)\sigma_{T-t}^{-2}] \eqsp .}
        \end{equation}
        The proof in the cases where $s \geq t^\star$, $t \geq t^\star$ and
        $s \leq t^\star$, $t \leq t^\star$ are similar and left to the reader.
  \end{proof}

  Our next goal is to control $\normLigne{\Delta b}$. We recall that
  $b, \bar{b}: \ \ccint{0,T} \times \rmc(\ccint{0,T}, \rset^d) \to \rset^d$
  where for any $u \in \coint{0,T}$ such that $u \in \coint{s_k, t_{k+1}}$ for
  some $k \in \{0, \dots, K\}$ and
  $\omega = (\omega_v)_{v \in \ccint{s,T}} \in \rmc(\ccint{s,T}, \rset^d)$
  \footnote{With a slight abuse of notation we assume that each process on
    $\rmc(\ccint{s, T})$ is extended on $\rmc(\ccint{0, T})$ by setting
    $\omega_u = \omega_s$ for any $u \in \ccint{0,s}$. } we have
  \begin{align}
    &b_u(\omega) = \beta_{T-u}( \omega_u + 2 \nabla \log p_{T-u}(\omega_u)) \eqsp , \qquad \bar{b}_u(\omega) = \beta_{T-u}(\omega_{u} + 2 \bm{s}(T -s_k, \omega_{s_k})) \eqsp , \\
%    &\volat_u(\omega) = \sqrt{2 \beta_{T-u}} \eqsp , \qquad  \bar{\volat}_u(\omega) = \sqrt{2 \beta_{T-u}} \eqsp , \\
    &\Delta b_u(\omega) = b_u(\omega) - \bar{b}_u(\omega) \eqsp , %\qquad \Delta \volat_u(\omega) = \volat_u(\omega) - \bar{\volat}(\omega) = 0 \eqsp .
  \end{align}
  where $s_k = \max(s, t_k)$.
  % \begin{align}
  %   &b_u(\omega) = \beta_{T-u}( \omega_u + 2 \nabla \log p_{T-u}(\omega_u)) \eqsp , \qquad \bar{b}_u(\omega) = \beta_{T-s_k}(\omega_{s_k} + 2 \bm{s}(T -s_k, \omega_{s_k})) \eqsp , \\
  %   &\volat_u(\omega) = \sqrt{2 \beta_{T-u}} \eqsp , \qquad  \bar{\volat}_u(\omega) = \sqrt{2 \beta_{T-t_u}} \eqsp , \\
  %   &\Delta b_u(\omega) = b_u(\omega) - \bar{b}_u(\omega) \eqsp , \qquad \Delta \volat_u(\omega) = \volat_u(\omega) - \bar{\volat}(\omega) \eqsp .
  % \end{align}
  We now provide upper bounds on $\Delta b$.  We introduce the intermediate
  drift functions $\drifta, \driftb, \driftc, \driftd$ such that $\drifta = b$
  and $\driftd = \bar{b}$. In addition, for any $s, u \in \coint{0,T}$ such that
  $u \geq s$, $u \in \coint{s_k, t_{k+1}}$ for some $k \in \{0, \dots, K\}$ and
  for any
  $\omega = (\omega_v)_{v \in \ccint{s,T}} \in \rmc(\ccint{s,T}, \rset^d)$ we
  have
  \begin{align}
    &\driftb_u(\omega) = \beta_{T-u}( \omega_u + 2 \nabla \log p_{T-s_k}(\omega_{u})) \eqsp , \qquad \driftc_u(\omega) = \beta_{T-u}(\omega_{u} + 2 \nabla \log p_{T-s_k}(\omega_{s_k})) \eqsp , \\
    &\Deltaab = \drifta - \driftb \eqsp , \qquad \Deltabc = \driftb - \driftc \eqsp , \qquad \Deltacd = \driftc - \driftd  \eqsp ,
  \end{align}
  where $s_k = \max(s, t_k)$.  We have that
\begin{equation}
  \label{eq:ineq_delta}
  \normLigne{\Delta b} \leq \normLigne{\Deltaab} + \normLigne{\Deltabc} + \normLigne{\Deltacd} \eqsp .
\end{equation}
In the rest of this section, we control each term on the right hand side of
\eqref{eq:ineq_delta}.

\begin{lemma}
  \label{lemma:controlab}
  For any $s, u \in \coint{0,T}$ such that $u \geq s$,
  $u \in \coint{s_k, t_{k+1}}$ for some $k \in \{0, \dots, K\}$ and
  $\omega = (\omega_v)_{v \in \ccint{s,T}} \in \rmc(\ccint{s,T}, \rset^d)$ we
  have
\begin{equation}
  \textstyle{
    \normLigne{\Deltaab_u(\omega)}  \leq 2  \sup_{v \in \ccint{T-u, T-t_k}} (\beta_{v}^2 /\sigma_{v}^6) (2 + \diam(\M)^2)(\diam(\M) + \normLigne{\omega_u}) \gamma_k  \eqsp .
    }
\end{equation}
\end{lemma}

\begin{proof}
  Assume that $s \leq t_k$. Then, we have
  \begin{align}
    \normLigne{\Deltaab_u(\omega)} &\leq 2 \beta_{T-u} \normLigne{\nabla \log p_{T-u}(\omega_{u}) - \nabla \log p_{T-t_k}(\omega_{u})} \\
   &\textstyle{\leq 2 \beta_{T-u} \gamma_k \sup_{v \in \ccint{T-u, T-t_k}} \normLigne{\partial_v \nabla \log p_{T-v}(\omega_u)}}  \eqsp . 
\end{align}
Using \Cref{lemma:control_time_space_der}, we have that
\begin{equation}
\textstyle{  \normLigne{\Deltaab_u(\omega)} \leq 2  \beta_{T-u} \sup_{v \in \ccint{T-u, T-t_k}} (\beta_{v} /\sigma_{v}^6) (2 + \diam(\M)^2)(\diam(\M) + \normLigne{\omega_{u}}) \gamma_k \eqsp ,}
\end{equation}
which concludes the proof in the case where $s \leq t_k$. The case where
$s \geq t_k$ is similar and left to the reader.
\end{proof}

\begin{lemma}
  \label{lemma:controlbc}
  For any $s, u \in \coint{0,T}$ such that $u \geq s$,
  $u \in \coint{s_k, t_{k+1}}$ for some $k \in \{0, \dots, K\}$ and
  $\omega = (\omega_v)_{v \in \ccint{s,T}} \in \rmc(\ccint{s,T}, \rset^d)$ we have
  \begin{equation}
    \normLigne{\Deltabc_u(\omega)} \leq 2 (\beta_{T-u} /\sigma_{T-u}^4)(1 + \diam(\M)^2) \normLigne{\omega_u - \omega_{s_k}} \eqsp ,
  \end{equation}
  where $s_k = \max(s, t_k)$.
\end{lemma}

\begin{proof}
  Assume that $s \leq t_k$. We have
  \begin{align}
    \textstyle{
      \normLigne{\Deltabc_u(\omega)}} &\leq \textstyle{2 \beta_{T-u} \normLigne{\nabla \log p_{T-t_k}(\omega_{t_k}) - \nabla \log p_{T-t_k}(\omega_{u})}} \\
    &\leq \textstyle{ 2 \beta_{T-u} \sup_{v \in \ccint{u, T-t_k}} \normLigne{\nabla^2 \log p_{T-t_k}(\omega_v)} \normLigne{\omega_{u} - \omega_{t_k}} \eqsp .
      }
  \end{align}
  Using \Cref{lemma:control_hessian} we have that
  \begin{equation}
    \normLigne{\Deltabc_u(\omega)} \leq 2 (\beta_{T-u} /\sigma_{T-u}^4)(1 + \diam(\M)^2) \normLigne{\omega_u - \omega_{t_k}} \eqsp ,
  \end{equation}
  which concludes the proof in the case where $s \leq t_k$. The case where
$s \geq t_k$ is similar and left to the reader.
\end{proof}

Finally, combining \Cref{lemma:controlab}, \Cref{lemma:controlbc} and
\Cref{assum:score_control} in \eqref{eq:ineq_delta}, we get that for any
$s, u \in \coint{0,T}$ such that $u \geq s$, $u \in \coint{s_k, t_{k+1}}$ for
some $k \in \{0, \dots, K\}$ and
$(\omega_v)_{v \in \ccint{s,T}} \in \rmc(\ccint{s,T}, \rset^d)$ we have
\begin{align}
  \label{eq:control_b}
  \normLigne{\Delta b_u(\omega)} &\leq \textstyle{ 2  \sup_{v \in \ccint{T-t_{k+1}, T-t_k}} (\beta_{v}^2 /\sigma_{v}^6) (2 + \diam(\M)^2)(\diam(\M) + \normLigne{\omega_{u}})\gamma_k } \\
                                 & \qquad \qquad + 2 (\beta_{T-u} /\sigma_{T-u}^4)(1 + \diam(\M)^2) \normLigne{\omega_u - \omega_{s_k}} \\
  & \qquad\qquad +2 \beta_{T-u} \Mtt (1 + \normLigne{\omega_u})/\sigma_{T-u}^2 \eqsp ,
\end{align}
where $s_k = \max(s, t_k)$.

  % and $\Delta \volat$. We
  % start by giving a bound on $\Delta \volat$.

  % \begin{lemma}
  %   $u \in \coint{0,T}$ such that $u \in \coint{t_k, t_{k+1}}$ for some
  %   $k \in \{0, \dots, K\}$ and
  %   $(\omega_v)_{v \in \ccint{s,u}} \in \rmc(\ccint{s,u}, \rset^d)$ we have
  %   \begin{equation}
  %     \textstyle{ \Delta \volat_u(\omega) \leq (1/\sqrt{2}) \gamma_k \sup_{s \in \ccint{T - t_{k+1}, T -t_k}} \absLigne{\beta'_s/\beta_s^{1/2}} \eqsp . }
  %   \end{equation}
  % \end{lemma}
The following proposition controls the local error
between the continuous-time backward process and the interpolation of the
discretized one where the true score is replaced by the approximation $\bm{s}$.

\begin{proposition}
  \label{prop:local-error-control}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:score_control}, \rref{assum:step_size}. In addition, assume that
  $\delta, \Mtt, \gamma_K \leq 1/32$.  Then, we have for any $s, u \in \ccint{0,t_K}$ with
  $u \geq s$
  \begin{equation}
    \expeLigne{\normLigne{\Delta b_u((\bbfY_{s,v})_{v \in \ccint{s,T}})}} \leq \Ctt_0 (T-t_K+\bar{\beta})^2 (\Mtt + \delta^{1/2}) /(T-t_K)^2  \eqsp ,
\end{equation}
where $\bbfY_{s,s} \sim \mathrm{N}(0, \Id)$ and
\begin{equation}
  \label{eq:Ctt0_def}
  \Ctt_0 = (1 + \bar{\beta})^{7/2}(4 + 256 d + 43664 (1+\diam(\M))^4) \eqsp . 
\end{equation}
\end{proposition}

\begin{proof}
  % Since for any $s \in \ccint{0,T}$, $\absLigne{\beta'_s} \leq \xi$ we have
  % that for any $u, v \in \coint{0,T}$ such that $u \in \coint{t_k, t_{k+1}}$
  % \begin{equation}
  %   \beta_{T-u} \leq \beta_{T-v} + \gamma_k \xi \eqsp .
  % \end{equation}
  Let $s, u \in \ccint{0,t_K}$ with $u \geq s$. In what follows, for ease of
  notation, we denote for any $k \in \{0, \dots, K\}$
\begin{equation}
 \textstyle{\kappa_k = \sup_{v \in \ccint{T-t_{k+1}, T-t_k}} \beta_{v} /
\sigma_{v}^2 \eqsp . } 
\end{equation}
  There exists $k \in \{0, \dots, K-1\}$ such that $u \in \ccint{t_k,
    t_{k+1}}$. Assume that $s \leq t_k$.  Recall that using
  \eqref{eq:control_b}, we have that for any
  $\omega = (\omega_v)_{v \in \ccint{s,T}} \in \rmc(\ccint{s,T}, \rset^d)$
\begin{align}
  \label{eq:control_b_proof}
  \normLigne{\Delta b_u(\omega)} &\leq \textstyle{ 2   \sup_{v \in \ccint{T-t_{k+1}, T-t_k}} (\beta_{v}^2 /\sigma_{v}^6) (2 + \diam(\M)^2)(\diam(\M) + \normLigne{\omega_{u}})\gamma_k } \\
                                 & \qquad \qquad + 2 (\beta_{T-u} /\sigma_{T-u}^4)(1 + \diam(\M)^2) \normLigne{\omega_u - \omega_{t_k}} \\
                                 & \qquad \qquad +2 \beta_{T-u} \Mtt (1 + \normLigne{\omega_u})/\sigma_{T-u}^2 \\
&\leq \textstyle{ 2  (\kappa_k^2/\sigma_{T-t_{k+1}}^2)\gamma_k (2 + \diam(\M)^2)(\diam(\M) + \normLigne{\omega_{u}}) } \\
                                 & \qquad \qquad + 2 \kappa_k^2 (1 + \diam(\M)^2)  \normLigne{\omega_u - \omega_{t_k}}/\beta_{T-u}  +2 \kappa_k \Mtt (1 + \normLigne{\omega_u})\eqsp .   
\end{align}
Combining this result with \Cref{lemma:control_growth_discrete_process}, its
following remark and \Cref{lemma:lipschitz-behavior}, we get that
\begin{align}
  \expeLigne{\normLigne{\Delta b_u((\bbfY_{s,v})_{v \in \ccint{s,T}})}} &\leq  2  (\kappa_k^2/\sigma_{T-t_{k+1}}^2)\gamma_k (2 + \diam(\M)^2)(\diam(\M) + \Ktt_0^{1/2}) \\
  &+ 2 \kappa_k^2 (1 + \diam(\M)^2) \Ltt_0^{1/2} \bar{\beta}^{3/2} \gamma_k^{1/2} + 2\kappa_k \Mtt (1+\Ktt_0^{1/2}) \eqsp . 
\end{align}
Denoting
$\Ctt = 2 (2 + \diam(\M)^2)(\diam(\M) + \Ktt_0^{1/2}) + 2 \Ltt_0^{1/2} \bar{\beta}^{3/2} (1 + \diam(\M)^2) + 2 (1 +
\Ktt_0^{1/2})$, we get that
\begin{equation}
  \expeLigne{\normLigne{\Delta b_u((\bbfY_{s,v})_{v \in \ccint{s,T}})}} \leq \Ctt ( (\kappa_k^2/\sigma_{T-t_{k+1}}^2)\gamma_k + \kappa_k^2 \gamma_k^{1/2} + \Mtt \kappa_k) \eqsp .
\end{equation}
Combining this result, \rref{assum:step_size} and \Cref{lemma:kappa_control} we have
  \begin{align}
    \expeLigne{\normLigne{\Delta b_u((\bbfY_{s,v})_{v \in \ccint{s,T}})}} &\leq \Ctt (1 + \bar{\beta})^2 (1+\bar{\beta}/(T-t_K))^2 (\delta^{1/2} + \Mtt ) \\
    & \qquad + \Ctt (1 + \bar{\beta}) (1+\bar{\beta}/(T-t_K)) (\delta/\sigma_{T-t_K}^2) \\
                                                                          &\leq \Ctt (1 + \bar{\beta})^2 (T-t_K+\bar{\beta})^2 (  \delta^{1/2} + \Mtt )/(T-t_K)^2 \\
    & \qquad + \Ctt (1 + \bar{\beta}) (T-t_K+\bar{\beta}) (\delta/\sigma_{T-t_K}^2)/(T-t_K) \eqsp . 
\end{align}
Finally, using \Cref{lemma:bound_sigma_t}, we have 
\begin{align}
  \sigma_{T-t_K}^{-2}& \textstyle{= (1 - \exp[-2\int_0^{T-t_K}\beta_s \rmd s ])^{-1}} \leq 1 + \bar{\beta}/(2(T-t_K)) \eqsp .
  \end{align}
  Therefore, using that $\gamma_K = T - t_K < 1$ we get that
  \begin{align}
    \expeLigne{\normLigne{\Delta b_u((\bbfY_{s,v})_{v \in \ccint{s,T}})}}
                                    &\leq \Ctt (1 + \bar{\beta})^2  (T-t_K+\bar{\beta})^2 ( \delta  + \delta^{1/2} + \Mtt )/(T-t_K)^2 \\
    &\leq 2 \Ctt (1 + \bar{\beta})^2  (T-t_K+\bar{\beta})^2 ( \delta^{1/2} + \Mtt )/(T-t_K)^2
\end{align}
which concludes the first part of the proof in the case where $s \leq t_k$.  The
same bound holds in the case where $s \geq t_k$. Finally, we conclude upon
noticing that $2 \Ctt (1 + \bar{\beta})^2 \leq \Ctt_0$ with $\Ctt_0$ given by
\eqref{eq:Ctt0_def}.
\end{proof}

We are now ready to control the global error between the backward process and
the interpolation of the associated discrete-time process where the true score
has been replaced by its approximation $\bm{s}$.

\begin{proposition}
  \label{prop:discretization_bound_final}
  Assume \rref{assum:manifold_hyp}, \rref{assum:assumption_beta},
  \rref{assum:score_control}, \rref{assum:step_size} and $\gamma_K =
  \vareps$. In addition, assume that $\vareps, \delta, \Mtt \leq 1/32$.  Then
  \begin{equation}
      \wassersteinD[1](\pi_\infty \rmQ_{t_K}, \pi_\infty \rmR_{K})  \leq  \Dtt_0 \exp[\diam(\M)^2(1+\bar{\beta})/(2\vareps)] (\Mtt + \delta^{1/2})/ \vareps^2  \eqsp ,
  \end{equation}
  where
  \begin{equation}
    \Dtt_0 = (1 + \bar{\beta})^7(8 + 512 d + 87328 (1 + \diam(\M))^4) (1 + \log(1 + \diam(\M))) \eqsp . 
  \end{equation}
\end{proposition}

\begin{proof}
  Using \Cref{prop:pierre-extended}, we have
    \begin{equation}
\textstyle{    \normLigne{\bfY_{t_K} - Y_K} = \normLigne{\bfY_{t_K} - \bbfY_{t_K}} \leq \int_0^{t_K} \normLigne{\nabla \bfY_{u,t_K}(\bbfY_{0,u})} \normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})} \rmd u } \eqsp .
\end{equation}
Combining this result, recalling that $t^\star$ is defined in
\eqref{eq:def_t_star} and \Cref{prop:control_gradient}, we get
    \begin{align}
      \textstyle{    \normLigne{\bfY_{t_K} - Y_K}} \leq & \textstyle{ \int_0^{t_K} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s \1_{\coint{0,t^\star}}(u)] \exp[(\diam(\M)^2/2)\sigma_{T-t_K}^{-2}]  \normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})} \rmd u } \\
                                                        &\leq \textstyle{ \exp[(\diam(\M)^2/2)\sigma_{T-t_K}^{-2}] (\int_{0}^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s] \normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})} \rmd u} \\
      & \qquad \qquad \textstyle{+ \int_{t^\star}^{t_K} \normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})} \rmd u ) \eqsp .  }
\end{align}
Using this result and \Cref{prop:local-error-control} we get
\begin{align}
  &\wassersteinD[1](\pi_\infty \rmQ_{t_K}, \pi_\infty \rmR_{K}) \leq \expeLigne{\normLigne{\bfY_{t_K} - Y_K}} \\
  &\qquad \leq \textstyle{ \exp[(\diam(\M)^2/2)\sigma_{T-t_K}^{-2}] (\int_{0}^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s] \expeLigne{\normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})}} \rmd u} \\
      & \qquad \qquad \textstyle{+ \int_{t^\star}^{t_K} \expeLigne{\normLigne{ \Delta b_u((\bbfY_{0,v})_{v\in \ccint{0,T}})}} \rmd u ) \eqsp .  } \\
  &\qquad \leq \textstyle{ \exp[(\diam(\M)^2/2)\sigma_{T-t_K}^{-2}] \Ctt_0 (T - t_K + \bar{\beta})^2 (\Mtt + \delta^{1/2}) /(T-t_K)^2 } \\
  & \qquad \qquad \textstyle{ \times (\int_0^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s]  \rmd u + t_K - t^\star)}  \eqsp . \label{eq:bound_wasserstein_intermediate}
\end{align}
We have that
\begin{equation}
  \textstyle{ \int_0^{t^\star} \exp[-(1/2) \int_{T-t^\star}^{T-u} \beta_s \rmd s]  \rmd u \leq \int_0^{t^\star} \exp[-(t^\star -u)/(2\bar{\beta})]  \rmd u \leq 2 \bar{\beta} \eqsp . } \label{eq:bound_integration}
\end{equation}
In addition, using \eqref{eq:def_t_star}  we have
\begin{equation}
  t_K - t^\star = T - \vareps - T +2 \bar{\beta} (1 + \log(1 + \diam(\M))) \leq 2 \bar{\beta} (1 + \log(1 + \diam(\M)))  \eqsp . \label{eq:bound_tk_tstar}
\end{equation}
Finally, using \Cref{lemma:bound_sigma_t}, we have that
$\sigma_{T-t_K}^{-2} \leq (1 + \bar{\beta})/\vareps$. Combining this result,
\eqref{eq:bound_integration} and \eqref{eq:bound_tk_tstar} in
\eqref{eq:bound_wasserstein_intermediate} we get
\begin{equation}
  \wassersteinD[1](\pi_\infty \rmQ_{t_K}, \pi_\infty \rmR_{K}) \leq 2 \Ctt_0 \exp[\diam(\M)^2(1+\bar{\beta})/(2\vareps)](1 + \bar{\beta})^3 (1 + \log(1 + \diam(\M))) (\Mtt + \delta^{1/2})/ \vareps^2 \eqsp ,
\end{equation}
which concludes the proof.
%   &\qquad \leq \textstyle{ \exp[(1/2)\sigma_{T-t_K}^{-2}] (1 + \Dtt) \Ctt (\Mtt + \delta^{1/2}) /(T-t_K)^2  (1 + t_K - t^\star)} \eqsp ,q:
% \end{align}
% where $\Dtt_0 = \int_0^{T} \exp[-(1/2) \int_0^{T-u} \beta_s \rmd s] \rmd u $. We conclude upon using that 
% \begin{equation}
%   t_K -t^\star \leq (\bar{\beta}/2) \log(2\{ -\diam(\M)^2/2 - 1/2 +(1 + \diam(\M)^2/2 +\diam(\M)^4/4)^{1/2}\}) \eqsp . 
% \end{equation}

\end{proof}


\subsection{Control of $\wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T - t_K})$}
\label{sec:convergence_backward}
In this section, we focus on the following error
$\wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K})$. First, note that
$\pi \Pker_{T-t_K} = \pi \Pker_{T} \Qker_{t_K}$. Therefore, using
\Cref{prop:wasserstein_forward}, we have
\begin{equation}
\label{eq:convergence_bound_backward_inter}  
  \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K}) = \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T} \Qker_{t_K}) \leq \exp[(1/2)\sigma_{T-t_K}^{-2}] \wassersteinD[1](\pi \Pker_T, \pi_\infty) \eqsp . 
\end{equation}
To control $\wassersteinD[1](\pi \Pker_T, \pi_\infty)$, we use a
synchronous coupling, i.e. we set $(\bfY_t, \bfZ_t)_{t \in \ccint{0,T}}$ such that
\begin{equation}
  \rmd \bfY_t = - \beta_t \bfY_t \rmd t + \sqrt{2 \beta_t} \rmd \bfB_t \eqsp , \qquad 
  \rmd \bfZ_t = - \beta_t \bfZ_t \rmd t + \sqrt{2 \beta_t} \rmd \bfB_t \eqsp ,
\end{equation}
where $(\bfB_t)_{t \in \ccint{0,T}}$ is a $d$-dimensional Brownian motion and
$\bfY_0 \sim \pi$, $\bfZ_0 \sim \pi_\infty$. We have that for any
$t \in \ccint{0,T}$, $\bfZ_t \sim \pi_\infty$. In addition, denoting
$u_t = \expeLigne{\normLigne{\bfY_t - \bfZ_t}}$ for any $t \in \ccint{0,T}$, we
have that $\textstyle{u_t \leq u_0 \exp[-\int_0^t \beta_s \rmd s] \eqsp . }$
Therefore, combining this result and
\eqref{eq:convergence_bound_backward_inter}, we get that
\begin{equation}
  \label{eq:convergence_bound_backward}
  \textstyle{
    \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K}) \leq \exp[(1/2)\sigma_{T-t_K}^{-2}] \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) \eqsp .
    }
  \end{equation}
Therefore, using \Cref{lemma:bound_sigma_t}, we have
\begin{equation}
  \textstyle{
    \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{T-t_K}) \leq \exp[(1 + \bar{\beta})\diam(\M)^2/(2\vareps)] \exp[-T/\bar{\beta}](\sqrt{d} + \diam(\M)) \eqsp . }
\end{equation}

\subsection{Control of $\wassersteinD[1](\pi \Pker_{T - t_K}, \pi)$ and conclusion}
\label{sec:noising_error_conclusion}

In this section, we focus on the error $\wassersteinD[1](\pi, \pi\Pker_{T-t_K})$
and conclude the proof.
First, we have that
\begin{equation}
  \wassersteinD[1](\pi, \pi\Pker_{T-t_K}) \leq \expeLigne{\normLigne{X - m_{T-t_K} X + \sigma_{T-t_K} Z}} \eqsp ,
\end{equation}
with $X \sim \pi$ and $Z \sim \mathrm{N}(0, \Id)$. Hence, using $1 - m_{T-t_K} \leq \sigma_{T-t_K}$, we get
\begin{equation}
  \textstyle{
    \wassersteinD[1](\pi, \pi\Pker_{T-t_K}) \leq \diam(\M) (1 - m_{T-t_K}) + \sigma_{T-t_K} \sqrt{d} \leq (\diam(\M) + \sqrt{d}) \sigma_{T-t_K} \eqsp .
    }
  \end{equation}
  Using \Cref{lemma:bound_sigma_t} and this result we have
  \begin{equation}
    \label{eq:control_noising}
  \textstyle{
    \wassersteinD[1](\pi, \pi\Pker_{T-t_K}) \leq (2 \bar{\beta})^{1/2} (\diam(\M) + \sqrt{d}) \vareps^{1/2} \eqsp .
  }
  \end{equation}
  Combining this result, \eqref{eq:convergence_bound_backward} and
  \Cref{prop:discretization_bound_final} in \eqref{eq:decomposition} we get that
  \begin{align}
    \wassersteinD[1](\pi_\infty \Rker_K, \pi)  &\leq \Dtt_0 (\exp[(1+\bar{\beta})\diam(\M)^2/(2\vareps)] (\Mtt + \delta^{1/2})/ \vareps^2 \\
    & \qquad + \exp[(1+\bar{\beta})\diam(\M)^2/(2\vareps)]\exp[-T/\bar{\beta}] + \vareps^{1/2}) \eqsp , 
  \end{align}
  which concludes the proof.
% \begin{align}
%   \wassersteinD[1](\pi_\infty \Rker_K, \pi) &\leq \wassersteinD[1](\pi_\infty \Rker_K, \pi_\infty \Qker_{t_K}) + \wassersteinD[1](\pi_\infty \Qker_{t_K}, \pi \Pker_{t_K}) + \wassersteinD[1](\pi \Pker_{t_K}, \pi) \\
%                                             &\leq \textstyle{ \exp[(1/2)\sigma_{T-t_K}^{-2}]} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2) /((T-t_K)^2\beta_{T-t_K})  (1 + t_K - t^\star) \\
%                                             & \qquad \textstyle{ + \exp[(1/2)\sigma_{T-t_K}^{-2}] \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\sigma_{T-t_K} \eqsp . } \label{eq:intermediate_bound_tb_ta}
% \end{align}
% In order to conclude the proof we know control $t_K - t^\star$ as well as
% $\sigma_{T-t_K}^2$.  Recall that
% $t_K = T - (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps))$ and that using \valentin{def t star}
% % \eqref{eq:t_star_def}
% , we have
% \begin{equation}
%   t^\star = T - (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \vareps +(1 + \vareps \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\vareps)) \eqsp . 
% \end{equation}
% \valentin{remove the eps dependency in ta}
% Therefore, we get that
% \begin{equation}
%   t_K -t^\star \leq (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \vareps +(1 + \vareps \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\vareps)) \eqsp . 
% \end{equation}
% Therefore, combining this result and \Cref{lemma:bound_sigma_t} in
% \eqref{eq:intermediate_bound_tb_ta}, we get that
% \begin{align}
%   &\wassersteinD[1](\pi_\infty \Rker_K, \pi)  \leq \textstyle{ \exp[(1/2)\sigma_{T-t_K}^{-2}]} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2) /((T-t_K)^2\beta_{T-t_K})  (1 + t_K - t^\star) \\
%                                              & \qquad \textstyle{ + \exp[(1/2)\sigma_{T-t_K}^{-2}] \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\sigma_{T-t_K} \eqsp . } \\
%                                              &\leq \textstyle{ 4\bar{\beta}^3 \exp[\bar{\beta}/(2\vareps)]\vareps^{-2}} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2)  \\
%   & \qquad \times (1 +  (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \eta +(1 + \eta \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\eta))) \\
%                                             & \qquad \textstyle{ + \exp[\bar{\beta}/(2\vareps)] \exp[-T/\bar{\beta}] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\vareps \eqsp , }
% \end{align}
% which concludes the proof upon letting
% \begin{align}
%   A = ... 
% \end{align}

 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/schedule.tex <==
\section{Assumptions on the schedule}
\label{sec:assumptions-schedule}

In what follows, we consider three schedules commonly used in practice:
\begin{enumerate*}[label=(\alph*)]
\item the constant schedule,
\item the linear schedule,
\item the cosine schedule.
\end{enumerate*}
We show that \Cref{assum:assumption_beta} is satisfied in all these cases. We
consider a generalized version of the cosine schedule which makes it
differentiable by replacing the hard clamping by a soft version with level $r>0$
(note that letting $r \to 0$ we recover the original cosine schedule). The
constant schedule is defined by $\beta_s = \beta_0$ for all $s \in
\ccint{0,T}$. The linear schedule was introduced in \citet{ho2020denoising} and
is defined by $\beta_s = \beta_0 + (\beta_T - \beta_0)t/T$ with
$\beta_T > \beta_0 >0$. Finally, the cosine schedule was introduced in
\cite[Equation (17)]{nichol2021improved} in discrete-time and can be defined as
follows in continuous-time
\begin{equation}
  \beta_t = \softmin_{r}(1,\lim_{h \to 0} (\bar{\alpha}_{t-h} - \bar{\alpha}_t)/(\bar{\alpha}_{t-h} h))  = \softmin_{r}(1,f)_t \eqsp , \qquad f(t)= - \bar{\alpha}'_t / \bar{\alpha}_t \eqsp ,
\end{equation}
with $\bar{\alpha}$ defined as
\begin{equation}
  \bar{\alpha}_t  = \cos((t/T + \eta)/(1+\eta)(\uppi/2))^2/\cos(\eta/(1+\eta)(\uppi/2))^2 \eqsp ,
\end{equation}
and where $\eta \geq 0$, $r >0$ are parameters and for any $f_1, f_2 : \ \ccint{0,T} \to \rset_+$ 
\begin{equation}
  \softmin_r(f_1,f_2)_t = -r\log(\exp[-f_1(t)/r] + \exp[-f_2(t)/r]) \eqsp . 
\end{equation}
In the special case where $f_1 = 1$ we have
\begin{equation}
  \softmin_r(1,f_2)_t = 1 -r \log(1 + \exp[(1-f_2(t))/r]) \eqsp ,
\end{equation}
We have 
\begin{equation}
  \bar{\alpha}'(t)/\bar{\alpha}(t) = -\uppi/(T(1+\eta)) \tan((t/T + \eta)/(1+\eta)(\uppi/2)) \eqsp . 
\end{equation}
In particular, $t \mapsto \beta_t$ is increasing and bounded above and below on $\ccint{0,T}$.

Finally, we end this section by remarking that if one aims at studying the
Euler-Maruyama discretization of the approximate backward, \ie the process
given by \eqref{eq:classical_EM_disc} then one needs to also assume some
Lipschitz property on the schedule $s \mapsto \beta_s$. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/stochastic-interpolation.tex <==
  \section{A stochastic interpolation formula}
\label{sec:stoch-interp-form}

In this section, we present a formula first introduced in \citet{del2019backward}
which is a stochastic extension of the Alekseev--Gr\"obner formula
\citep{alekseev1961estimate}.  We recall the definition of the stochastic flows
$(\bfY_{s,t}^x)_{s, t \in \ccint{0,T}}$ and the interpolation of its
discretization $(\bbfY_{s,t}^x)_{s, t \in \ccint{0,T}}$, for any $x \in \rset^d$
\begin{equation}
  \textstyle{
    \rmd \bfY_{s,t}^x = \beta_{T-t} \{ \bfY_{s,t}^x + 2 \nabla \log q_{T-t}(\bfY_{s,t}^x) \} \rmd t + \sqrt{2 \beta_{T-t}} \rmd \bfB_t \eqsp , \qquad \bfY_{s,s}^x = x \eqsp .
    }
\end{equation}
and 
\begin{equation}
  \textstyle{
    \rmd \bbfY_{s,t}^x = \beta_{T-t} \{ \bbfY_{s, t}^x + 2 \bm{s}(T-t_k, \bbfY_{s, t_k}^x) \} \rmd t + \sqrt{2\beta_{T-t}} \rmd \bfB_t \eqsp , \qquad \bbfY_{s,s}^x = x \eqsp .
    }
\end{equation}
The following proposition is a straightforward application of \cite[Theorem
1.2]{del2019backward}. Note that these results apply since the drift and the
volatility of the backward processes have bounded differential up to order
three, see \Cref{lemma:higher_order}.

\begin{proposition}
  \label{prop:pierre-extended_appendix}
  Assume \rref{assum:manifold_hyp}. Then, for any $s, t \in \coint{0,T}$ with $s<t$ and $x \in \rset^d$
  \begin{equation}
\textstyle{    \bfY_{s,t}^x - \bbfY_{s,t}^x = \int_s^t \nabla \bfY_{u,t}(\bbfY_{s,u})^\top \Delta b_u((\bbfY_{s,v})_{v\in \ccint{s,u}}) \rmd u } \eqsp , %+  \int_s^t \nabla \bfY_{u,t}(\bbfY_{s,u})^\top \Delta \volat_u((\bbfY_{s,v})_{v\in \ccint{s,u}}) \rmd \bfB_u \eqsp ,  }
\end{equation}
where for any $u \in \coint{0,T}$ such that $u \in \coint{t_k, t_{k+1}}$ for
some $k \in \{0, \dots, K-1\}$ and $(\omega_v)_{v \in \ccint{s,u}} \in \rmc(\ccint{s,u}, \rset^d)$ we have 
  \begin{align}
    &b_u(\omega) = \beta_{T-u}( \omega_u + 2 \nabla \log q_{T-u}(\omega_u)) \eqsp , \qquad \bar{b}_u(\omega) = \beta_{T-t_u}(\omega_{u} + 2 \bm{s}(T -t_k, \omega_{t_k})) \eqsp , \\
%    &\volat_u(\omega) = \sqrt{2 \beta_{T-u}} \eqsp , \qquad  \bar{\volat}_u(\omega) = \sqrt{2 \beta_{T-u}} \eqsp , \\
    &\Delta b_u(\omega) = b_u(\omega) - \bar{b}_u(\omega) \eqsp . %\qquad \Delta \volat_u(\omega) = \volat_u(\omega) - \bar{\volat}(\omega) = 0 \eqsp .
  \end{align}
\end{proposition}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arxiv/trash.tex <==











At this point, we emphasize that better control on the covariance term in the
  expansion of $\nabla^2 \log p_t$ might lead to better controls in
  \Cref{prop:control_gradient}. In particular, using a stronger assumption than
  \rref{assum:manifold_hyp} and quantitative parametric Laplace expansion
  techniques, we prove that the term $\exp[(1/2)\sigma_{T-t_1}^{-2]}$ can be
  replaced by. Finally, the following result will allow us to
  control the convergence of the backward process initialized at the Gaussian distribution
  \valentin{mettre le truc sur Laplace dans la conclusion}


I don't need the next lemma.
\begin{lemma}
  \label{item:bound_p_infty}
  Let $T \geq \log(2 \mathrm{diam}(\M)^2) + \log(2)/2$. Then, we have
  \begin{equation}    
    \textstyle{
      \int_{\rset^d} p_\infty(x_T)^2 / p_T^N(x_T) \rmd x_T \leq \Ctrois \eqsp , \qquad \int_{\rset^d} p_\infty(x_T)^2 / p_T(x_T) \rmd x_T \leq \Ctrois \eqsp . 
      }
    \end{equation}
    with $E_T  \sim C\exp[-T]$ when $T \to +\infty$ and $C \geq 0$.
  \end{lemma}

  Use Fatou to generalize to $p_t$
  
\begin{proof}
  Let $T \geq 0$, $\vareps >0$ and $x_T \in \rset^d$
  \begin{equation}
    \normLigne{x_T - \rme^{-T} x_0}^2 \leq (1 + \vareps) \normLigne{x_T}^2 + (1+1/\vareps) \rme^{-2T} \normLigne{x_0}^2 \eqsp . 
  \end{equation}
  Let $\vareps >0$ and $x_T \in \rset^d$, we have
  \begin{align}
    &\textstyle{
      p_T(x_T)^{-2} \leq \exp[(1+\vareps)/\sigma_T^2\normLigne{x_T}^2 ] }\\
    & \qquad \qquad \qquad \qquad \times \textstyle{(\int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/(2\sigma_T^2)\normLigne{x_0}^2]\rmd x_0)^{-2} (2\uppi\sigma_T^2)^d  \eqsp .
      }
  \end{align}
  For any $x_T \in \rset^d$, we have
  \begin{align}
    p_\infty(x_T)^2/p_T(x_T) &\leq \exp[\{-1+(1+\vareps)/(2\sigma_T^2)\}\normLigne{x_T}^2 ](2\uppi/\sigma_T^2)^{-d/2} \\ & \qquad \qquad \textstyle{ (\int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/(2\sigma_T^2)\normLigne{x_0}^2] \rmd x_0)^{-1}  \eqsp . }
  \end{align}
  In what follows, we set $\vareps = \rme^{-T}$. We have that
  \begin{equation}
    -1 + (1+\vareps)/(2\sigma_T^2) = (2\sigma_T^2)^{-1}(-2\sigma_T^2 + 1 + \vareps) = -(1 - 2\rme^{-T} + \vareps)/(2\sigma_T^2) = -(1 - \rme^{-T})/(2\sigma_T^2) \eqsp . 
  \end{equation}
  Therefore, we get that
  \begin{equation}
    \label{eq:UNO_de}
    \textstyle{
      \int_{\rset^d} \exp[\{-1+(1+\vareps)/(2\sigma_T^2)\}\normLigne{x_T}^2 ](2\uppi/\sigma_T^2)^{-d/2} \rmd x_T = (1 - \rme^{-T})^{-d/2} \eqsp .
      }
    \end{equation}
    In addition, we have that for any $R \geq 0$ using that $\sigma_T^2 \geq 1/2$ since $T \geq \log(2)/2$
    \begin{align}
      &\textstyle{
        \int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2\normLigne{x_0}^2] \rmd x_0 } \\
      & \qquad \qquad  \geq \textstyle{\probaLigne{X_0 \in \cball{0}{R}} \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2R^2]} \\ 
        & \qquad \qquad  \geq \textstyle{\probaLigne{X_0 \in \cball{0}{R}} \exp[-4\rme^{-T}R^2]
        } \label{eq:inter_DUO}
    \end{align}
    Now let $R^2 = \rme^T$. We obtain
    \begin{equation}
      \textstyle{
        \int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2\normLigne{x_0}^2] \rmd x_0 } \geq \probaLigne{X_0 \in \cball{0}{\rme^{T/2}}} \exp[-4] \eqsp . 
    \end{equation}
    In addition, using Markov inequality, we have
    \begin{equation}
      \probaLigne{X_0 \in \cball{0}{\rme^{T/2}}} = 1 - \probaLigne{\normLigne{X_0}^2 \geq \rme^T} \geq 1 - \expeLigne{\normLigne{X_0}^2} \rme^{-T} \geq 0 \eqsp . 
    \end{equation}
    Therefore, combining this result and \eqref{eq:inter_DUO}, we have
    \begin{equation}
      \label{eq:DUO_de}
      \textstyle{
        \int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2\normLigne{x_0}^2] \rmd x_0 } \geq \exp[-4] (1 - \expeLigne{\normLigne{X_0}^2} \rme^{-T}) > 0 \eqsp . 
    \end{equation}
    We conclude upon combining \eqref{eq:UNO_de} and \eqref{eq:DUO_de}.
  \end{proof}


\section{Entropy bounds and convergence of the backward process}

WE DONT NEED THE ENTROPY BOUNDS ! THE BACKWARD KERNEL CONVERGES

Second, we are going to bound the entropy between $p_t$ and $\pi_\infty$ the
Gaussian distribution with zero mean and identity covariance matrix. To do so,
we are going to provide lower and upper bound on the density.

\begin{lemma}
  Assume \rref{assum:manifold_hyp}. Then for any $t > 0$ we have that
  \begin{equation}
    \KLLigne{p_t^N}{p_\infty} \leq \Cdeux \eqsp , \qquad     \KLLigne{p_t}{p_\infty} \leq \Cdeux \eqsp ,
  \end{equation}
  where we recall that $p_\infty$ is the density w.r.t. the Lebesgue measure of
  the Gaussian distribution with zero mean and identity covariance matrix.
\end{lemma}

\begin{proof}
  Let $N \in \nset$. First, let us
  give an upper-bound $p_t^N$
  independent of $N \in \nset$. We
  have that for any
  $x_t \in \rset^d$
  \begin{equation}
    \label{eq:def_pt}
    p_t^N(x_t) = (1/N) \sum_{k=1}^N \exp[-\normLigne{x_t - m_t X^k}^2/(2 \sigma_t^2)] (2 \uppi \sigma_t^2)^{-d/2} \eqsp . 
  \end{equation}
  In addition, we have that for any $k \in \{1, \dots, N\}$
  \begin{align}
    \normLigne{x_t - m_t X^k}^2 &= \normLigne{x_t}^2 + m_t^2 \normLigne{X^k}^2 - 2m_t \langle x_t, X^k \rangle \geq (1/2) \normLigne{x_t}^2 - m_t^2 \normLigne{X^k}^2 \\
    &\geq (1/2) \normLigne{x_t}^2 - m_t^2 \mathrm{diam}(\M)^2 \eqsp .
  \end{align}
  Combining this result and \eqref{eq:def_pt} we get that
  \begin{equation}
    p_t^N(x_t) \leq q_t(x_t) = (2 \uppi \sigma_t^2)^{-d/2} \exp[-\normLigne{x_t}^2/(4\sigma_t^2)] \exp[m_t^2 \mathrm{diam}(\M)^2/(2\sigma_t^2)] \eqsp .
  \end{equation}
  Using this upper-bound we can now compute a lower-bound on the entropy of $p_t$.
  \begin{align}
    \mathrm{H}(p_t) &= -\int_{\rset^d} p_t(x_t) \log p_t(x_t) \rmd x_t \\
                    &\geq - \int_{\rset^d} \1_{p_t(x_t) \geq 1} p_t(x_t) \log p_t(x_t) \rmd x_t \\
                    &\geq - \int_{\rset^d} \1_{q_t(x_t) \geq 1} q_t(x_t) \log q_t(x_t) \rmd x_t \\
                    &\geq - \int_{\rset^d} q_t(x_t) \absLigne{ \log q_t(x_t)} \rmd x_t \\    
                    &\geq - 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] \expeLigne{\absLigne{\log q_t(X_t)}} \eqsp ,
  \end{align}
  where $X_t$ has Gaussian distribution with zero mean and covariance matrix $2\sigma_t^2 \Id$.
  We have that
  \begin{align}
    \expeLigne{\absLigne{\log q_t(X_t)}}& \leq \abs{(d/2)\log(2\uppi\sigma_t^2)} + m_t^2 \mathrm{diam}(\M)^2/ (2 \sigma_t^2) + d/2 
  \end{align}
  Therefore, we have that
  \begin{equation}
    \label{eq:entropy_bound}
    \mathrm{H}(p_t) \geq - 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] [\abs{(d/2)\log(2\uppi\sigma_t^2)} + m_t^2 \mathrm{diam}(\M)^2/ (2 \sigma_t^2) + d/2 ] \eqsp . 
  \end{equation}
  In addition, we have that
  \begin{equation}
    \label{eq:moment_bound}
    \int_{\rset^d} \normLigne{x_t}^2 p_t(x_t) \rmd x_t \leq 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] 2 d \sigma_t^2
  \end{equation}
  Hence, we get that 
  \begin{equation}
 \KLLigne{p_t^N}{p_\infty} \leq 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] \{ 2 d \sigma_t^2 + \abs{(d/2)\log(2\uppi\sigma_t^2)} + m_t^2 \mathrm{diam}(\M)^2/ (2 \sigma_t^2) + d/2 \} \eqsp .     
\end{equation}
Then using that $\pi_t^N$ weakly
converges to $\pi_t$ and using
\cite{dupuis2011weak} we get that the
same result holds replacing $p_t^N$
by $p_t$.
\end{proof}

Remark, choosing $t \geq (1/2) \log(1 + 1/2K)$ implies that $m_t / (2 \sigma_t^2) \leq K$.
Remark, can we remove the dependency w.r.t the dimension by choosing something else instead of $1/2$?


  
  We have the following proposition.

  \begin{proposition}
      Assume \rref{assum:manifold_hyp}.
    \begin{equation}
      \wassersteinD[1](\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{t_0}) \leq C_2 C_3  (...) \exp[-(T-t_0)] \eqsp . 
    \end{equation}
  \end{proposition}

  \begin{proof}
    Let $\nu$ be the optimal
    coupling between
    $\pi_\infty \rmQ_{T-t_0}$
    and $\pi \rmP_{t_0}$
    w.r.t. the total variation
    distance. Using the
    Cauchy-Schwarz inequality we
    have
    \begin{align}
      \wassersteinD[1](\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{t_0}) &\leq \int_{\rset^d \times \rset^d} \normLigne{x-y} \rmd \nu(x,y) \\
                                                                            &\leq \sqrt{2} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \tvnormLigne{\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{t_0}}^{1/2} \\
                                                                &\leq \sqrt{2} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \tvnormLigne{\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{T} \rmQ_{T-t_0}}^{1/2}      \\
                                                                &\leq \sqrt{2} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \tvnormLigne{\pi_\infty - \pi \rmP_{T}}^{1/2}            \\
                                                                &\leq 2^{3/4} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \KLLigne{\pi \rmP_{T}}{\pi_\infty}^{1/4}  \\
      &\leq 2^{3/4} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \rme^{-(T-t_0)/4} \KLLigne{\pi \rmP_{t_0}}{\pi_\infty}^{1/4} \eqsp . 
    \end{align}
  \end{proof}


  (\bbfY_{s,v})_{v\in \ccint{s,u}}
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proof.tex <==
% \section{Stability and growth of the backward process}
% \label{sec:stab-backw-proc}







%   \section{Backward interpolation error}
% \label{sec:backw-interp-error}

% In this section, we focus on the following error
% $\wassersteinD[1](\pi_\infty \rmQ_{t_1}, \pi_\infty \rmR_{N})$. To control
% this term, we use \Cref{prop:pierre-extended} together with the controls derived
% in \Cref{sec:stab-backw-proc}.

% \subsection{Drift controls}
% \label{sec:drift-decomp-contr}

% We start with the following useful lemma.

% % \begin{lemma}
% %   \label{lemma:condition_beta_integral}
% %   Assume \rref{assum:assumption_beta}. Then for any $t \in \ccint{0,T}$, $\textstyle{\int_0^t \beta_s \rmd s \geq t \beta_t / (1 + C)}$.
% % \end{lemma}

% % \begin{proof}
% %   We have that for any $t \in \ocint{0,T}$, $\beta_t' \leq C \beta_t /t$ using
% %   \rref{assum:assumption_beta}. Hence, we get that for any $t \in \ocint{0,T}$,
% %   $C \beta_t \geq t\beta_t'$ and hence $(1+C)\beta_t \geq
% %   (t\beta_t)'$. Therefore, we have that for any $t \in \ccint{0,T}$,
% %   $\textstyle{\int_0^t \beta_s \rmd s \geq t \beta_t / (1 + C)}$, which
% %   concludes the proof.
% % \end{proof}

% The following lemma controls the growth of $\kappa_k$ w.r.t. $k \in \{0, \dots, N-1\}$.


% \valentin{faire les changements plus haut t0 devient ta et t1 devient tb}

%   \section{Wasserstein approximation and conclusion}
% \label{sec:wass-appr-concl}

% In this section, we focus on the error $\wassersteinD[1](\pi, \pi\Pker_{T-t_b})$
% and conclude the proof.
% First, we have that
% \begin{equation}
%   \wassersteinD[1](\pi, \pi\Pker_{T-t_b}) \leq \expeLigne{\normLigne{X - m_{T-t_b} X + \sigma_{T-t_b} Z}} \eqsp ,
% \end{equation}
% with $X \sim \pi$ and $Z \sim \mathrm{N}(0, \Id)$. Hence, we have 
% \begin{equation}
%   \wassersteinD[1](\pi, \pi\Pker_{T-t_b}) \leq \diam(\M) (1 - m_{T-t_b}) + \sigma_{T-t_b} d \leq (\diam(\M) + d) \sigma_{T-t_b} \eqsp .
% \end{equation}
% Combining this result, \eqref{eq:convergence_bound_backward} and
% \Cref{prop:discretization_bound_final} we get that
% \begin{align}
%   \wassersteinD[1](\pi_\infty \Rker_N, \pi) &\leq \wassersteinD[1](\pi_\infty \Rker_N, \pi_\infty \Qker_{t_b}) + \wassersteinD[1](\pi_\infty \Qker_{t_b}, \pi \Pker_{t_b}) + \wassersteinD[1](\pi \Pker_{t_b}, \pi) \\
%                                             &\leq \textstyle{ \exp[(1/2)\sigma_{T-t_b}^{-2}]} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2) /((T-t_b)^2\beta_{T-t_b})  (1 + t_b - t_a) \\
%                                             & \qquad \textstyle{ + \exp[(1/2)\sigma_{T-t_b}^{-2}] \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\sigma_{T-t_b} \eqsp . } \label{eq:intermediate_bound_tb_ta}
% \end{align}

% In order to conclude, we now link $t$ and $\sigma_{T-t}^2$ with the following lemma.

% % \begin{lemma}
% %   \label{lemma:bound_sigma_t}
% %   Let $t = (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps))$ then $\sigma_{t}^2 \leq \vareps$ and $\sigma_t^2 \geq \vareps/\bar{\beta}^2$. We also have that $t \geq \vareps/(2\bar{\beta})$.
% % \end{lemma}

% % \begin{proof}
% %   First, we have that
% %   \begin{equation}
% %     \textstyle{\sigma_t^2 = 1 - \exp[-2\int_0^t \beta_s \rmd s] \leq 1 - \exp[-\log(1 + \vareps/(1-\vareps))]} \leq \vareps \eqsp . 
% %   \end{equation}
% %   Then, we have
% %   \begin{equation}
% %     \textstyle{\sigma_t^2 = 1 - \exp[-2\int_0^t \beta_s \rmd s] \geq 1 - \exp[-\bar{\beta}^{-2}\log(1 + \vareps/(1-\vareps))]} \geq 1 - (1-\vareps)^{\bar{\beta}^{-2}} \eqsp . 
% %   \end{equation}
% %   We conclude upon using that $(1-\vareps)^{\bar{\beta}^{-2}} \leq 1 - \vareps/\bar{\beta}^2$.
% % \end{proof}

% \valentin{modifier la suite en fonction !}

% In what follows, we set
% $t_b = T - (1/(2\bar{\beta}))\log(1 + \vareps/(1-\vareps))$ and recall that
% using \eqref{eq:t_a_def}, we have
% \begin{equation}
%   t_a = T - (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \vareps +(1 + \vareps \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\vareps)) \eqsp . 
% \end{equation}
% \valentin{remove the eps dependency in ta}
% Therefore, we get that
% \begin{equation}
%   t_b -t_a \leq (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \vareps +(1 + \vareps \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\vareps)) \eqsp . 
% \end{equation}
% \valentin{this gives a natural condition on $T$ to be large enough so that everything is positive (when I say everything I am talking about ta)}
% Therefore, combining this result and \Cref{lemma:bound_sigma_t} in
% \eqref{eq:intermediate_bound_tb_ta}, we get that
% \begin{align}
%   &\wassersteinD[1](\pi_\infty \Rker_N, \pi)  \leq \textstyle{ \exp[(1/2)\sigma_{T-t_b}^{-2}]} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2) /((T-t_b)^2\beta_{T-t_b})  (1 + t_b - t_a) \\
%                                              & \qquad \textstyle{ + \exp[(1/2)\sigma_{T-t_b}^{-2}] \exp[-\int_0^T \beta_t \rmd t] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\sigma_{T-t_b} \eqsp . } \\
%                                              &\leq \textstyle{ 4\bar{\beta}^3 \exp[\bar{\beta}/(2\vareps)]\vareps^{-2}} \Ctt(1 + \Dtt) (\Mtt + \delta + \delta^2)  \\
%   & \qquad \times (1 +  (\bar{\beta}/2) \log(\{ -\diam(\M)^2/2 - \eta +(1 + \eta \diam(\M)^2 +\diam(\M)^4/4)^{1/2}\}/(1-\eta))) \\
%                                             & \qquad \textstyle{ + \exp[\bar{\beta}/(2\vareps)] \exp[-T/\bar{\beta}] \wassersteinD[1](\pi, \pi_\infty) + (\diam(\M) + d)\vareps \eqsp , }
% \end{align}
% which concludes the proof.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> trash.tex <==











At this point, we emphasize that better control on the covariance term in the
  expansion of $\nabla^2 \log p_t$ might lead to better controls in
  \Cref{prop:control_gradient}. In particular, using a stronger assumption than
  \rref{assum:manifold_hyp} and quantitative parametric Laplace expansion
  techniques, we prove that the term $\exp[(1/2)\sigma_{T-t_1}^{-2]}$ can be
  replaced by. Finally, the following result will allow us to
  control the convergence of the backward process initialized at the Gaussian distribution
  \valentin{mettre le truc sur Laplace dans la conclusion}


I don't need the next lemma.
\begin{lemma}
  \label{item:bound_p_infty}
  Let $T \geq \log(2 \mathrm{diam}(\M)^2) + \log(2)/2$. Then, we have
  \begin{equation}    
    \textstyle{
      \int_{\rset^d} p_\infty(x_T)^2 / p_T^N(x_T) \rmd x_T \leq \Ctrois \eqsp , \qquad \int_{\rset^d} p_\infty(x_T)^2 / p_T(x_T) \rmd x_T \leq \Ctrois \eqsp . 
      }
    \end{equation}
    with $E_T  \sim C\exp[-T]$ when $T \to +\infty$ and $C \geq 0$.
  \end{lemma}

  Use Fatou to generalize to $p_t$
  
\begin{proof}
  Let $T \geq 0$, $\vareps >0$ and $x_T \in \rset^d$
  \begin{equation}
    \normLigne{x_T - \rme^{-T} x_0}^2 \leq (1 + \vareps) \normLigne{x_T}^2 + (1+1/\vareps) \rme^{-2T} \normLigne{x_0}^2 \eqsp . 
  \end{equation}
  Let $\vareps >0$ and $x_T \in \rset^d$, we have
  \begin{align}
    &\textstyle{
      p_T(x_T)^{-2} \leq \exp[(1+\vareps)/\sigma_T^2\normLigne{x_T}^2 ] }\\
    & \qquad \qquad \qquad \qquad \times \textstyle{(\int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/(2\sigma_T^2)\normLigne{x_0}^2]\rmd x_0)^{-2} (2\uppi\sigma_T^2)^d  \eqsp .
      }
  \end{align}
  For any $x_T \in \rset^d$, we have
  \begin{align}
    p_\infty(x_T)^2/p_T(x_T) &\leq \exp[\{-1+(1+\vareps)/(2\sigma_T^2)\}\normLigne{x_T}^2 ](2\uppi/\sigma_T^2)^{-d/2} \\ & \qquad \qquad \textstyle{ (\int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/(2\sigma_T^2)\normLigne{x_0}^2] \rmd x_0)^{-1}  \eqsp . }
  \end{align}
  In what follows, we set $\vareps = \rme^{-T}$. We have that
  \begin{equation}
    -1 + (1+\vareps)/(2\sigma_T^2) = (2\sigma_T^2)^{-1}(-2\sigma_T^2 + 1 + \vareps) = -(1 - 2\rme^{-T} + \vareps)/(2\sigma_T^2) = -(1 - \rme^{-T})/(2\sigma_T^2) \eqsp . 
  \end{equation}
  Therefore, we get that
  \begin{equation}
    \label{eq:UNO_de}
    \textstyle{
      \int_{\rset^d} \exp[\{-1+(1+\vareps)/(2\sigma_T^2)\}\normLigne{x_T}^2 ](2\uppi/\sigma_T^2)^{-d/2} \rmd x_T = (1 - \rme^{-T})^{-d/2} \eqsp .
      }
    \end{equation}
    In addition, we have that for any $R \geq 0$ using that $\sigma_T^2 \geq 1/2$ since $T \geq \log(2)/2$
    \begin{align}
      &\textstyle{
        \int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2\normLigne{x_0}^2] \rmd x_0 } \\
      & \qquad \qquad  \geq \textstyle{\probaLigne{X_0 \in \cball{0}{R}} \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2R^2]} \\ 
        & \qquad \qquad  \geq \textstyle{\probaLigne{X_0 \in \cball{0}{R}} \exp[-4\rme^{-T}R^2]
        } \label{eq:inter_DUO}
    \end{align}
    Now let $R^2 = \rme^T$. We obtain
    \begin{equation}
      \textstyle{
        \int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2\normLigne{x_0}^2] \rmd x_0 } \geq \probaLigne{X_0 \in \cball{0}{\rme^{T/2}}} \exp[-4] \eqsp . 
    \end{equation}
    In addition, using Markov inequality, we have
    \begin{equation}
      \probaLigne{X_0 \in \cball{0}{\rme^{T/2}}} = 1 - \probaLigne{\normLigne{X_0}^2 \geq \rme^T} \geq 1 - \expeLigne{\normLigne{X_0}^2} \rme^{-T} \geq 0 \eqsp . 
    \end{equation}
    Therefore, combining this result and \eqref{eq:inter_DUO}, we have
    \begin{equation}
      \label{eq:DUO_de}
      \textstyle{
        \int_{\rset^d} p(x_0) \exp[-\rme^{-2T}(1+1/\vareps)/\sigma_T^2\normLigne{x_0}^2] \rmd x_0 } \geq \exp[-4] (1 - \expeLigne{\normLigne{X_0}^2} \rme^{-T}) > 0 \eqsp . 
    \end{equation}
    We conclude upon combining \eqref{eq:UNO_de} and \eqref{eq:DUO_de}.
  \end{proof}


\section{Entropy bounds and convergence of the backward process}

WE DONT NEED THE ENTROPY BOUNDS ! THE BACKWARD KERNEL CONVERGES

Second, we are going to bound the entropy between $p_t$ and $\pi_\infty$ the
Gaussian distribution with zero mean and identity covariance matrix. To do so,
we are going to provide lower and upper bound on the density.

\begin{lemma}
  Assume \rref{assum:manifold_hyp}. Then for any $t > 0$ we have that
  \begin{equation}
    \KLLigne{p_t^N}{p_\infty} \leq \Cdeux \eqsp , \qquad     \KLLigne{p_t}{p_\infty} \leq \Cdeux \eqsp ,
  \end{equation}
  where we recall that $p_\infty$ is the density w.r.t. the Lebesgue measure of
  the Gaussian distribution with zero mean and identity covariance matrix.
\end{lemma}

\begin{proof}
  Let $N \in \nset$. First, let us
  give an upper-bound $p_t^N$
  independent of $N \in \nset$. We
  have that for any
  $x_t \in \rset^d$
  \begin{equation}
    \label{eq:def_pt}
    p_t^N(x_t) = (1/N) \sum_{k=1}^N \exp[-\normLigne{x_t - m_t X^k}^2/(2 \sigma_t^2)] (2 \uppi \sigma_t^2)^{-d/2} \eqsp . 
  \end{equation}
  In addition, we have that for any $k \in \{1, \dots, N\}$
  \begin{align}
    \normLigne{x_t - m_t X^k}^2 &= \normLigne{x_t}^2 + m_t^2 \normLigne{X^k}^2 - 2m_t \langle x_t, X^k \rangle \geq (1/2) \normLigne{x_t}^2 - m_t^2 \normLigne{X^k}^2 \\
    &\geq (1/2) \normLigne{x_t}^2 - m_t^2 \mathrm{diam}(\M)^2 \eqsp .
  \end{align}
  Combining this result and \eqref{eq:def_pt} we get that
  \begin{equation}
    p_t^N(x_t) \leq q_t(x_t) = (2 \uppi \sigma_t^2)^{-d/2} \exp[-\normLigne{x_t}^2/(4\sigma_t^2)] \exp[m_t^2 \mathrm{diam}(\M)^2/(2\sigma_t^2)] \eqsp .
  \end{equation}
  Using this upper-bound we can now compute a lower-bound on the entropy of $p_t$.
  \begin{align}
    \mathrm{H}(p_t) &= -\int_{\rset^d} p_t(x_t) \log p_t(x_t) \rmd x_t \\
                    &\geq - \int_{\rset^d} \1_{p_t(x_t) \geq 1} p_t(x_t) \log p_t(x_t) \rmd x_t \\
                    &\geq - \int_{\rset^d} \1_{q_t(x_t) \geq 1} q_t(x_t) \log q_t(x_t) \rmd x_t \\
                    &\geq - \int_{\rset^d} q_t(x_t) \absLigne{ \log q_t(x_t)} \rmd x_t \\    
                    &\geq - 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] \expeLigne{\absLigne{\log q_t(X_t)}} \eqsp ,
  \end{align}
  where $X_t$ has Gaussian distribution with zero mean and covariance matrix $2\sigma_t^2 \Id$.
  We have that
  \begin{align}
    \expeLigne{\absLigne{\log q_t(X_t)}}& \leq \abs{(d/2)\log(2\uppi\sigma_t^2)} + m_t^2 \mathrm{diam}(\M)^2/ (2 \sigma_t^2) + d/2 
  \end{align}
  Therefore, we have that
  \begin{equation}
    \label{eq:entropy_bound}
    \mathrm{H}(p_t) \geq - 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] [\abs{(d/2)\log(2\uppi\sigma_t^2)} + m_t^2 \mathrm{diam}(\M)^2/ (2 \sigma_t^2) + d/2 ] \eqsp . 
  \end{equation}
  In addition, we have that
  \begin{equation}
    \label{eq:moment_bound}
    \int_{\rset^d} \normLigne{x_t}^2 p_t(x_t) \rmd x_t \leq 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] 2 d \sigma_t^2
  \end{equation}
  Hence, we get that 
  \begin{equation}
 \KLLigne{p_t^N}{p_\infty} \leq 2^{d/2} \exp[m_t^2 \mathrm{diam}(\M)^2/2\sigma_t^2] \{ 2 d \sigma_t^2 + \abs{(d/2)\log(2\uppi\sigma_t^2)} + m_t^2 \mathrm{diam}(\M)^2/ (2 \sigma_t^2) + d/2 \} \eqsp .     
\end{equation}
Then using that $\pi_t^N$ weakly
converges to $\pi_t$ and using
\cite{dupuis2011weak} we get that the
same result holds replacing $p_t^N$
by $p_t$.
\end{proof}

Remark, choosing $t \geq (1/2) \log(1 + 1/2K)$ implies that $m_t / (2 \sigma_t^2) \leq K$.
Remark, can we remove the dependency w.r.t the dimension by choosing something else instead of $1/2$?


  
  We have the following proposition.

  \begin{proposition}
      Assume \rref{assum:manifold_hyp}.
    \begin{equation}
      \wassersteinD[1](\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{t_0}) \leq C_2 C_3  (...) \exp[-(T-t_0)] \eqsp . 
    \end{equation}
  \end{proposition}

  \begin{proof}
    Let $\nu$ be the optimal
    coupling between
    $\pi_\infty \rmQ_{T-t_0}$
    and $\pi \rmP_{t_0}$
    w.r.t. the total variation
    distance. Using the
    Cauchy-Schwarz inequality we
    have
    \begin{align}
      \wassersteinD[1](\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{t_0}) &\leq \int_{\rset^d \times \rset^d} \normLigne{x-y} \rmd \nu(x,y) \\
                                                                            &\leq \sqrt{2} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \tvnormLigne{\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{t_0}}^{1/2} \\
                                                                &\leq \sqrt{2} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \tvnormLigne{\pi_\infty \rmQ_{T-t_0}, \pi \rmP_{T} \rmQ_{T-t_0}}^{1/2}      \\
                                                                &\leq \sqrt{2} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \tvnormLigne{\pi_\infty - \pi \rmP_{T}}^{1/2}            \\
                                                                &\leq 2^{3/4} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \KLLigne{\pi \rmP_{T}}{\pi_\infty}^{1/4}  \\
      &\leq 2^{3/4} ((\int_{\rset^d} \normLigne{x}^2 \rmd  \pi_\infty \rmQ_{T-t_0}(x))^{1/2} + (\int_{\rset^d} \normLigne{x}^2 \rmd  \pi \rmP_{t_0}(x))^{1/2} ) \rme^{-(T-t_0)/4} \KLLigne{\pi \rmP_{t_0}}{\pi_\infty}^{1/4} \eqsp . 
    \end{align}
  \end{proof}


  (\bbfY_{s,v})_{v\in \ccint{s,u}}
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

